SuperNIC: A Hardware-Based, Programmable, and Multi-Tenant SmartNIC

With CPU scaling slowing down in today's data centers, more functionalities are being offloaded from the CPU to auxiliary devices. One such device is the SmartNIC, which is being increasingly adopted in data centers. In today's cloud environment, VMs on the same server can each have their own network computation (or network tasks) or workflows of network tasks to offload to a SmartNIC. These network tasks can be dynamically added/removed as VMs come and go and can be shared across VMs. Such dynamism demands that a SmartNIC not only schedules and processes packets but also manages and executes offloaded network tasks for different users. Although software solutions like an OS exist for managing software-based network tasks, such software-based SmartNICs cannot keep up with the quickly increasing data-center network speed. This paper proposes a new SmartNIC platform called SuperNIC that allows multiple tenants to efficiently and safely offload FPGA-based network computation DAGs. For efficiency and scalability, our core idea is to group network tasks into chains that are connected and scheduled as one unit. We further propose techniques to automatically scale network task chains with different types of parallelism. Moreover, we propose a fair share mechanism that considers both fair space sharing and fair time sharing of different types of hardware resources. Our FPGA prototype of SuperNIC achieves high bandwidth, low latency performance whilst efficiently utilizing and fairly sharing resources.

==> Makefile <==
MY_DATE := $(strip $(shell date +"%F_%H_%M_%S"))
LATEXDIFF=./latexdiff-so

ifeq ($(OS),Windows_NT)
$(warning Windows NT detected "$(USER)")
DVI = yap
DVIBIN = yap
DISTILL = "$(HOME)"/bin/acrodist.exe

PREFIX=c:\\cygwin\\home\\$(USER)\\papers\\2008SASP-arsenal\\
ACROREAD = "$(HOME)"/bin/acroread.exe
ALL = show_nt
else # mac

ifeq ($(USER),mbt)
ALL = show_nt
ACROREAD = kpdf
else
ALL =  pdf
endif

endif


TEX=$(wildcard *.tex)
FIGS=$(wildcard Figures/*.pdf)
GRAPHS=$(wildcard Graphs/*.pdf)

PDF_TARGETS= paper.pdf
GENERATED = draft.tex rev.tex draft.pdf paper.pdf diff-preamble.tex diff-preamble-new.tex

.PHONY: test_build clean

all: $(ALL)

paper.pdf:  $(TEX) $(GRAPHS) $(FIGS) Makefile paper.bib

paper.ps: paper.pdf
	pdftops paper.pdf paper.ps

singlefile.tex: $(filter-out singlefile.tex,$(TEX))
	echo "" > singlefile.tex
	while read line; do if [ "`echo $$line | grep '^\\input{' | tr '{' ' ' | tr '}' ' ' | awk '{print $$2}'`" == "" ]; then echo $$line >> singlefile.tex; else cat `echo $$line | grep '^\\input{' | tr '{' ' ' | tr '}' ' ' | awk '{print $$2}'`.tex >> singlefile.tex; fi; done < paper.tex

draft.tex: paper.tex Makefile
	perl -ne 's/title\{/title\{r\\input\{rev\}: /g; s/^(\\(numberofauthors|conference|Copy))/\%$$1/; s/texheader/draftheader/g; print' < $< >  $@ || rm -f $@

.PHONY: update_rev
update_rev:
	@REV=$$(svn info * */* 2>&1 | grep "Last Changed Rev" | sort -k4 -n | tail -n 1 | awk '{print $$4}');\
	OLDREV=$$(cat rev.tex);\
	if [ "$$REV" != "$$OLDREV" ]; then svn info * */* 2>&1 | grep "Last Changed Rev" | sort -k4 -n | tail -n 1 | awk '{print $$4}' > rev.tex; fi

.PHONY: draft
draft:
	svn update
	make draft.pdf

draft.pdf: draft.tex update_rev $(TEX) $(GRAPHS) $(FIGS) Makefile paper.bib draftheader.tex


.PHONY: diff
diff: diff-preamble.tex singlefile.tex
	-@rm -rf diffsrc
	-@mkdir -p diffsrc
	@if [ "$$REV" == "" ]; then \
	   echo using head revision, override with REV=1234; \
	   REV=$$(svn info * */* 2>&1 | grep "Last Changed Rev" | sort -k4 -n | tail -n 1 | awk '{print $$4}'); \
	 fi; \
	 SVNURL=$$(svn info | grep URL | awk '{print $$2}'); cd diffsrc; svn co -N -r $$REV $$SVNURL .;
	$(LATEXDIFF) --append-context2cmd="tabcolsep" --flatten --type=UNDERLINE diffsrc/paper.tex paper.tex > diff.tex;
	@mv diff.tex diff2.tex		
	@cat singlefile.tex | grep 'begin{document}' -B99999 | grep -v 'begin{document}' > diff.tex
	@cat diff-preamble.tex >> diff.tex
	@cat diff2.tex | grep 'begin{document}' -A99999 >> diff.tex
	@make diff.pdf
	@rm -rf diffsrc
	@rm diff.tex diff2.tex diff.blg diff.log

diff-new: diff-preamble-new.tex singlefile.tex
	-@rm -rf diffsrc
	-@mkdir -p diffsrc
	@if [ "$$REV" == "" ]; then \
	   echo using head revision, override with REV=1234; \
	   REV=$$(svn info * */* 2>&1 | grep "Last Changed Rev" | sort -k4 -n | tail -n 1 | awk '{print $$4}'); \
	 fi; \
	 SVNURL=$$(svn info | grep URL | awk '{print $$2}'); cd diffsrc; svn co -N -r $$REV $$SVNURL .;
	$(LATEXDIFF) --append-context2cmd="tabcolsep" --flatten --type=UNDERLINE diffsrc/paper.tex paper.tex > diff.tex;
	@cat diff.tex | awk -v RS='(\\\\DIFdelbegin |\\\\DIFdelend )' -v ORS= 'NR%2' > diff2.tex
	@cat singlefile.tex | grep 'begin{document}' -B99999 | grep -v 'begin{document}' > diff.tex
	@cat diff-preamble-new.tex >> diff.tex
	@cat diff2.tex | grep 'begin{document}' -A99999 >> diff.tex
	@make diff.pdf
	@rm -rf diffsrc
	@rm diff.tex diff2.tex diff.blg diff.log

diff.pdf: diff.tex $(FIGURES) $(GRAPHS) Makefile paper.bib


test_build:
	rm -rf _test_build
	mkdir _test_build
	(REPO=$$(svn info | grep URL | sed 's/URL: //');\
	 DIR=$$(svn info | grep URL | sed 's/.*\///');\
	 cd _test_build; \
	 svn checkout $$REPO;\
	 cd $$DIR;\
	 make;\
	 open paper.pdf;\
	)	

%_abbrv.bib: %.bib
	./abbrv.py $< $@

pdf: $(PDF_TARGETS)

%.aux : %.tex $(TEX_STUFF)
	pdflatex $(PDFLATEX_BATCH_OPTIONS) $* 

%.bbl : %.aux 
	bibtex $* || true

%.pdf : %.bbl
	pdflatex $(PDFLATEX_BATCH_OPTIONS) $*
	pdflatex $(PDFLATEX_BATCH_OPTIONS) $*

#
# copies file to prevent write-after-read problems
# uses date as suffix.
#
show_nt: pdf
	- killall $(ACROREAD)
	cp paper.pdf paper_$(MY_DATE).pdf
	$(ACROREAD) $(PREFIX)paper_$(MY_DATE).pdf &

clean:
	rm -rf *.aux *.log *.bbl *.blg *.out $(GENERATED)
	rm -rf paper_abbrv.bib 
	rm -rf _test_build

.PHONY: mailme
mailme: draft.pdf pdf
	@REV=$$(svn info * */* 2>&1 | grep "Last Changed Rev" | sort -k4 -n | tail -n 1 | awk '{print $$4}');\
	CLEAN=$$(if [ "`svn diff | wc -l`" == "0" ]; then echo ""; else echo " modified"; fi);\
	EMAIL=$$(finger `whoami` | head -n1 | tr ' ' '\n' | grep @ | tr '<' ' ' | tr '>' ' ');\
	URL=$$(svn info | grep URL | head -n1);\
	URLSHORT=$$(echo $$URL | tr '/' '\n' | tail -n 1);\
	echo -e "Paper from\n$$URL\nRev: $$REV $$CLEAN\nBuild: $$(date)" | mutt -s "Paper $$URLSHORT @ $$REV $$CLEAN" -a paper.pdf -a draft.pdf $$EMAIL;\
	echo Paper emailed to $$EMAIL



diff-preamble.tex: Makefile
	@echo '\RequirePackage[normalem]{ulem}                                 ' > $@
	@echo '\providecommand{\DIFadd}[1]{{\protect\color{blue}\uwave{#1}}}   ' >> $@
	@echo '\providecommand{\DIFdel}[1]{{\protect\color{red}\sout{#1}}}     ' >> $@
	@echo '\providecommand{\DIFaddbegin}{}                                 ' >> $@
	@echo '\providecommand{\DIFaddend}{}                                   ' >> $@
	@echo '\providecommand{\DIFdelbegin}{}                                 ' >> $@
	@echo '\providecommand{\DIFdelend}{}                                   ' >> $@
	@echo '\providecommand{\DIFaddFL}[1]{\DIFadd{#1}}                      ' >> $@
	@echo '\providecommand{\DIFdelFL}[1]{\DIFdel{#1}}                      ' >> $@
	@echo '\providecommand{\DIFaddbeginFL}{}                               ' >> $@
	@echo '\providecommand{\DIFaddendFL}{}                                 ' >> $@
	@echo '\providecommand{\DIFdelbeginFL}{}                               ' >> $@
	@echo '\providecommand{\DIFdelendFL}{}                                 ' >> $@


diff-preamble-new.tex: Makefile
	@echo '\RequirePackage[normalem]{ulem}                                 ' > $@
	@echo '\usepackage{comment}                                            ' >> $@
	@echo '\excludecomment{DIFdelregion}                                   ' >> $@
	@echo '\providecommand{\DIFadd}[1]{{\protect\color{blue}\uwave{#1}}}   ' >> $@
	@echo '\providecommand{\DIFdel}[1]{{\protect\color{red}\sout{#1}}}     ' >> $@
	@echo '\providecommand{\DIFaddbegin}{}                                 ' >> $@
	@echo '\providecommand{\DIFaddend}{}                                   ' >> $@
	@echo '\providecommand{\DIFaddFL}[1]{\DIFadd{#1}}                      ' >> $@
	@echo '\providecommand{\DIFdelFL}[1]{\DIFdel{#1}}                      ' >> $@
	@echo '\providecommand{\DIFaddbeginFL}{}                               ' >> $@
	@echo '\providecommand{\DIFaddendFL}{}                                 ' >> $@
	@echo '\providecommand{\DIFdelbeginFL}{}                               ' >> $@
	@echo '\providecommand{\DIFdelendFL}{}                                 ' >> $@





==> algo-fairness.tex <==
\begin{algorithm}[tb]
 \caption{Fairness algorithm pseudo-code}
\label{algo-fairness}

\SetAlgoLined
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\SetKwComment{Comment}{/* }{ */}

$F$: FPGA Fabric \\
$I$: ingress Bandwidth \\
$E$: egress Bandwidth \\
$M$: memory \\
\BlankLine
$n$:   Number of users\\
$k_i$: Number of DAGs for user $i$\\
\BlankLine
\textbf{Input for user i:} \\
$Demand_i$ \\ \Comment*[r]{Ingress bandwidth demand for user $i$}\\
$Chain\_ratio_i=\langle chain_{i,1}, ... chain_{i,k_i} \rangle$ \\
\BlankLine
\textbf{Internal states:} \\
$R=\langle r_{F}, r_I, r_E, r_M \rangle$ \Comment*[r]{resource capacity}\\
$C=\langle c_{F}, c_I, c_E, c_M \rangle$ \Comment*[r]{resource consumed}\\
$U_{i}=\langle u_{F}, u_I, u_E, u_M \rangle$ \Comment*[r]{user $i$'s allocation}\\
$s_i\ (i=1..n)$ \Comment*[r]{user $i$'s dominant share}\\
$A_{p}=\langle a_{1}, .. a_p \rangle$ \Comment*[r]{number of regions for chain $p$}\\

%\Output{}

\BlankLine
\BlankLine

\Comment*[r]{\textbf{Calculate demand vectors:}}\\
\ForEach{User: $i = 1..n$}{
    \ForEach{Resource: $m = [F, I, E, M]$}{
        $D_{i,m} = \sum_{j=1}^{k_i}Demand_{i} * Chain\_ratio_{i,j}$
    }
}

\textbf{Space-sharing Phase (DRF):}\\
\textbf{pick} user $i$ with lowest dominant share $s_i$\\
$D_i \leftarrow$ demand of user $i$ \\
  \eIf{$C+D_i <= R$}
  {
    $C = C + D_i$\\
    $U = U_i + D_i$\\
    $s_i = \max^{m}_{j=1}\{u_{i,j}/r_j\}$\\

  }
  {
%  \ForEach{\mathtext{MR} that the attacker has access to}{
%     \If{\mathtext{MR} $\ne$ victim's MR}{
%         insert \mathtext{MR} into \mathtext{MR\_set}\; 
%     }
%  }
%\mathtext{index\_bits \leftarrow 10};\ \ \ %\mathtext{high\_index\_start \leftarrow 12}\;
  \Comment*[r]{Calculate \nt\ chain allocation for region}
   $A_p = \lceil (\sum_{i=1}^{n} U_{i,F} * Chain\_ratio_{i,p}) / Chain_F \rceil$\\
   \algorithmicreturn\ {$A$}
  }

%\BlankLine
%  \ForEach{\mathtext{MR} in \mathtext{MR\_set}}{
%    perform 8-byte \rdma-read to \mathtext{MR}\;
%  }      
\textbf{Time-sharing (DRFQ):}

\end{algorithm}


==> design_yizhou.tex <==
\input{tbl-techniques}

\if 0
\section{\sysname\ Overview}
\label{sec:overview}

We walk through the key challenges and present out solutions.

\boldunderpara{Key Challenges:}
\begin{itemize}[leftmargin=0cm,itemindent=.35cm]

\myitem{C1:}
After decoupling the network, what's left at the endpoints?
And how can endpoints communicate with the NetPool?
%
\textbf{Answer:} \TODO{}
We observe that a reliable link layer is sufficient
to connect endpoints and NetPool.
We design a shim library at the endpoints.

\myitem{C2:}
How to efficiently and safely consolidate applications onto NetPool
with limited amount of resource?
%
\textbf{Answer:} \TODO{}
Scheduling: space and time sharing limited resource.
Auto Scaling: xxx.
Isolation: segmented virtual memory, XXX.
Fairness: PIFO, XXX.



\myitem{C3:}
How to design a flexible management interface so that
we can deploy, upgrade, scale applications easily?
\textbf{Answer:}
Although FPGA enables in field reconfiguration,
it is far from a complete solution.
In response, \sysname\ makes a clean separation between the management and data plane.
The management plane makes decisions based on runtime policies
and react to real time traffic load. The data plane simply follows
the management plane's instructions and adapts its computation layout.
We build the management plane using C running at softcores.
As a result, \sysname\ has software-alike configurability
while able to run at raw hardware speed.

\myitem{C4:} The NetPool adds another hop in the path and is
shared by many applications, how to ensure low latency and high throughput?
%
\textbf{Answer:}
Latency: we make two technical contributions.
a) to optimize the common case, we propose \textif{partial chaining}
to shorten the connection latency between chained functions.
b) we use service-level parallelism to shorten critical path.
Throughput:
we use \textit{resource partitioning} and ensure SuperNIC's system
component (e.g., packet scheduler) is able to sustain peak throughput.
\yizhou{partitioning maybe beneficial for side channels}.
When consolidated computation exceeds SuperNIC's capacity,
we use either time- or space-sharing to multiplex resource.
As a result, the execution latency build up.
We trade some extra latency for the consolidation benefits.
Luckily, we obverse that datacenter traffic is bursty and mostly underutilized,
thus peak load scenario is rare.

\myitem{C5:} Failure.
The failure domain is enlarged.
Shall we handle it? If so, how?
Make endpoints multi-homed. Add another link
to switch or to another sNIC.

\yizhou{other challenges: tail latency. security, side channels, programming framework.}

\yizhou{for latency part: it would be great to say:
we obverse the average chain length is XXX,
and we find XX\% traffic will traverse N NFs.
Also, in our eval, during low load, we found offloading transport and NF
to SuperNIC actually improves latency compared to baselin (running transport
on CPU or smartnic like bluefield.)
}

\end{itemize}
%
\\


\textbf{Features}

1. Distributed setup.
A resource pool has set of connected SuperNIC, in mesh or others.
3 planes.
Traffic can bounce among SuperNICs.
Load balancing. (\TODO{depends.})

2. Resource consolidation and abstraction groups.
Describe how end points can choose to offload whatever to supernic,
they could enjoy flexible combo. (this is essentially our Abstraction discussion earlier.)

3. New smartnic architecture.
Highlight prior archs, esp PANIC, show the difference.
Our arch has the benefits of both worlds (we have a diagram for this).

4. Packet Processing Parallelism.
We introduce service-level and instance-level parallelism.
And to ensure ordering, we introduce Reorder Buffer, a mechanism that XXX.

5. Runtime NF Scheduling and scaling, time and space sharing.
We closely monitor NF status and does automatic NF scheduling and scaling

6. Performance Isolation and Protection.
We have virtual memory interface for on-board memory.
We use PIFO and other things to control bandwidth etc.
\fi

\section{\sysname\ Design Yizhou}
\label{sec:design}

\subsection{Overview}

SuperNIC's innovation comes from two parts, the board-level design and the distributed design.

\subsubsection{At Board-Level}

We adopt PANIC’s architecture as our baseline.
Its design enables resource consolidation and flexible NF chaining.
Despite its advantages over traditional RMT, Pipeline, and SoC-based SmartNICs, PANIC suffers from long chaining latency and cannot scale resources.

We propose three techniques to improve this state-of-the-art SmartNIC architecture, namely, 1) traffic-aware NF merging, 2) eager credit allocation scheduling, 3) on-demand scheduling and auto-scaling. These techniques are crucial for reducing latency and enable flexible consolidation. We will cover the details later. (NF merging has two benefits: reduce latency, and increase slot resource utilization while reducing the pressure on the xbar. We need experiments to show.)

In addition, we introduce a softcore (could be a real SoC in the future)
to run the management and control plane tasks.
Our microservice-style software is partitioned into \texttt{agents}.
Each agent is responsible for one particular task, e.g., we currently have monitoring agent, auto-scaling agent, Inter-SuperNIC agent, PR agent, and so on.
It presents a shell-alike interface hence administrates can control SuperNIC via simple commands. 

In all, a single SuperNIC supports multi-tenancy chaining,
traffic-aware NF merging, on-demand scheduling, and auto scaling.
It presents flexible policies with a clean separation of data and management/control planes.

\subsubsection{At Distributed-Level}

A single SuperNIC has limited resources and may become the computation bottleneck during peak load.
To tackle this issue, we leverage the fact that SuperNICs under one ToR are
connected in a ring or a mesh.
We \textit{logically} group such a pool of physically distributed SuperNICs as one giant computation entity.
Within the pool, SuperNICs are able to auto-scale, migrate, and balance computation among each other.

We offer two-level auto-scaling, in which a certain computation offload
can not only scale-up within one SuperNIC
but also scale-out across SuperNICs.
On top of it, SuperNICs can migrate computation and balance traffic on demand.

These designs are possible because of the following components.
First, each SuperNIC board has extensive monitoring facilities collecting runtime statistics for software agents to consume and make decisions using flexible policies.
Second, our fast PR mechanism serves as the basis.
Third, we deploys a hardware routing agent to help re-route traffic.

\subsection{Physical Connections}

\textit{Endpoints and Link Layer}.
We need to describe what's the minimum setting required at the endpoint side. The minimum setting is used when the whole transport and NF are moved to SuperNIC.
The minimum setting should include: a) a reliable link layer, with one-hop flow control, error detection and correction. b) a shim layer exposed to applications. this layer needs to save at least the connection IDs.
I'm a bit worried about the error correction part - what if we cannot guarantee
100\% error-free, then what's the guarantee we offer to endpoints.
We had discussion on this part before, e.g., expose bit error as network failure.

\subsection{On-chip Architecture}

\yizhou{Overview. Add a figure.}

\subsubsection{Parser}
Each RX port has a Parser attached. All parsers share a service chain store.
The parser uses Match-Action-Table style to generate a runtime
descriptor for each packet.
This descriptor is a metadata placeholder, includes XXX.

\subsubsection{Central Scheduler}

\yizhou{Deserves a zoom-in figure.}

\textbf{On-demand and eager credit management}:
The classical pull and push model proposed by
Click (used by PANIC) is designed for single element/NF.
With a NF chain, especially consider the extra cost
of going back to Scheduler or going across xbar,
it is beneficial to favor push over pull.
Mapping to our model, we propose on-demand
and eager credit management.

On-demand credit allocation:
If a packet is going to use a NF, the packet must allocate credit right before traversing the NF.
Hence, if a packet needs to traverse a NF chain, the packet must go back to the central scheduler to
allocate credit for the next NF in the chain. 

Eager credit allocation:
The packet can pre-allocate credits for services it going to use.
Hence, if a packet wants to traverse a NF chain, the packet would 
allocate credits for all NFs in the chain.
Implication: a packet will wait until all NFs in a chain have available credits.

Eager credit pre-allocate resources, lower latency, but may have poor resource utilization.
We think the eager should be the default policy during low load.
We should switch to on-demand when load spikes.

\subsubsection{Parallelism}
Reorder buffer.

Three-level parallelism.
1) pipeline level.
2) fine-grained, needs help from a PL framework.
3) service-level, coarse-grained. Either manual linking, or use a high-level scripting language like Click.
4) instance-level, among instances of the same service.

For now, 1) come from user, 2) is our future work,
We can do 3), manually. We have to do 4).
Both 3 and 4 need the help of ROB.

\yizhou{we could briefly mention that this can benefit from a programming framework. The PL part is deferred to the Discussion section.}

\subsubsection{Service Scheduling}
Mechanism: we use counters. rely on fpga PR, a softcore.
Policy: based on counters? once it exceeds/lowers than XXX, we do YYY.

\subsubsection{Abstraction Groups}

0. Wrapper, and other facilities: slot, PR wrapper, etc.

1. Transports (what about congestion control?)
2. Network Function

\if 0
\subsubsection{NF Shell}
We expose a standard shell abstraction to each running NF.
The shell is analogous to a system call interface,
through which NF will communicate with the rest of SuperNIC.
The shell has several standard signals such as fixed clock (250 MHz),
a pair of network interface, memory access interface, and control signals. Amazon F1 has a similar shell.
\fi

\subsubsection{Security Measures}
Consolidating resource means we need security measures.
1) NFs are only allowed to access shared resource via a fixed set of interfaces provided by shell. This reduced the exposed attack surface.
2) On-board memory employs a simple segment-based permission checking.
3) From FPGA's perspective, the generation framework (we should have a section describing what's this) would do security checks during compilation time, to filter FPGA side-channels designs (bunch papers on this).

\subsection{Distributed SuperNICs}

\subsubsection{Scale-out}
\subsubsection{Migration}
\subsubsection{Hardware Routing Agent}



==> discussion.tex <==
\section{Discussion}

\subsection{Programming Model}
Couple points.
1) why we need such a PL model?
2) what's in this PL model?
3) the challenges and benefits of designing/using this PL model?

We could benefit from having a programming framework, like ClickNP, the ones
that provide APIs to do packet processing. Through these APIs,
SuperNIC can do better scheduling etc.
We do not have such model yet.
Ideally, such model can be:
1) a way to describe services, their linking etc.
And SuperNIC is able to infer better NF merging and runtime scheduling policies.
2) a set of shell interfaces through which NFs interact with SuperNIC.

Also its worth mentioning: it is user/system's responsibility to partition
the function among endpoints and SuperNIC. 

\subsection{Failure}

We restrict out discussion to transient failures.
We assume permanent failures are rare.
SuperNIC adds back fate-sharing failure domain (all the connected devices and the SuperNIC). It is making failure handling a bit worse than a full disaggregation model.

Ideally, we want SuperNIC be able to physically isolate its on-board
failure domains, possibly by using different power supplies and chips.
For example, the board has two domains, one pass-through and one computation domain.
The latter hosts all logic and softcore.
If the latter fails, SuperNIC is still able to route traffic via the pass-through domain hence the connected
devices are still reachable from others.

\subsection{Security and FPGA Side-Channels}

We ensure security by properly isolate resources.
FPGA side-channels are possible, but they can be prevented
during compile time by checking user logic.
Most malicious FPGA programs have a certain signature logic.


==> dist.tex <==
\subsection{Distributed SuperNIC}
\label{sec:dist}

%\notearvind{Make this a subsection of previous section so its size doesn't stand out?}
The design discussion so far focused on a single \snic. To enable better consolidation and network as a service, we 
%When we use a single \snic\ to consolidate \nt{}s of its connected endpoints, the \snic\ needs to be provisioned with the aggregated peak load of these endpoints.
%To further reduce cost, we 
build a rack-scale distributed \snic\ platform that enables one \snic\ to use other \snic{}s' resources (\textbf{G6}).
With this platform, a rack's \snic{}s can collectively provision for the maximum aggregated load of all the endpoints in the rack.

%\boldpara{Distributed Control Plane.}~~
SoftCores on the \snic{}s in a rack form a distributed control plane. 
They communicate with each other to exchange metadata and cooperate in performing distributed tasks. % like \nt\ migration and memory swapping.
We choose this de-centralized design instead of a centralized one, because the latter requires another global manager and adds complexity and cost to the rack architecture. %\zac{I am not sure about this argument -- I have heard that other places (e.g. google) have used the centralized manager architecture because it's easier to build and deploy than P2P ones. I personally don't buy this argument either. Do you have stronger support?}
Every \snic\ collects its FPGA space, on-board memory, port bandwidth, and individual \nt{} usage, which it periodically sends to all the other \snic{}s in the rack.
Each \snic\ thus has a global view of the rack. When an \snic\ is overloaded with some \nt\ chain being the bottleneck, it first finds if another \snic\ has available bandwidth, is running the same \nt{} chain, and has remaining bandwidth on the chain. If so, the \snic\ redirects traffic to this other \snic{}, by setting a rule in the parser MAT for packet forwarding.
If there are more than one \snic{}s that can handle the traffic, the \snic\ picks the one that is closest in distance to it (\ie, fewest hops).

%to forward certain packets (\eg, ones to be processed by an \nt\ chain on another \snic) to the remote \snic.

%\notearvind{We could also talk about something more basic - if the same NT is loaded on many snics, we can balance the load across all instances and achieve good consolidation. Maybe that would be easier for reviewers to accept before we talk about NT migration.}

%\boldpara{\nt\ Migration.}~~
If an \snic\ is overloaded and no other \snic{}s currently have corredponding \nt\ chain available, the \snic\ tries to launch the chain at another \snic.
Specifically, %the \snic's SoftCore first identifies the set of \snic{}s in the same rack that have available resources to host the \nt\ chain.
the \snic's SoftCore then sends the bitstreams of the \nt{} chain to a remote \snic\ that has free space. This remote \snic\ launches the chain in one of its own free regions.
When the original \snic\ has a free region, it moves back the migrated \nt\ chain. 
%It does so by first launching the \nt\ chain locally, then removing the MAT tunneling rule, and finally instructing the remote \snic\ to remove its \nt\ chain.
If the \nt\ chain is stateful, then the SoftCore manages a state migration process after launching the \nt\ chain locally, by first pausing new traffic, then migrating the \nt's states. % from the remote \snic\ to the local \snic. %and finally removing the MAT rule.



==> extended_abstract.tex <==
%\documentclass[pageno]{jpaper}
%\newcommand{\asplossubmissionnumber}{234}
%\usepackage[normalem]{ulem}
%\begin{document}

\title{Disaggregating and Consolidating Network Functionalities with SuperNIC}
\date{}
\maketitle
\thispagestyle{empty}

\if 0
\twocolumn[
    \begin{@twocolumnfalse}
    \begin{center}
	{\Large\bf Disaggregating and Consolidating Network Functionalities with SuperNIC}
    \end{center}
    \smallskip
%    \centerline{Yizhou Shan}
%    \centerline{\em UCSD}
    \end{@twocolumnfalse}
]
\fi

{\em Resource disaggregation}, a concept that organizes hardware resources as separate types of network-attached pools instead of as monolithic servers, has quickly gained popularity in both academia and industry in recent years~\cite{Shan18-OSDI,HP-TheMachine,IntelRackScale,FireBox-FASTKeynote,Tsai20-ATC,Nitu18-EUROSYS,DDC-hotcloud20,Ali-SinglesDay}.
Existing production and research disaggregated systems have focused on separating three types of resources: compute (processing)~\cite{Shan18-OSDI,any-gpu-disagg-work}, memory (or persistent memory)~\cite{Shan18-OSDI,HP-TheMachine,Lim09-disaggregate,Aguilera-FarMemory,Tsai20-ATC}, and storage~\cite{cao2018polarfs,SnowFlake-NSDI20}.
%These efforts have seen real success, and more data centers have started to adopt disaggregation at the production-scale~\cite{Ali-SinglesDay}.
%For example, Alibaba listed their disaggregated storage solution as a key enabling factor of serving 544,000 orders per second during their shopping festival~\cite{Ali-SinglesDay}.

The fourth major resource in computing, \textit{network}, has been completely left out in resource disaggregation research.
No work has attempted to disaggregate the network.
At first glance, ``network'' cannot be disaggregated from either a traditional monolithic server or a disaggregated device, as they both need to be attached to the network.

\section{Key Insights and Proposal}
Our insight is that even though each endpoint still needs its own network interface, its \emph{network-related tasks} such as a layer in the network stack or a customized network function do not have to run at the endpoint, \ie, they could potentially be disaggregated and run as a separate resource pool.  

With this insight, we propose to \textit{segregate} network tasks (or {\em \nt{}s}) from individual endpoints and \textit{consolidate} them in a network resource pool.
This pool consists of a distributed set of \textit{SuperNIC}s (or \textit{\snic} for short), a new programmable device that executes \nt{}s for the endpoints.
Each \snic\ connects to a small set of endpoints (\eg, 4 to 8) and a ToR switch,
and all \snic{}s are connected, \eg, as a ring.
%Together, the disaggregated \snic\ pool offers \textit{Network Functionality as a Service} ({\em NFaaS}).
In building \snic, we answer six key research questions.
%it is an essential part after disaggregation,

\vspace{0.05in}
\noindent \textbf{\textit{What is the benefit of disaggregating and consolidating network functionalities?}} 
To answer this question, we study network communication patterns and needs in the traditional server-based data-center environment and in the disaggregated data-center environment by understanding the unique architecture of these environments and by analyzing real-world network traces.
We discover three potential benefits of network disaggregation and consolidation for the disaggregated environment: it enables an existing rack and ToR switch to host a large number of disaggregated devices; it avoids the need to implement hardware and/or software units for \nt{}s at each type of device; and it uses less hardware resources to run \nt{}s.
Server-based data centers share the last and to some extent the second benefits.
To elaborate on the last benefit, the cost saving comes from the fact that both server-based and disaggregated data centers exhibits a highly bursty pattern.
Thus, after consolidation, an \snic{} only needs to provision the \textit{aggregated} peak bandwidth and hardware utilization,
while traditional endpoints need to each provision for its own peak.


\vspace{0.05in}
\noindent \textbf{\textit{What network functionalities should be disaggregated?}}
To answer this question, we explore two dimensions.
In the first dimension, we consider what type of \nt{}s that would benefit from disaggregation and consolidation for different types of endpoints. 
For example, regular servers could offload their TCP transport to \snic\ and potentially share one transport at \snic\ for consolidation.
Servers and disaggregated devices could also offload various network functions like encryption and filtering or application-specific functions like caching and replication.

In the second dimension, we explore where different parts of an \nt{} should be located.
We separate each network functionality into three parts: computation logic (\eg, transmission protocol), states (\eg, packet sequence number, connection information), and data (\eg, un-acknowledged send buffer, or un-ack buffer).
While traditional network solutions bundle all three at one location (host CPU or host NIC), with \sysname's flexible offloading choice, each part of each network functionality could sit at different locations.
For example, the link-layer logic and states and transport-layer states could be at an endpoint, while the link-layer un-ack buffer, transport logic and un-ack buffer for this end host could be maintained at its connected \snic.
Such flexibility could potentially unlock new ways to build network stacks and functions and new mechanisms to provide end-to-end reliability, and it will be especially useful when exploring customized communication abstractions for disaggregated devices.

\vspace{0.05in}
\noindent \textbf{\textit{How to consolidate network functionalities in a way that maximizes the utilization of \snic{} hardware resources while ensuring fairness and minimizing impact on application execution?}}
Instead of provisioning for the peak load at each individual end point, we leverage statistical multiplexing to provision for the aggregated peak load of all connected end points at an \snic.
We achieve this goal with three techniques: 1) sharing an \snic's hardware resources across different \nt{}s ({\em space sharing}), 2) sharing the same \nt{} across different applications ({\em time sharing}), and 3) configuring the same hardware resources for different \nt{}s at different time ({\em time sharing with context switching}).
%Our goal of network disaggregation is to reduce the total amount of hardware resources (CapEx and OpEx) compared to no disaggregation (\ie, each endpoint hosts its own network device for all its network functionalities) while achieving application performance on par with no disaggregation. 
%For 1), we partition the reconfigurable hardware resource of an \snic\ (\eg, FPGA logic cells, on-chip memory, etc.) into fix-sized {\em regions}, each of which can be reconfigured independently. 
%A region can be configured to run different \nt{}s over time.
Space sharing is relatively straightforward and has no side effect; we partition the FPGA space to chunks of different sizes, with each hosting one or more \nt{}s.
On the other hand, time sharing is more challenging, as it could potentially impact application performance and fairness.
Moreover, context switching would hurt application performance a lot more as reconfiguring an area on reconfigurable hardware is orders of magnitude slower than processing a packet.

We solve these challenges by designing policies and mechanisms that leverage the flexiblity network disaggregation and our \snic\ brings.
Our policies include heuristics that favor space sharing over time sharing and fallback to context switching as the last resort. Before starting context switching, we first try migrating the \nt\ to another \snic\ and give applications a chance to mitigate the problem (\eg, by slowing down the sending speed or by switching to software implementation of the \nt). We also frame \nt\ allocation as a multi-dimensional resource allocation problem and considers Dominant Resource Fairness~\cite{DRF} when making the allocation decision.
Our mechanisms focus on reducing the need to reconfigure spaces and on {\em hiding} the reconfiguration performance overhead. We use a technique similar to victim cache for the former. For the latter, we always leave one or more empty slots to quickly start new \nt{}s, while in the background we evict least used \nt{}s to make more empty slots.

\vspace{0.05in}
\noindent \textbf{\textit{How to achieve high-throughput, low-latency, and scalable performance?}}
When we consolidate the \nt{}s of multiple endpoints to one \snic, the \snic\ should provide high throughput for all the endpoints, minimize latency overhead spent at \snic, and be able to handle many concurrent \nt{}s.
We provide high throughput by two levels of parallelism:
{\em \nt{} parallelism} where a packet goes through multiple \nt{}s in parallel and {\em instance parallelism} where we launch multiple instances of the same \nt{} to handle different packets in an application.
\snic\ automatically scales an \nt{} out/down as its load increases/decreases. 
To achieve low latency and scalability, we propose a scheduling system that centers around a new notion, {\em \nt\ chaining}.
The idea is to group \nt{}s that are likely to be executed in a sequence into a chain and to have our central scheduler schedule packets only once for the entire chain. 
Our scheduler reserves credits for the entire chain and only sends packets over when there are credits.
Doing so avoids going through scheduler after each \nt\ and thus improves both packet-processing latency and scheduler scalability.
Finally, to accomodate more types of \nt\ combinations, we support skipping arbitrary \nt{}s in a chain (\eg, a chain falls back to a single \nt\ when all other \nt{}s are skipped).


\vspace{0.05in}
\noindent \textbf{\textit{How to build and utilize a distributed \snic{} framework?}}
When one \snic\ is overloaded and need to accommodate too much network bandwidth, on-chip hardware resources, or off-chip memory space, traditional solutions would drop packets or an entire \nt{} to make room for others or to provision a larger \snic. The former impacts application performance and the latter results in resource wastes when loads are not at their peaks. 
Our idea is to utilize other \snic{}s to handle load spikes, based on the observation that not all \snic{}s under a rack would run at their peak load at the same time. Essentially, with distributed \snic{}s, we provision for the maximum aggregated bandwidth in a rack instead of the sum of peak loads under each \snic.
Specifically, to support overloaded network bandwidth or on-chip hardware resources at an \snic, we create an \nt\ at another \snic\ (one with light load). 
The current \snic\ then only serves as a simple pass-through device to redirect packets to the new \snic, with the latter sending packets to the next hop after processing them.
To support overloaded memory space at an \snic, we deploy a {\em transparent} swapping mechanism that swaps colder data to another \snic's memory.

\vspace{0.05in}
\noindent \textbf{\textit{How to best exploit \snic{}s to build disaggregated applications?}}
While network disaggregation has its benefits in resource and port consolidation, independent network resource scaling and management, it offers additional unique benefits to disaggregated applications. 
We made an initial exploration in this direction with two examples.
First, we explore a customized network abstraction for disaggregated memory device: a key-value store interface (rather than the standard messaging interface).
Second, we explore using \snic{}s as centralized, in-network computation for tasks like data replication, caching, and \fixme{XXX}.


In building \snic\ and its distributed framework, we separate data and control plane, with the former performed in ASIC and FPGA and the latter done in software.
We prototyped \snic\ with FPGA (Xilinx \fixme{XXX}) and connect \snic{}s with both regular server and disaggregated devices.
We demonstrate \snic's benefits and tradeoffs by disaggregating and consolidating three types of network functionalities:
a go-back-N reliable transport, a set of network functions including firewall, AES, and \fixme{XXX}, and a set application-specific functions including \fixme{XXX}.
We evaluated these scenarios with micro- and macro-benchmarks and compared \snic\ with no disaggregation and disaggregation using a device similar to a recent programmable NIC~\cite{PANIC}.
Our results show that \fixme{XXX}.
We will open source \snic\ upon the publication of this paper.



%\pagebreak
%\bibliographystyle{plain}
%\bibliography{references}
%\end{document}


==> fig-architecture.tex <==
{
\begin{figure*}[th]
\begin{center}
\centerline{\includegraphics[width=\textwidth]{Figures/fig-architecture.pdf}}
\mycaption{fig-arch}{\system\ Architecture}
{
%
}
\end{center}
\end{figure*}
}

==> fig-chip-arch.tex <==
{
\begin{figure}
\begin{center}
\centerline{\includegraphics[width=0.8\columnwidth]{Figures/fig-chip-arch.png}}
\mycaption{fig-chip-arch}{\sysname Architecture.}
{

}
\end{center}
\end{figure}
}


==> fig-eval3.tex <==
{
\begin{figure}[th]
\begin{center}
\centerline{\includegraphics[width=3.2in]{Figures/drf.pdf}}
%\vspace{-0.2in}
\mycaption{fig-drf}{\nt{} Scheduling.}
{
SO: Scaling Out.
}
\end{center}
%\vspace{-0.3in}
\end{figure}
}

==> fig-eval6.tex <==
{
\begin{figure*}[th]
\begin{minipage}{1.65in}
\begin{center}
\centerline{\includegraphics[width=\columnwidth]{Figures/fig3_tput.pdf}}
\vspace{-0.13in}
\mycaption{fig-dummy-nt-chain-lat-50}{Real \nt{} DAG Pipeline throughput 50 cycle NT.}
{
}
\end{center}
\end{minipage}
\begin{minipage}{1.65in}
\begin{center}
\centerline{\includegraphics[width=\columnwidth]{Figures/fig3_lat.pdf}}
\vspace{-0.13in}
\mycaption{fig-dummy-nt-chain-tput-50}{Real \nt{} DAG Pipeline latency 50 cycle NT.}
{
}
\end{center}
\end{minipage}
\begin{minipage}{1.65in}
\begin{center}
\centerline{\includegraphics[width=\columnwidth]{Figures/fig3_tput_10d.pdf}}
\vspace{-0.13in}
\mycaption{fig-dummy-nt-chain-lat-10}{Real \nt{} DAG Pipeline throughput 10 cycle NT.}
{
}
\end{center}
\end{minipage}
\begin{minipage}{1.65in}
\begin{center}
\centerline{\includegraphics[width=\columnwidth]{Figures/fig3_lat_10d.pdf}}
\vspace{-0.13in}
\mycaption{fig-dummy-nt-chain-tput-10}{Real \nt{} DAG Pipeline latency 10 cycle NT.}
{
}
\end{center}
\end{minipage}
\vspace{-0.1in}
\end{figure*}
}

==> fig-fairness-tput.tex <==
{
\begin{figure}[th]
\begin{minipage}{2.9in}
\begin{center}
\centerline{\includegraphics[width=0.7\columnwidth]{Figures/tput.png}}
\vspace{-0.1in}
\mycaption{fig-tput}{Aggregated Throughput}{}
\end{center}
\end{minipage}
\vspace{-0.1in}
\end{figure}
}

==> fig-one-fig-example.tex <==
{
\begin{figure*}
\begin{center}
\centerline{\includegraphics[width=\textwidth]{Figures/WideMissing.pdf}}
\mycaption{fig-fig3}{Example Figure 3.}
{
blabla
}
\end{center}
\end{figure*}
}


==> fig-osdi16-net-trace.tex <==
{
\begin{figure*}
\begin{minipage}{0.25\textwidth}
\begin{center}
\centerline{\includegraphics[width=\textwidth]{Figures/fig_fb_alibaba_trace.pdf}}
\vspace{-0.1in}
\mycaption{fig-fb-alibaba}{Consolidation Analysis of Facebook and Alibaba Traces.}
{
Load represent relative amount and have different units for FB and Alibaba.
}
\end{center}
\end{minipage}
\begin{minipage}{0.25\textwidth}
\begin{center}
\centerline{\includegraphics[width=\textwidth]{Figures/spike-trace-analysis.pdf}}
\vspace{-0.1in}
\mycaption{fig-spike-var}{Load Spike Variation across Endhosts in FB.}
{
}
\end{center}
\end{minipage}
\begin{minipage}{0.5\textwidth}
\begin{center}
\centerline{\includegraphics[width=\textwidth]{Figures/fig-osdi16-net-trace.pdf}}
\vspace{-0.15in}
\mycaption{fig-OSDI16NetTrace}{Network traffic for accessing disaggregated memory.}
{
}
\end{center}
\end{minipage}
\vspace{-0.15in}
\end{figure*}
}


==> fig-topology.tex <==
{
\begin{figure}
\begin{center}
\centerline{\includegraphics[width=\columnwidth]{Figures/fig-topology.pdf}}
\vspace{-0.1in}
\mycaption{fig-topology}{Possible Architectures of Network Disaggregation.}
{
Pink boxes represent disaggregated pools. 
}
\end{center}
\vspace{-0.2in}
\end{figure}
}


==> fig-two-fig-example.tex <==
{
\begin{figure*}[th]
\begin{minipage}{\figWidth}
\begin{center}
\centerline{\includegraphics[width=\figWidth]{Figures/NarrowMissing.pdf}}
\mycaption{fig-fig1}{Example Figure 1.}
{
blabla
}
\end{center}
\end{minipage}
\begin{minipage}{\figSep}
\hspace{\figSep}
\end{minipage}
\begin{minipage}{\figWidth}
\begin{center}
\centerline{\includegraphics[width=\figWidth]{Figures/NarrowMissing.pdf}}
\mycaption{fig-fig2}{Example Figure 2.}
{
blablabla
}
\end{center}
\end{minipage}
%\vspace{-0.1in}
\end{figure*}
}


==> implementation.tex <==
\section{Implementation}
\label{sec:implementation}


==> intro-v1.tex <==
\section{Introduction}
\label{sec:intro}

{\em Hardware resource disaggregation} is an architecture that decomposes full-blown, general-purpose servers into segregated, network-attached hardware resource pools, each of which can be built, managed, and scaled independently. With disaggregation, resources can be allocated from any device in their corresponding pools, exposing vast amounts of resources to applications and at the same time improving resource utilization. Disaggregation also allows data-center providers to independently deploy, manage, and scale different types of resources.
Because of these benefits, disaggregation has gained significant traction from both academia~\cite{LegoOS,FireBox-FASTKeynote,ATC20-pDPM,Nitu18-EUROSYS,DDC-hotcloud20,aifm-osdi20,semeru,kona,infiniswap,fastswap} and industry~\cite{HP-TheMachine,IntelRackScale,alibaba-polardb,facebook-disaggregation,SnowFlake-NSDI20}.

While increasing amounts of effort go into disaggregating compute~\cite{LegoOS,disagg-gpu}, memory (or persistent memory)~\cite{LegoOS,HP-TheMachine,Lim09-disaggregate,remote-region-atc18,ATC20-pDPM,semeru,infiniswap,fastswap,hotpot-socc17}, and storage~\cite{PolarFS-VLDB18,SnowFlake-NSDI20,hailstorm-asplos20,ana-eurosys16,gimbal}, the fourth major resource, \textit{network}, has attracted little attention.
Today, both servers and disaggregated devices spend significant resources on running software and/or hardware for network communication, such as transport layers, network virtualization utilities, security tasks like firewall, and application-specific tasks like key-value store caching.
\noteyiying{any better examples?}
In this paper, we call all types of functionalities that process network packets {\em network task}s, or {\em \nt}s.
\textbf{\textit{What would it imply to disaggregate netowrk tasks?}}
%like \yiying{Yizhou, fill some good examples with refs here}. stacks that are used for processing various tasks related to network communication (what we call {\em network task}s or {\em \nt}s in this paper), such as 
 
Less intuitively but as effective, we believe that network disaggregation can bring real benefits, just as compute, memory, and storage disaggregation.
Disaggregating \nt{}s into a separate pool allows data center providers to build and manage them all at one place instead of at each endpoint. 
We can further {\em consolidate} \nt{}s by allowing an N-to-1 ratio of endpoints and network devices.
With consolidation, the total number of network devices can be reduced, decreasing capital cost and/or allowing a rack to host more endpoints.

\input{fig-topology}

A recent work from Google called Aquila~\cite{aquila} uses a single network device to consolidate NIC and switching functionalities for two end hosts.
This and previous multi-host-NICs~\cite{bluefield,ocp-nic,Intel-RedRockCanyon} represent the first step towards network disaggregation, by allowing one NIC to drive multiple ``NIC-less'' end hosts.
%As witnessed by the evolution of single-host NICs, the need to offload network functionalities and application-specific functionalities to a NIC quickly grows, which gave rise to (single-host) SmartNIC. Similarly, 
A recent multi-host SmartNIC, NVidia BlueField~\cite{bluefield}, adds the support for computation offloading on top of a regular multi-host NIC.
BlueField allows users to offload software computation and a limited set of fixed-logic hardware accelerators like IPSec, but the former has limited performance~\cite{XXX} and the latter supports limited functionalities.
%BlueField contains general-purpose cores and a small number of fixed-logic accelerators like IPSec. With this design, users can only benefit from software-offloading (with limited performance) or the few fixed-logic accelerators (with limited flexibility).
Beside these limitations, existing multi-host solutions have no or limited multi-tenancy support.
Moreover, these prior solutions only allow end hosts to use one (Smart)NIC instead of a pool of network devices.
%, lacking the benefits of resource pooling.
%\notearvind{revisit and flesh this out more?}\noteyiying{I added more.}
%At first glance, ``network'' cannot be disaggregated from either a traditional monolithic server or a disaggregated device (in this paper collectively called {\em endpoints}), as they both need to be attached to the network.        
%However, we observe that even though endpoints need basic connectivity, it is not necessary to run {\em network-related tasks} at the endpoints.
%These network tasks, or {\em \nt}s, include the transport layer and all high-level layers such as network virtualization, packet filtering and encryption, and application-specific functions.

This paper proposes a network disaggregation solution that addresses the limitations of existing works by adding three key features: \textbf{fully programmable and hardware-based network task acceleration, multi-tenancy support, and distributed network resource pooling}.  Specifically, we built a rack-level platform that consists of a pool of \textit{\textbf{SuperNIC}s} (or \textit{\snic}s for short), a new hardware-based programmable network device designed for network disaggregation and consolidation.
%why new hardware-based sNIC. functions like transport need high speed parallel processing, and software is too slow for that. however, traditional NIC hardware or hardware-based SmartNIC does not offer the autoscaling or fair sharing feature we need for consolidation.
An \snic\ consists of an ASIC for fixed systems logic, FPGA for executing \nt{}s, and software cores for executing the control plane.
Users can deploy a single \nt\ written for FPGA or a directed acyclic graph (DAG) execution plan of \nt{}s to \snic.
One \snic\ can directly connect to a handful of endpoints and sit in the middle between endpoints and the ToR switch to allow more endpoints in a rack as shown in Figure~\ref{fig-topology}(b). Alternatively, \snic{}s can be integrated into the ToR switch for tight packaging as in Figure~\ref{fig-topology}(c). They can also be densely connected with auxiliary switching functionalities to achieve ultra low latency as in Figure~\ref{fig-topology}(d).
This work focuses on architecture (b), as it can be directly deployed with today's ToR-based racks.
Architectures (c) and (d) are seeing their initial adoption in the industry~\cite{XXX,Aquila} but are not yet commercially available.
\noteyiying{This part is a bit long. Shall we move it to Sec3? But if we don't say anything about the architecture, then the later part of distributed in the intro may not make much sense}
%\noteyiying{Delete the switch-attached topology if need space}
%\noteyiying{Shall we mention a third architecture: replacing Aquila TiNs with sNICs and keep the Aquila toplogy}
%\snic{}s can further be connected among themselves to form a disaggregated network resource pool. 
%As this paper focuses on the low-level, single-\snic\ design, we only briefly discuss the potential of such a distributed platform (\S\ref{sec:discussion}).

\if 0
%\bolditpara{Proposal: disaggregated network resource pool.}
At the core of our network-disaggregation proposal is the concept of a rack-scale disaggregated {\em network resource pool}, which consists of a set of hardware devices that can execute \nt{}s and collectively provide ``network'' as a service (Figure~\ref{fig-topology}), similar to how today's disaggregated storage pool provides data storage service to compute nodes. 
Endpoints can offload (\ie, disaggregate) part or all of their \nt{}s to the network resource pool.
After \nt{}s are disaggregated, we further propose to {\em consolidate} them by aggregating a rack's endpoint \nt{}s onto a small set of network devices.
%\notearvind{might need to generalize to a network pool}
%, thereby reducing the total number of network .

Network disaggregation and consolidation have several key benefits.
(1) (2) Disaggregating \nt{}s into a separate pool allows the {\em independent scaling} of hardware resources used for network functionalities without the need to change endpoints.
(3) Each endpoint can use more network resources than what can traditionally fit in a single NIC. 
(4) %The final and important benefit comes from consolidation.
(5) The network pool only needs to provision hardware resources for the peak \textit{aggregated} bandwidth in a rack instead of each endpoint provisioning for its own peak, reducing the overall CapEx cost.

%Several industry products are already adopting similar architectures, \eg, multi-host NIC~\cite{bluefield} (for the first architecture) and NIC-enhanced programmable switches~\cite{arubacx10000} (for the second architecture).
%\note{I'm confused on why the ToR has to be a smart/programmable switch, not made clear in it's explanation in first half of paragraph}.
%Network disaggregation would be a new usage case of these architectures. However, it requires new features that no existing systems fully support.
Before these benefits can be exploited in a real data center, network disaggregation needs to first meet several goals, which no existing solutions fully support (see \S\ref{sec:related}).
\fi

Building a hardware-based smart disaggregated network pool in a multi-tenant environment brings several key challenges. 
%\bolditpara{Building: what are the key requirements of network disaggregation and consolidation?}
First, an \snic\ consolidates \nt{}s for multiple endpoints and can experience higher and more load spikes. Both \snic's control plane and data plane need to efficiently handle these spikes.
Second, the \nt{}s offloaded to \snic\ include not only traditional NIC functionalities but also transports and customized packet processing logic. Thus, \snic\ needs to handle more types of functionalities than traditional SmartNICs. Moreover, an application may need multiple \nt{}s to process packets in a chain or a DAG, adding the potential complexity that \snic\ needs to address.
Third, an \snic\ should efficiently use all hardware resources so as to minimize the capital and energy costs. This indicates the need for tight consolidation and resource sharing among multiple tenants.
Fourth, \snic\ needs to provide an isolated execution environment and fair sharing of hardware resources for different tenants.
Finally, network devices in a pool need to work together so that lightly loaded devices can handle traffic for other devices that are overloaded. This load balancing would allow each device to provision less hardware resources as long as the entire pool can handle the peak aggregated load of the rack.
\noteyiying{This part is a bit long. Shall we cut it altogether or somehow shorten it?}
To confront these challenges, we propose the following designs. \noteyiying{better to have some sentence here to summarize the high-level approach/idea}
%The aggregated load will also likely require many different \nt{}s, ranging from transports to application-specific functionalities. Moreover, after aggregating traffic, there are likely more load spikes (each coming from a different endpoint) that the device needs to handle.
%Second, using a disaggregated network pool should reduce the total cost of a cluster. This means that each disaggregated network device should provision the right amount of hardware resources (CapEx) and use as little of them as needed at run time (OpEx). At the same time, the remaining part of a rack (\eg, endpoints, ToR switch, cables) needs to be carefully designed to be low cost.
%Third, as we are consolidating \nt{}s from multiple endpoints, in a multi-tenant environment, there would be more entities that need to be isolated. We should ensure that they fairly and safely share various hardware resources in a disaggregated network pool. 
%
%Meeting these requirements together is not easy as they imply that the disaggregated network devices need to use minimal and properly isolated hardware resources to handle large loads with high variation, while achieving application performance as if there is no disaggregation.

To tightly \textbf{consolidate} \nt{}s within an \snic, we support three types of resource sharing: (1) splitting an \snic's hardware resources across different \nt{}s ({\em space sharing}), (2) allowing multiple applications to use the same \nt{} at different times ({\em time sharing}), and (3) configuring the same hardware resources to run different \nt{}s at different times ({\em time sharing with context switching}).
For space sharing, we partition the FPGA space into {\em region}s, with each hosting one or more \nt{}s.
Each region could be individually reconfigured %(via FPGA partial reconfiguration, or {\em PR}) 
for starting new \nt{}s or to context switch \nt{}s.
Different from traditional software systems, hardware context switching via FPGS partial reconfiguration, or {\em PR}, is orders of magnitude slower, which could potentially impact application performance significantly.
To solve this unique challenge, we propose a set of policies and mechanisms to reduce the need to perform PR or to move it off the performance-critical path. %, \eg, by keeping de-scheduled \nt{}s around like a traditional victim cache, by not over-reacting to load spikes, and by utilizing other \snic{}s when one \snic\ is overloaded.
%\notearvind{Might be worth saying that we also rely on other sNICs' resources if a local sNIC is overloaded.}

To achieve high \textbf{performance} under large, varying load with minimal cost, we automatically scale ({\em auto-scale}) an \nt{} by adding/removing instances of it and sending different flows in an application across these instances.
%\noteyiying{@Yizhou, do we send different flows to different instances or it's packet level? --- YS: We use flows. We cannot do individual packet LB, because there are states associated with each flow.}
We further launch different \nt{}s belonging to the same application in parallel and send forked packets to them in parallel for faster processing.
%We achieve high throughput using two levels of parallelism:
%{\em \nt{} parallelism} where a packet goes through multiple \nt{}s in parallel and {\em instance parallelism} where we launch multiple instances of the same \nt{} to handle different packets in an application.
%Apart from the above data-plane designs, we build a scalable control plane.
%To achieve low scheduling latency and scalability, we 
%propose a scheduler that centers around a new notion, {\em \nt\ chaining}.
%The idea is to 
To achieve low scheduling latency and improve scalability, we group \nt{}s that are likely to be executed in a sequence into a chain.
% and to have our central scheduler schedule packets only once for the entire chain. 
Our scheduler reserves credits for the entire chain as much as possible so that packets execute the chain as a whole without involving the scheduler in between.
%Doing so improves both packet-processing latency and scheduler scalability.

To provide \textbf{fairness}, we propose an algorithm that jointly considers fair space and fair time sharing, in an adaptive and fine-grained manner. 
The main idea is to decide space allocation of different resources like FPGA chip area and payload buffer space periodically based on Dominant Resource Fairness (DRF)~\cite{DRF}, guided by the monitored actual load demands (instead of the original DRF's static resource demand vector). Between these periods, we constantly~\noteyiying{Will, constantly or frequently?} run DRFQ~\cite{DRFQ} for fair time sharing of the current space allocation.
%adopt a fine-grained approach that treats each internal hardware resource separately, \eg, ingress/egress bandwidth, internal bandwidth of each shared \nt, payload buffer space, and on-board memory, as doing so allows a higher degree of consolidation.
%Our context is unique in that the packet processing system itself requires multi-dimensional resource sharing. 
%We adopt Dominant Resource Fairness (DRF)~\cite{DRF} for this multi-dimensional resource sharing.
%For the first time in networking systems, we consider multi-dimensional resource sharing and provide Dominant Resource Fairness (DRF)~\cite{DRF}. 
%Instead of user-supplied, static per-resource demands as in traditional DRF systems, we monitor the actual load demands at run time and use them as the target in the DRF algorithm.
When adjusting resource allocation, instead of throttling at each type of resource, we use ingress bandwidth throttling to control the allocation of most other types of resources.
We also build a simple virtual memory system to \textbf{isolate and protect} accesses to on-board memory. %All \nt's memory accesses use 

Finally, for \textbf{distributed \snic{}s}, we automatically scale out \nt{}s beyond a single \snic\ when load increases and balance loads across \snic{}s. %We use a de-centralized manner to let \snic{}s exchange load information and initiate load migration when one \snic\ is overloaded.
With this resource pooling, we can collectively provision the total network resource of a rack to be roughly the peak of the aggregated traffic in the rack, which is much lower than today's rack which needs each endpoint to provision for its own peak.
%depending on the network pool architectures.
%For example, with the switch-attached pool architecture, we use the ToR switch to balance all traffic across \snic{}s.
%With the intermediate pool architecture, we further support a peer-to-peer, \snic-initiated load migration when one \snic\ is overloaded.

\if 0
When one \snic\ is overloaded and needs to accommodate too much network bandwidth, on-chip hardware resources, or off-chip memory space, traditional solutions would drop packets/\nt{}s or provision more hardware resources. The former impacts application performance, and the latter results in resource wastage when loads are not at their peaks. 
Our idea is to utilize other \snic{}s to handle load spikes, based on the observation that not all \snic{}s under a rack would run at their peak load at the same time. Essentially, with distributed \snic{}s, we provision for the maximum aggregated bandwidth in a rack instead of the sum of peak loads under each \snic.
Specifically, to support overloaded network bandwidth or on-chip hardware resources at an \snic, we create an \nt\ at another \snic\ that has a lighter load. 
The current \snic\ then only serves as a simple pass-through device to redirect packets to the new \snic.
%, with the latter sending packets to the next hop after processing them.
To support overloaded memory space at an \snic, our virtual memory system transparently swaps memory to/from an \snic{} with less memory pressure.
\fi

\input{fig-osdi16-net-trace}


We prototype \snic\ with FPGA using two 100\Gbps, multi-port HiTech Global HTG-9200 boards~\cite{htg9200}.
%The data plane runs on FPGA directly, while the control plane runs in software cores deployed on FPGA.
We build three types of \nt{}s to run on \snic:
reliable transport, traditional network functions, and application-specific tasks. We port two end-to-end use cases to \snic.
The first use case is a key-value store we built on top of real disaggregated memory devices~\cite{Clio}.
We explore using \snic{}s for traditional \nt{}s like the transport layer and customized \nt{}s like key-value data replication and caching.
%For the latter, the client only needs to send one copy to the \snic, which will send copies of the data to multiple memory devices.
%customized network abstraction for disaggregated memory device: a key-value store interface (rather than the standard messaging interface).
%Furthermore, we 
The second use case is a Virtual Private Cloud application we built on top of regular servers by connecting \snic{}s at both the sender and the receiver side.
We disaggregate \nt{}s like encapsulation, firewall, and encryption to the \snic{}s.
%a go-back-N reliable transport; a set of network functions including firewall, AES encryption, and VPN Gateway; and a set of application-specific functions including key-value store replication and caching.
We evaluate \snic\ and the ported applications with micro- and macro-benchmarks and compare \snic\ with no network disaggregation and disaggregation using alternative solutions such as multi-host NICs and a recent multi-tenant, single-host SmartNIC~\cite{panic-osdi20}.
Overall, \snic\ achieves 52\% to 56\% CapEx and OpEx cost savings with only 4\% performance overhead compared to a traditional non-disaggregated per-endpoint SmartNIC scenario.
%Our results running a Facebook key-value trace~\cite{Atikoglu12-SIGMETRICS} show that \snic's consolidation of four endhosts and two \nt{}s saves 64\% costs compared to no consolidation, with only 1.3\% performance overhead.
Furthermore, the customized key-value store caching and replication functionalities on \snic\ improves throughput by 1.31\x\ to 3.88\x\ and latency by 1.21\x\ to 1.37\x\ when compared to today's remote memory systems with no \snic.
%We will open source \snic\ upon the publication of this paper.





\if 0
There is a trend in disaggregating datacenters,
in which monolithic servers are segregated into cpu, memory, disk
resource pools and connected to the network directly.
Disaggregation makes it easy to manage and scale each resource pool independently.
While increasing amount of effort go into disaggregating compute,
memory, and storage, the fourth major resource in datacenter, network,
has been completely left out. No work has attempted to disaggregate the network.
At first glance, network cannot be disaggregated from either
a traditional monolithic server or a disaggregated device, as
they both need to be attached to the network
and each endpoint is provisioned with its own network interface (i.e., NIC)
and the associated network stack. This raises the question:

\textit{Should we and how can we disaggregate the network?}

We answer this question in the affirmative:
we should disaggregate and then consolidate the network.
In our preliminary study,
we find both regular server and disaggregated clusters have bursty network traffic
while the networking resource is highly under-utilized.
The root cause is that network is tightly coupled with
other resources (e.g., compute or memory) and hence,
making it impossible to
provision the right amount of networking resource for individual endpoints.
Similar to traditional disaggregation,
if we can disaggregate the networking resource and further
aggregate them into a network resource pool,
it could enjoy easier management, scaling, and resource packing.
We envision this is applicable and beneficial
for two types of endpoints: regular monolithic servers
and disaggregated devices.

We propose to \textit{disaggregate} network functionalities
from individual endpoints in a rack
and \textit{consolidate} them into a \textbf{\textit{network resource pool}}.
%
Crucially, the consolidation enables statistical multiplexing of resources that
allows us to move away from provisioning for peak utilization
on a per-node basis to provisioning for the
expected peak utilization for a cluster of nodes.
Also, consolidating network functionalities into a separate
pool makes it easy for datacenter operators to manage them.
%
Three types of network functionalities are moved:
\textit{1)} packet processing logic in NIC hardware,
\textit{2)} software network stacking running at host CPU,
and \textit{3)} advanced application-specific network functions.
%
As a result, individual endpoints no longer need to provision
hardware and software resources for networking,
they can directly use services exposed by the network resource pool.
%
In other words, the network resource pool essentially provides
\textbf{\textit{network-as-a-service}} to the rest of the datacenter.


Network disaggregation and consolidation presents several new challenges.
%
First, network has always been an integral part for any computer systems design.
Hence, it is challenging to extract the network functions
while ensuring correctness and performance.
%
Second, a key question is how to implement the network resource pool.
In order to meet the goals of disaggregation,
the pool must be flexible, power-efficient, high-performance, easy to manage, and secure.
Disaggregated datacenter poses several unique challenges
like the exploded number of network ports and the mix of heterogeneous devices
\fi



\if 0
In this paper, we will focus on the second challenge.
We take a detailed survey on all emerging network devices
and evaluate whether they are qualified to make the network resource pool.
In specific, we review
\textit{programmable switch}~\cite{netcache-sosp17,incbricks-asplos17,distcache-fast19,pegasus-osdi20,hpcc-sigcomm19,netlock-sigcomm20,cheetah-sigmod20,racksched-osdi20,tea-sigcomm20},
\textit{circuit switch}~\cite{helios-sigcomm10,mordia-sigcomm13,reactor-nsdi14,rotornet-sigcomm17,sirius-sigcomm20,dRedBox-DATE,shoal-nsdi19},
\textit{coherent fabrics}~\cite{GenZ,OpenCAPI,CCIX,CXL},
\textit{middleboxes}~\cite{walfish-osdi04,comb-nsdi12,aplomb-sigcomm20},
\textit{NFV}~\cite{clickos-nsdi14,e2,netbricks,resq-nsdi18,metron-nsdi18,flowblaze-nsdi19,panic-osdi20,azure-nsdi18},
and \textit{multi-host NICs}~\cite{Intel-RedRockCanyon,Mellanox-Multihost}.

After a rigorous examination, we find none of them meets all our goals.
In response, we propose \sysname, a new network device specifically
designed for network disaggregation and consolidation.
A set of SuperNICs make a disaggregated network resource pool,
which sits in between endpoints and a ToR switch.
All the SuperNICs are connected together through a ring or a torus (see Figure~\ref{fig-topology}).
We expect it to have high performance, flexible abstractions,
safe and efficient consolidation, adaptive scaling, and failure handling.


Overall, our contributions are:
\begin{itemize}
\vspace{-0.05in}
\item To the best of our knowledge, we are the first to
disaggregate and consolidate network in datacenters.
\vspace{-0.05in}
\item We review various emerging networking devices.
\vspace{-0.05in}
\item We propose SuperNIC, a new device specifically tailored for network disaggregation and consolidation.
\end{itemize}

\fi



==> latexdiff-so <==
#!/usr/bin/perl -w
# latexdiff - differences two latex files on the word level
#             and produces a latex file with the differences marked up.
#
#   Copyright (C) 2004-2007  F J Tilmann (tilmann@esc.cam.ac.uk)
#
#    This program is free software; you can redistribute it and/or modify
#    it under the terms of the GNU General Public License Version 2 as published by
#    the Free Software Foundation.
#
#    This program is distributed in the hope that it will be useful,
#    but WITHOUT ANY WARRANTY; without even the implied warranty of
#    MERCHANTABILITY or FITNESS FOR A PARTICULAR PURPOSE.  See the
#    GNU General Public License for more details.
#
#    You should have received a copy of the GNU General Public License
#    along with this program; if not, write to the Free Software
#    Foundation, Inc., 59 Temple Place, Suite 330, Boston, MA  02111-1307  USA
#
# Detailed usage information at the end of the file
#
# Version 0.5  A number of minor improvements based on feedback
#              Deleted blocks are now shown before added blocks
#              Package specific processing
#
# Version 0.43 unreleased typo in list of styles at the end
#              Add protect to all \cbstart, \cbend commands
#              More robust substitution of deleted math commands
#
# Version 0.42 November 06  Bug fixes only
#
# Version 0.4   March 06 option for fast differencing using UNIX diff command, several minor bug fixes (\par bug, improved highlighting of textcmds)
#
# Version 0.3   August 05 improved parsing of displayed math, --allow-spaces 
#               option, several minor bug fixes
#
# Version 0.25  October 04 Fix bug with deleted equations, add math mode commands to safecmd, add | to allowed interpunctuation signs
# Version 0.2   September 04 extension to utf-8 and variable encodings
# Version 0.1   August 04    First public release

# Inserted block for stand-alone version replaces
# use Algorithm::Diff qw(traverse_sequences);
# in standard version
# The following BEGIN block contains a verbatim copy of
# Ned Konz' Algorithm::Diff package version 1.15 except
# that all POD documentation has been stripped out.
# I encourage you to download and install the Algorithm::Diff
# package and use the standard latexdiff version instead
# (current distribution available from http://search.cpan.org/~nedkonz/Algorithm-Diff-1.15
#  the most recent version can be found via  http://search.cpan.org/search?module=Algorithm::Diff )
# Please note that the LICENCSE for Algorithm::Diff :
#   "Copyright (c) 2000-2002 Ned Konz.  All rights reserved.
#    This program is free software;
#    you can redistribute it and/or modify it under the same terms
#    as Perl itself."
# The stand-alone version of latexdiff is provided as a convenience
# for latex users with no knowledge of PERL who do not wish to install
# additional packages to be able to use latexdiff.  If you believe
# the inlining of Algorithm::Diff violates its license please contact
# me and I will modify the latexdiff distribution accordingly.
# Frederik Tilmann (tilmann@esc.cam.ac.uk)
BEGIN { 
package Algorithm::Diff;
use strict;
use vars qw($VERSION @EXPORT_OK @ISA @EXPORT);
use integer;    # see below in _replaceNextLargerWith() for mod to make
                # if you don't use this
require Exporter;
@ISA       = qw(Exporter);
@EXPORT    = qw();
@EXPORT_OK = qw(LCS diff traverse_sequences traverse_balanced sdiff);
$VERSION = sprintf('%d.%02d so', (q$Revision: 1.15 $ =~ /\d+/g));

# McIlroy-Hunt diff algorithm
# Adapted from the Smalltalk code of Mario I. Wolczko, <mario@wolczko.com>
# by Ned Konz, perl@bike-nomad.com


# Create a hash that maps each element of $aCollection to the set of positions
# it occupies in $aCollection, restricted to the elements within the range of
# indexes specified by $start and $end.
# The fourth parameter is a subroutine reference that will be called to
# generate a string to use as a key.
# Additional parameters, if any, will be passed to this subroutine.
#
# my $hashRef = _withPositionsOfInInterval( \@array, $start, $end, $keyGen );

sub _withPositionsOfInInterval
{
	my $aCollection = shift;    # array ref
	my $start       = shift;
	my $end         = shift;
	my $keyGen      = shift;
	my %d;
	my $index;
	for ( $index = $start ; $index <= $end ; $index++ )
	{
		my $element = $aCollection->[$index];
		my $key = &$keyGen( $element, @_ );
		if ( exists( $d{$key} ) )
		{
			unshift ( @{ $d{$key} }, $index );
		}
		else
		{
			$d{$key} = [$index];
		}
	}
	return wantarray ? %d : \%d;
}

# Find the place at which aValue would normally be inserted into the array. If
# that place is already occupied by aValue, do nothing, and return undef. If
# the place does not exist (i.e., it is off the end of the array), add it to
# the end, otherwise replace the element at that point with aValue.
# It is assumed that the array's values are numeric.
# This is where the bulk (75%) of the time is spent in this module, so try to
# make it fast!

sub _replaceNextLargerWith
{
	my ( $array, $aValue, $high ) = @_;
	$high ||= $#$array;

	# off the end?
	if ( $high == -1 || $aValue > $array->[-1] )
	{
		push ( @$array, $aValue );
		return $high + 1;
	}

	# binary search for insertion point...
	my $low = 0;
	my $index;
	my $found;
	while ( $low <= $high )
	{
		$index = ( $high + $low ) / 2;

		#		$index = int(( $high + $low ) / 2);		# without 'use integer'
		$found = $array->[$index];

		if ( $aValue == $found )
		{
			return undef;
		}
		elsif ( $aValue > $found )
		{
			$low = $index + 1;
		}
		else
		{
			$high = $index - 1;
		}
	}

	# now insertion point is in $low.
	$array->[$low] = $aValue;    # overwrite next larger
	return $low;
}

# This method computes the longest common subsequence in $a and $b.

# Result is array or ref, whose contents is such that
# 	$a->[ $i ] == $b->[ $result[ $i ] ]
# foreach $i in ( 0 .. $#result ) if $result[ $i ] is defined.

# An additional argument may be passed; this is a hash or key generating
# function that should return a string that uniquely identifies the given
# element.  It should be the case that if the key is the same, the elements
# will compare the same. If this parameter is undef or missing, the key
# will be the element as a string.

# By default, comparisons will use "eq" and elements will be turned into keys
# using the default stringizing operator '""'.

# Additional parameters, if any, will be passed to the key generation routine.

sub _longestCommonSubsequence
{
	my $a      = shift;    # array ref
	my $b      = shift;    # array ref
	my $keyGen = shift;    # code ref
	my $compare;           # code ref

	# set up code refs
	# Note that these are optimized.
	if ( !defined($keyGen) )    # optimize for strings
	{
		$keyGen = sub { $_[0] };
		$compare = sub { my ( $a, $b ) = @_; $a eq $b };
	}
	else
	{
		$compare = sub {
			my $a = shift;
			my $b = shift;
			&$keyGen( $a, @_ ) eq &$keyGen( $b, @_ );
		};
	}

	my ( $aStart, $aFinish, $bStart, $bFinish, $matchVector ) =
	  ( 0, $#$a, 0, $#$b, [] );

	# First we prune off any common elements at the beginning
	while ( $aStart <= $aFinish
		and $bStart <= $bFinish
		and &$compare( $a->[$aStart], $b->[$bStart], @_ ) )
	{
		$matchVector->[ $aStart++ ] = $bStart++;
	}

	# now the end
	while ( $aStart <= $aFinish
		and $bStart <= $bFinish
		and &$compare( $a->[$aFinish], $b->[$bFinish], @_ ) )
	{
		$matchVector->[ $aFinish-- ] = $bFinish--;
	}

	# Now compute the equivalence classes of positions of elements
	my $bMatches =
	  _withPositionsOfInInterval( $b, $bStart, $bFinish, $keyGen, @_ );
	my $thresh = [];
	my $links  = [];

	my ( $i, $ai, $j, $k );
	for ( $i = $aStart ; $i <= $aFinish ; $i++ )
	{
		$ai = &$keyGen( $a->[$i], @_ );
		if ( exists( $bMatches->{$ai} ) )
		{
			$k = 0;
			for $j ( @{ $bMatches->{$ai} } )
			{

				# optimization: most of the time this will be true
				if ( $k and $thresh->[$k] > $j and $thresh->[ $k - 1 ] < $j )
				{
					$thresh->[$k] = $j;
				}
				else
				{
					$k = _replaceNextLargerWith( $thresh, $j, $k );
				}

				# oddly, it's faster to always test this (CPU cache?).
				if ( defined($k) )
				{
					$links->[$k] =
					  [ ( $k ? $links->[ $k - 1 ] : undef ), $i, $j ];
				}
			}
		}
	}

	if (@$thresh)
	{
		for ( my $link = $links->[$#$thresh] ; $link ; $link = $link->[0] )
		{
			$matchVector->[ $link->[1] ] = $link->[2];
		}
	}

	return wantarray ? @$matchVector : $matchVector;
}

sub traverse_sequences
{
	my $a                 = shift;                                  # array ref
	my $b                 = shift;                                  # array ref
	my $callbacks         = shift || {};
	my $keyGen            = shift;
	my $matchCallback     = $callbacks->{'MATCH'} || sub { };
	my $discardACallback  = $callbacks->{'DISCARD_A'} || sub { };
	my $finishedACallback = $callbacks->{'A_FINISHED'};
	my $discardBCallback  = $callbacks->{'DISCARD_B'} || sub { };
	my $finishedBCallback = $callbacks->{'B_FINISHED'};
	my $matchVector = _longestCommonSubsequence( $a, $b, $keyGen, @_ );

	# Process all the lines in @$matchVector
	my $lastA = $#$a;
	my $lastB = $#$b;
	my $bi    = 0;
	my $ai;

	for ( $ai = 0 ; $ai <= $#$matchVector ; $ai++ )
	{
		my $bLine = $matchVector->[$ai];
		if ( defined($bLine) )    # matched
		{
			&$discardBCallback( $ai, $bi++, @_ ) while $bi < $bLine;
			&$matchCallback( $ai,    $bi++, @_ );
		}
		else
		{
			&$discardACallback( $ai, $bi, @_ );
		}
	}

	# The last entry (if any) processed was a match.
	# $ai and $bi point just past the last matching lines in their sequences.

	while ( $ai <= $lastA or $bi <= $lastB )
	{

		# last A?
		if ( $ai == $lastA + 1 and $bi <= $lastB )
		{
			if ( defined($finishedACallback) )
			{
				&$finishedACallback( $lastA, @_ );
				$finishedACallback = undef;
			}
			else
			{
				&$discardBCallback( $ai, $bi++, @_ ) while $bi <= $lastB;
			}
		}

		# last B?
		if ( $bi == $lastB + 1 and $ai <= $lastA )
		{
			if ( defined($finishedBCallback) )
			{
				&$finishedBCallback( $lastB, @_ );
				$finishedBCallback = undef;
			}
			else
			{
				&$discardACallback( $ai++, $bi, @_ ) while $ai <= $lastA;
			}
		}

		&$discardACallback( $ai++, $bi, @_ ) if $ai <= $lastA;
		&$discardBCallback( $ai, $bi++, @_ ) if $bi <= $lastB;
	}

	return 1;
}

sub traverse_balanced
{
	my $a                 = shift;                                  # array ref
	my $b                 = shift;                                  # array ref
	my $callbacks         = shift || {};
	my $keyGen            = shift;
	my $matchCallback     = $callbacks->{'MATCH'} || sub { };
	my $discardACallback  = $callbacks->{'DISCARD_A'} || sub { };
	my $discardBCallback  = $callbacks->{'DISCARD_B'} || sub { };
	my $changeCallback    = $callbacks->{'CHANGE'};
	my $matchVector = _longestCommonSubsequence( $a, $b, $keyGen, @_ );

	# Process all the lines in match vector
	my $lastA = $#$a;
	my $lastB = $#$b;
	my $bi    = 0;
	my $ai    = 0;
	my $ma    = -1;
	my $mb;

	while (1)
	{

		# Find next match indices $ma and $mb
		do { $ma++ } while ( $ma <= $#$matchVector && !defined $matchVector->[$ma] );

		last if $ma > $#$matchVector;    # end of matchVector?
		$mb = $matchVector->[$ma];

		# Proceed with discard a/b or change events until
		# next match
		while ( $ai < $ma || $bi < $mb )
		{

			if ( $ai < $ma && $bi < $mb )
			{

				# Change
				if ( defined $changeCallback )
				{
					&$changeCallback( $ai++, $bi++, @_ );
				}
				else
				{
					&$discardACallback( $ai++, $bi, @_ );
					&$discardBCallback( $ai, $bi++, @_ );
				}
			}
			elsif ( $ai < $ma )
			{
				&$discardACallback( $ai++, $bi, @_ );
			}
			else
			{

				# $bi < $mb
				&$discardBCallback( $ai, $bi++, @_ );
			}
		}

		# Match
		&$matchCallback( $ai++, $bi++, @_ );
	}

	while ( $ai <= $lastA || $bi <= $lastB )
	{
		if ( $ai <= $lastA && $bi <= $lastB )
		{

			# Change
			if ( defined $changeCallback )
			{
				&$changeCallback( $ai++, $bi++, @_ );
			}
			else
			{
				&$discardACallback( $ai++, $bi, @_ );
				&$discardBCallback( $ai, $bi++, @_ );
			}
		}
		elsif ( $ai <= $lastA )
		{
			&$discardACallback( $ai++, $bi, @_ );
		}
		else
		{

			# $bi <= $lastB
			&$discardBCallback( $ai, $bi++, @_ );
		}
	}

	return 1;
}

sub LCS
{
	my $a = shift;                                           # array ref
	my $matchVector = _longestCommonSubsequence( $a, @_ );
	my @retval;
	my $i;
	for ( $i = 0 ; $i <= $#$matchVector ; $i++ )
	{
		if ( defined( $matchVector->[$i] ) )
		{
			push ( @retval, $a->[$i] );
		}
	}
	return wantarray ? @retval : \@retval;
}

sub diff
{
	my $a      = shift;    # array ref
	my $b      = shift;    # array ref
	my $retval = [];
	my $hunk   = [];
	my $discard = sub { push ( @$hunk, [ '-', $_[0], $a->[ $_[0] ] ] ) };
	my $add = sub { push ( @$hunk, [ '+', $_[1], $b->[ $_[1] ] ] ) };
	my $match = sub { push ( @$retval, $hunk ) if scalar(@$hunk); $hunk = [] };
	traverse_sequences( $a, $b,
		{ MATCH => $match, DISCARD_A => $discard, DISCARD_B => $add }, @_ );
	&$match();
	return wantarray ? @$retval : $retval;
}

sub sdiff
{
	my $a      = shift;    # array ref
	my $b      = shift;    # array ref
	my $retval = [];
	my $discard = sub { push ( @$retval, [ '-', $a->[ $_[0] ], "" ] ) };
	my $add = sub { push ( @$retval, [ '+', "", $b->[ $_[1] ] ] ) };
	my $change = sub {
		push ( @$retval, [ 'c', $a->[ $_[0] ], $b->[ $_[1] ] ] );
	};
	my $match = sub {
		push ( @$retval, [ 'u', $a->[ $_[0] ], $b->[ $_[1] ] ] );
	};
	traverse_balanced(
		$a,
		$b,
		{
			MATCH     => $match,
			DISCARD_A => $discard,
			DISCARD_B => $add,
			CHANGE    => $change,
		},
		@_
	);
	return wantarray ? @$retval : $retval;
}

1;
}
import Algorithm::Diff qw(traverse_sequences);
# End of inserted block for stand-alone version

use Getopt::Long ;
use strict ;
use utf8 ;

my ($algodiffversion)=split(/ /,$Algorithm::Diff::VERSION);


my ($versionstring)=<<EOF ;
This is LATEXDIFF 0.5  (Algorithm::Diff $Algorithm::Diff::VERSION)
  (c) 2004-2007 F J Tilmann
EOF

# Configuration variables: these have to be visible from the subroutines
my $MINWORDSBLOCK=3; # minimum number of tokens to form an independent block
                     # shorter identical blocks will be merged to the previous word
my $FLOATENV='(?:figure|table|plate)[\w\d*@]*' ;   # Environments in which FL variants of defined commands are used
my $PICTUREENV='(?:picture|DIFnomarkup)[\w\d*@]*' ;   # Environments in which all change markup is removed
my $MATHENV='(?:equation|displaymath|DOLLARDOLLAR)' ;           # Environments turning on display math mode (code also knows about \[ and \]
my $MATHREPL='displaymath';  # Environment introducing deleted maths blocks
my $MATHARRENV='(?:eqnarray|align|gather|multiline|flalign)[*]?' ;           # Environments turning on eqnarray math mode
my $MATHARRREPL='eqnarray*';  # Environment introducing deleted maths blocks
my $ARRENV='(?:array|[pbvBV]matrix)'; # Enviroments making arrays in math mode.  The underlining style does not cope well with those - as a result in-text math environments are surrounded by \mbox{ } if any of these commands is used in an inline math block
my $COUNTERCMD='(?:footnote|part|section|subsection|subsubsection|paragraph|subparagraph)';  # textcmds which are associated with a counter
                                        # If any of these commands occur in a deleted block
                                        # they will be succeeded by an \addtocounter{...}{-1}
                                        # for the associated counter such that the overall numbers
                                        # should be the same as in the new file

# Markup strings
# If at all possible, do not change these as parts of the program
# depend on the actual name (particularly post-processing)
# At the very least adapt subroutine postprocess to new tokens.
my $ADDMARKOPEN='\DIFaddbegin ';   # Token to mark begin of appended text
my $ADDMARKCLOSE='\DIFaddend ';   # Token to mark end of appended text
my $ADDOPEN='\DIFadd{';  # To mark begin of added text passage
my $ADDCLOSE='}';        # To mark end of added text passage
my $ADDCOMMENT='DIF > ';   # To mark added comment line
my $DELMARKOPEN='\DIFdelbegin ';   # Token to mark begin of deleted text
my $DELMARKCLOSE='\DIFdelend ';   # Token to mark end of deleted text
my $DELOPEN='\DIFdel{';  # To mark begin of deleted text passage
my $DELCLOSE='}';        # To mark end of deleted text passage
my $DELCMDOPEN='%DIFDELCMD < ';  # To mark begin of deleted commands (must begin with %, i.e., be a comment
my $DELCMDCLOSE="%%%\n";    # To mark end of deleted commands (must end with a new line)
my $AUXCMD='%DIFAUXCMD' ; #  follows auxiliary commands put in by latexdiff to make difference file legal
                          # auxiliary commands must be on a line of their own
my $DELCOMMENT='DIF < ';   # To mark deleted comment line


# main local variables:
my @TEXTCMDLIST=();  # array containing patterns of commands with text arguments
my @TEXTCMDEXCL=();  # array containing patterns of commands without text arguments (if a pattern
                     # matches both TEXTCMDLIST and TEXTCMDEXCL it is excluded)
my @CONTEXT1CMDLIST=();  # array containing patterns of commands with text arguments (subset of text commands),
                         # but which cause confusion if used out of context (e.g. \caption). 
                         # In deleted passages, the command will be disabled but its argument is marked up
                         # Otherwise they behave exactly like TEXTCMD's 
my @CONTEXT1CMDEXCL=();  # exclude list for above, but always empty
my @CONTEXT2CMDLIST=();  # array containing patterns of commands with text arguments, but which fail cause confusion
                         # if used out of context (e.g. \title). They and their arguments will be disabled in deleted
                         # passages
my @CONTEXT2CMDEXCL=();  # exclude list for above, but always empty

my @SAFECMDLIST=();  # array containing patterns of safe commands (which do not break when in the argument of DIFadd or DIFDEL)
my @SAFECMDEXCL=();

my ($i,$j,$l);
my ($old,$new);
my ($line);
my ($newpreamble,$oldpreamble);
my (@newpreamble,@oldpreamble,@diffpreamble,@diffbody);
my ($latexdiffpreamble);
my ($oldbody, $newbody, $diffbo);
my ($oldpost, $newpost);
my ($diffall);
# Option names
my ($type,$subtype,$floattype,$config,$preamblefile,$encoding,
    $showpreamble,$showsafe,$showtext,$showconfig,$showall,
    $replacesafe,$appendsafe,$excludesafe,
    $replacetext,$appendtext,$excludetext,
    $replacecontext1,$appendcontext1,
    $replacecontext2,$appendcontext2,
    $help,$verbose,$version,$ignorewarnings,$allowspaces,$flatten,$debug);
my (@configlist,
    @appendsafelist,@excludesafelist,
    @appendtextlist,@excludetextlist,
    @appendcontext1list,@appendcontext2list,
    @packagelist);
my ($assign,@config);
# Hash where keys corresponds to the names of  all included packages (including the documentclass as another package
# the optional arguments to the package are the values of the hash elements
my ($pkg,%packages);
# Defaults
$type='UNDERLINE';
$subtype='SAFE';
$floattype='FLOATSAFE';

$verbose=0;
$debug=1; 
# define character properties
sub IsNonAsciiPunct { return <<'END'    # Unicode punctuation but excluding ASCII punctuation
+utf8::IsPunct
-utf8::IsASCII
END
}
sub IsNonAsciiS { return <<'END'       # Unicode symbol but excluding ASCII
+utf8::IsS
-utf8::IsASCII
END
}



  my %verbhash;

Getopt::Long::Configure('bundling');
GetOptions('type|t=s' => \$type, 
	   'subtype|s=s' => \$subtype, 
	   'floattype|f=s' => \$floattype, 
	   'config|c=s' => \@configlist,
	   'preamble|p=s' => \$preamblefile,
	   'encoding|e=s' => \$encoding,
	   'exclude-safecmd|A=s' => \@excludesafelist,
	   'replace-safecmd=s' => \$replacesafe,
	   'append-safecmd|a=s' => \@appendsafelist,
	   'exclude-textcmd|X=s' => \@excludetextlist,
	   'replace-textcmd=s' => \$replacetext,
	   'append-textcmd|x=s' => \@appendtextlist,
	   'replace-context1cmd=s' => \$replacecontext1,
	   'append-context1cmd=s' => \@appendcontext1list,
	   'replace-context2cmd=s' => \$replacecontext2,
	   'append-context2cmd=s' => \@appendcontext2list,
	   'show-preamble' => \$showpreamble,
	   'show-safecmd' => \$showsafe,
	   'show-textcmd' => \$showtext,
	   'show-config' => \$showconfig,
	   'show-all' => \$showall,
           'packages=s' => \@packagelist,
	   'verbose|V' => \$verbose,
	   'ignore-warnings' => \$ignorewarnings,
	   'allow-spaces' => \$allowspaces,
	   'flatten' => \$flatten,
	   'version' => \$version,
	   'help|h|H' => \$help);

if ( $help ) {
  usage() ;
}


if ( $version ) {
  die $versionstring ; 
}

print STDERR $versionstring if $verbose; 

if (defined($showall)){
  $showpreamble=$showsafe=$showtext=$showconfig=1;
}

# setting extra preamble commands
if (defined($preamblefile)) {
  $latexdiffpreamble=join "\n",(extrapream($preamblefile),"");
} else {
  $latexdiffpreamble=join "\n",(extrapream($type,$subtype,$floattype),"");
}

# setting up @SAFECMDLIST and @SAFECMDEXCL
if (defined($replacesafe)) {
  init_regex_arr_ext(\@SAFECMDLIST,$replacesafe);
} else {
  init_regex_arr_data(\@SAFECMDLIST, "SAFE COMMANDS");
}
foreach $appendsafe ( @appendsafelist ) {
  init_regex_arr_ext(\@SAFECMDLIST, $appendsafe);
}
foreach $excludesafe ( @excludesafelist ) {
  init_regex_arr_ext(\@SAFECMDEXCL, $excludesafe);
}

# Special: treat all cite commands as safe except in UNDERLINE and FONTSTRIKE mode
# (there is a conflict between citation and ulem package, see
# package documentation)
if ( uc($type) ne "UNDERLINE" && uc($type) ne "FONTSTRIKE" && uc($type) ne "CULINECHBAR" ) {
  push (@SAFECMDLIST, qr/^cite.*$/);
}

# setting up @TEXTCMDLIST and @TEXTCMDEXCL
if (defined($replacetext)) {
  init_regex_arr_ext(\@TEXTCMDLIST,$replacetext);
} else {
  init_regex_arr_data(\@TEXTCMDLIST, "TEXT COMMANDS");
}
foreach $appendtext ( @appendtextlist ) {
  init_regex_arr_ext(\@TEXTCMDLIST, $appendtext);
}
foreach $excludetext ( @excludetextlist ) {
  init_regex_arr_ext(\@TEXTCMDEXCL, $excludetext);
}


# setting up @CONTEXT1CMDLIST ( @CONTEXT1CMDEXCL exist but is always empty )
if (defined($replacecontext1)) {
  init_regex_arr_ext(\@CONTEXT1CMDLIST,$replacecontext1);
} else {
  init_regex_arr_data(\@CONTEXT1CMDLIST, "CONTEXT1 COMMANDS");
}
foreach $appendcontext1 ( @appendcontext1list ) {
  init_regex_arr_ext(\@CONTEXT1CMDLIST, $appendcontext1);
}


# setting up @CONTEXT2CMDLIST ( @CONTEXT2CMDEXCL exist but is always empty )
if (defined($replacecontext2)) {
  init_regex_arr_ext(\@CONTEXT2CMDLIST,$replacecontext2);
} else {
  init_regex_arr_data(\@CONTEXT2CMDLIST, "CONTEXT2 COMMANDS");
}
foreach $appendcontext2 ( @appendcontext2list ) {
  init_regex_arr_ext(\@CONTEXT2CMDLIST, $appendcontext2);
}




# setting configuration variables
@config=();
foreach $config ( @configlist ) {
  if (-f $config ) {
    open(FILE,$config) or die ("Couldn't open configuration file $config: $!");
    while (<FILE>) {
      chomp;
      next if /^\s*#/ || /^\s*%/ || /^\s*$/ ;
      push (@config,$_);
    }
    close(FILE);
  }
  else {
#    foreach ( split(",",$config) ) {
#      push @config,$_;
#    }
     push @config,split(",",$config)
  }
}
foreach $assign ( @config ) {
  $assign=~ m/\s*(\w*)\s*=\s*(\S*)\s*$/ or die "Illegal assignment $assign in configuration list (must be variable=value)";  
  if ( $1 eq "MINWORDSBLOCK" ) { $MINWORDSBLOCK = $2; }
  elsif ( $1 eq "FLOATENV" ) { $FLOATENV = $2 ; }
  elsif ( $1 eq "PICTUREENV" ) { $PICTUREENV = $2 ; }
  elsif ( $1 eq "MATHENV" ) { $MATHENV = $2 ; }
  elsif ( $1 eq "MATHREPL" ) { $MATHREPL = $2 ; }
  elsif ( $1 eq "MATHARRENV" ) { $MATHARRENV = $2 ; }
  elsif ( $1 eq "MATHARRREPL" ) { $MATHARRREPL = $2 ; }
  elsif ( $1 eq "ARRENV" ) { $ARRENV = $2 ; }
  elsif ( $1 eq "COUNTERCMD" ) { $COUNTERCMD = $2 ; }
  else { die "Unknown variable $1 in assignment.";}
}


foreach $pkg ( @packagelist ) {
  map { $packages{$_}="" } split(/,/,$pkg) ;
}

if ($showpreamble) {
  print "\nPreamble commands:\n";
  print $latexdiffpreamble ;
}

if ($showsafe) {
  print "\nCommands safe within scope of $ADDOPEN $ADDCLOSE and $DELOPEN $DELCLOSE (unless excluded):\n";
  print_regex_arr(@SAFECMDLIST);
  print "\nCommands not safe within scope of $ADDOPEN $ADDCLOSE and $DELOPEN $DELCLOSE :\n";
  print_regex_arr(@SAFECMDEXCL);
}

if ($showtext) {
  print "\nCommands with last argument textual (unless excluded) and safe in every context:\n";
  print_regex_arr(@TEXTCMDLIST);
  print "\nContext1 commands (last argument textual, command will be disabled in deleted passages, last argument will be shown as plain text):\n";
  print_regex_arr(@CONTEXT1CMDLIST);
  print "\nContext2 commands (last argument textual, command ant its argument will be disabled in deleted passages):\n";
  print_regex_arr(@CONTEXT2CMDLIST);  
  print "\nExclude list of Commands with last argument not textual (overrides patterns above):\n";
  print_regex_arr(@TEXTCMDEXCL);
}

if ($showconfig) {
  print "Configuration variables:\n";
  print "MINWORDSBLOCK=$MINWORDSBLOCK\n";
  print "FLOATENV=$FLOATENV\n";
  print "PICTUREENV=$PICTUREENV\n";
  print "MATHENV=$MATHENV\n";
  print "MATHREPL=$MATHREPL\n";
  print "MATHARRENV=$MATHARRENV\n";
  print "MATHARRREPL=$MATHARRREPL\n";
  print "ARRENV=$ARRENV\n";
  print "COUNTERCMD=$COUNTERCMD\n";
}
if ($showconfig || $showtext || $showsafe || $showpreamble) {
  exit 0; }
if ( @ARGV != 2 ) { 
  print STDERR "2 and only 2 non-option arguments required.  Write latexdiff -h to get help\n";
  exit(2);
}

# Are extra spaces between command arguments permissible?
my $extraspace;
if ($allowspaces) {
  $extraspace='\s*'; 
} else {
  $extraspace='';
}

# append context lists to text lists (as text property is implied)
push @TEXTCMDLIST, @CONTEXT1CMDLIST;
push @TEXTCMDLIST, @CONTEXT2CMDLIST;


# Patterns. These are used by some of the subroutines, too
# I can only define them down here because value of extraspace depends on an option
  my $pat0 = '(?:[^{}]|\\\{|\\\})*';
  my $pat1 = '(?:[^{}]|\\\{|\\\}|\{'.$pat0.'\})*';
  my $pat2 = '(?:[^{}]|\\\{|\\\}|\{'.$pat1.'\})*'; # 
  my $pat3 = '(?:[^{}]|\\\{|\\\}|\{'.$pat2.'\})*';
  my $pat4 = '(?:[^{}]|\\\{|\\\}|\{'.$pat3.'\})*';
  my $brat0 = '(?:[^\[\]]|\\\[|\\\])*'; 

  my $quotemarks = '(?:\'\')|(?:\`\`)';
  my $punct='[0.,\/\'\`:;\"\?\(\)\[\]!~\p{IsNonAsciiPunct}\p{IsNonAsciiS}]';
  my $number='-?\d*\.\d*';
  my $mathpunct='[+=<>\-\|]';
  my $and = '&';
  my $coords= '[\-.,\s\d]*';
# word: sequence of letters or accents followed by letter
  my $word='(?:[-\w\d*]|\\\\[\"\'\`~^][A-Za-z\*])+';
  my $cmdleftright='\\\\(?:left|right)\s*(?:[()\[\]|]|\\\\(?:[|{}]|\w+))';

  my $cmdoptseq='\\\\[\w\d\*]+'.$extraspace.'(?:(?:\['.$brat0.'\]|\{'. $pat4 . '\}|\(' . $coords .'\))'.$extraspace.')*';
  my $oneletcmd='\\\\.(?:\['.$brat0.'\]|\{'. $pat4 . '\})*';
  my $math='\$(?:[^$]|\\\$)*?\$|\\\\[(].*?\\\\[)]';
#  my $math='\$(?:[^$]|\\\$)*\$';
  my $comment='%.*?\n';
  my $pat=qr/(?:\A\s*)?(?:${and}|${quotemarks}|${number}|${word}|$cmdleftright|${cmdoptseq}|${math}|${oneletcmd}|${comment}|${punct}|${mathpunct}|\{|\})\s*/ ;



# now we are done setting up and can start working   
my ($oldfile, $newfile) = @ARGV;

$encoding=guess_encoding($newfile) unless defined($encoding);

$encoding = "utf8" if $encoding =~ m/^utf8/i ;
if (lc($encoding) eq "utf8" ) {
  binmode(STDOUT, ":utf8");
  binmode(STDERR, ":utf8");
}

$old=read_file_with_encoding($oldfile,$encoding);
$new=read_file_with_encoding($newfile,$encoding);




# reset time
exetime(1);
($oldpreamble,$oldbody,$oldpost)=splitdoc($old,'\\\\begin\{document\}','\\\\end\{document\}');


($newpreamble,$newbody,$newpost)=splitdoc($new,'\\\\begin\{document\}','\\\\end\{document\}');


if ($flatten) {
  $oldbody=flatten($oldbody,$oldpreamble,$oldfile,$encoding);
  $newbody=flatten($newbody,$newpreamble,$newfile,$encoding);
}

if ( length $oldpreamble && length $newpreamble ) {
  @oldpreamble = split /\n/, $oldpreamble;
  @newpreamble = split /\n/, $newpreamble;
  
  %packages=list_packages(@newpreamble) unless %packages;
  if (defined $packages{"hyperref"} ) {
    print STDERR "hyperref package detected.\n" if $verbose ;
    $latexdiffpreamble =~ s/\{\\DIFadd\}/{\\DIFaddtex}/g;
    $latexdiffpreamble =~ s/\{\\DIFdel\}/{\\DIFdeltex}/g;
    $latexdiffpreamble .= join "\n",(extrapream("HYPERREF"),"");
  }
  # insert dummy first line such that line count begins with line 1 (rather than perl's line 0) - just so that line numbers inserted by linediff are correct
  unshift @newpreamble,'';
  unshift @oldpreamble,'';
  print STDERR "Differencing preamble.\n" if $verbose;
  @diffpreamble = linediff(\@oldpreamble, \@newpreamble);
  # remove dummy line again
  shift @diffpreamble; 
  push @diffpreamble,$latexdiffpreamble;
  push @diffpreamble,'\begin{document}';
}
elsif ( !length $oldpreamble && !length $newpreamble ) {
  @diffpreamble=();
} else {
  print STDERR "Either both texts must have preamble or neither text must have the preamble.\n";
  exit(2);
}

if (defined $packages{"amsmath"} ) {
  print STDERR "amsmath package detected.\n" if $verbose ;
  $MATHARRREPL='align*';
}

print STDERR "Preprocessing body.  " if $verbose;
my ($oldleadin,$newleadin)=preprocess($oldbody,$newbody);


# run difference algorithm
@diffbody=bodydiff($oldbody, $newbody);
$diffbo=join("",@diffbody);
print STDERR "(",exetime()," s)\n","Postprocessing body. \n " if $verbose;
postprocess($diffbo);
$diffall =join("\n",@diffpreamble) ;
$diffall .= "$newleadin$diffbo" ;
$diffall .= "\\end{document}$newpost" if length $newpreamble ;
if ( lc($encoding) ne "utf8" && lc($encoding) ne "ascii" ) {
  print STDERR "Encoding output file to $encoding\n" if $verbose;
  $diffall=Encode::encode($encoding,$diffall);
  binmode STDOUT;
}
print $diffall;


print STDERR "(",exetime()," s)\n","Done.\n" if $verbose;



## guess_encoding(filename)
## reads the first 20 lines of filename and looks for call of inputenc package
## if found, return the option of this package (encoding), otherwise return ascii
sub guess_encoding {
  my ($filename)=@_;
  my ($i,$enc);
  open (FH, $filename) or die("Couldn't open $filename: $!");
  $i=0;
  while (<FH>) {
    next if /^\s*%/;    # skip comment lines
    if (m/\\usepackage\[(\w*?)\]\{inputenc\}/) {
      close(FH);
      return($1);
    }
    last if (++$i > 20 ); # scan at most 20 non-comment lines
  }
  close(FH);
  return("ascii");
}


sub read_file_with_encoding {
  my ($output);
  my ($filename, $encoding) = @_;

  if (lc($encoding) eq "utf8" ) {
    open (FILE, "<:utf8",$filename) or die("Couldn't open $filename: $!");
    local $/ ; # locally set record operator to undefined, ie. enable whole-file mode
    $output=<FILE>;
  } elsif ( lc($encoding) eq "ascii") {
    open (FILE, $filename) or die("Couldn't open $filename: $!");
    local $/ ; # locally set record operator to undefined, ie. enable whole-file mode
    $output=<FILE>;
  } else {
    require Encode;
    open (FILE, "<",$filename) or die("Couldn't open $filename: $!");
    local $/ ; # locally set record operator to undefined, ie. enable whole-file mode
    $output=<FILE>;
    print STDERR "Converting $filename from $encoding to utf8\n" if $verbose;
    $output=Encode::decode($encoding,$output);
  }
  close FILE;
  return $output;
}

# %packages=list_packages(@preamble)
# scans the arguments for \documentclass and \usepackage statements and constructs a hash
# whose keys are the included packages, and whose values are the associated optional arguments
sub list_packages {
  my (@preamble)=@_;
  my %packages=();
  foreach $line ( @preamble ) {
    # get rid of comments
    $line=~s/(?<!\\)%.*$// ;
    if ( $line =~ m/\\(?:documentclass|usepackage)(?:\[(.+?)\])?\{(.*?)\}/ ) {
#      print STDERR "Found something: |$line|\n";
      if (defined($1)) {
	$packages{$2}=$1;
      } else {
	$packages{$2}="";
      }
    }
  }
  return (%packages);
}

# flatten($text,$preamble,$filename,$encoding)
# expands \input and \include commands within text
# premable is scanned for includeonly commands
# encoding is the encoding
sub flatten {
  my ($text,$preamble,$filename,$encoding)=@_;
  my ($includeonly,$dirname,$fname,$newpage,$replacement);
  require File::Basename ; 
  require File::Spec ; 
  $dirname = File::Basename::dirname($filename);

  if ( ($includeonly) = ($preamble =~ m/\\includeonly{(.*?)}/ ) ) {
    $includeonly =~ s/,/|/g;
  } else {
    $includeonly = '.*?';
  }

  print STDERR "DEBUG: includeonly $includeonly\n";

  $text=~s/\\input{(.*?)}|\\include{(${includeonly}(?:\.tex)?)}/{ 
	    $fname = $1 if defined($1)  ;
	    $fname = $2 if defined($2) ;       
            #      # add tex extension unless there is a three letter extension already 
            $fname .= ".tex" unless $fname =~ m|\.\w{3}|;
            print STDERR "Include file $fname\n" if $verbose;
            print STDERR "DEBUG looking for file ",File::Spec->catfile($dirname,$fname), "\n";
            # content of file becomes replacement value, add \newpage if the command was include
            $replacement=read_file_with_encoding(File::Spec->catfile($dirname,$fname), $encoding) or die
                "Couldn't find file ",File::Spec->catfile($dirname,$fname),": $!";
	    $newpage=(defined($2)? " \\newpage " : "") ;
	    "$newpage$replacement$newpage";
          }/exg;

  return($text);
}


# print_regex_arr(@arr)
# prints regex array without x-ism expansion put in by pearl to stdout
sub print_regex_arr {
  my $dumstring;
  $dumstring = join(" ",@_);     # PERL generates string (?-xism:^ref$) for quoted refex ^ref$
  $dumstring =~ s/\(\?-xism:\^(.*?)\$\)/$1/g;   # remove string and ^,$ marks before output
  print $dumstring,"\n";
}


# @lines=extrapream($type)
# reads line from appendix (end of file after __END__ token)
sub extrapream {
  my $type;
  my @retval=("%DIF PREAMBLE EXTENSION ADDED BY LATEXDIFF") ;
  my ($copy);

  while (@_) {
    $copy=0;
    $type=shift ;
    if ( -f $type ) {
      open (FILE,$type) or die "Cannot open preamble file $type: $!";
      print STDERR "Reading preamble file $type\n" if $verbose ;
      while (<FILE>) {
	chomp ;
	if ( $_ =~ m/%DIF PREAMBLE/ ) {
	  push (@retval,"$_"); 
	} else {
	  push (@retval,"$_ %DIF PREAMBLE"); 
	}
      }
    } 
    else {    # not (-f $type)
      $type=uc($type);   # upcase argument
      print STDERR "Preamble Internal Type $type\n" if $verbose;
      while (<DATA>) {
	if ( m/^%DIF $type/ ) {
	  $copy=1; }
	elsif ( m/^%DIF END $type/ ) {
	  last; }
	chomp;
	push (@retval,"$_ %DIF PREAMBLE") if $copy;
      }
      if ( $copy == 0 ) {
	print STDERR "\nPreamble style $type not implemented.\n";
        print STDERR "Write latexdiff -h to get help with available styles\n";
        exit(2);
      }
      seek DATA,0,0;    # rewind DATA handle to file begin
    }
  }
  push (@retval,"%DIF END PREAMBLE EXTENSION ADDED BY LATEXDIFF")  ;
  return @retval;
}


# ($part1,$part2,$part3)=splitdoc($text,$word1,$word2)
# splits $text into 3 parts at $word1 and $word2.
# if neither $word1 nor $word2 exist, $part1 and $part3 are empty, $part2 is $text
# If only $word1 or $word2 exist but not the other, output an error message.

# NB this version avoids $` and $' for performance reason although it only makes a tiny difference
# (in one test gain a tenth of a second for a 30s run)
sub splitdoc {
  my ($text,$word1,$word2)=@_;
  my ($part1,$part2,$part3)=("","","");
  my ($rest,$pos);

  if ( $text =~ m/(^[^%]*)($word1)/mg ) {
    $pos=pos $text;
    $part1=substr($text,0,$pos-length($2));
    $rest=substr($text,$pos);
    if ( $rest =~ m/(^[^%]*)($word2)/mg ) {
      $pos=pos $rest;
      $part2=substr($rest,0,$pos-length($2));
      $part3=substr($rest,$pos);
    } 
    else {
      die "$word1 and $word2 not in the correct order or not present as a pair." ;
    }
  } else {
    $part2=$text;
    die "$word2 present but not $word1." if ( $text =~ m/(^[^%]*)$word2/ms );
  }
  return ($part1,$part2,$part3);
}





# bodydiff($old,$new)
sub bodydiff {
  my ($oldwords, $newwords) = @_;
  my @retwords;

  print STDERR "(",exetime()," s)\n","Splitting into latex tokens \n" if $verbose;
  print STDERR "Parsing $oldfile \n" if $verbose;
  my @oldwords = splitlatex($oldwords);
  print STDERR "Parsing $newfile \n" if $verbose;
  my @newwords = splitlatex($newwords);
  my $token;

  print STDERR "(",exetime()," s)\n","Pass 1: Expanding text commands and merging isolated identities with changed blocks  " if $verbose;
  pass1(\@oldwords, \@newwords);


  print STDERR "(",exetime()," s)\n","Pass 2: inserting DIF tokens and mark up.  " if $verbose;

  @retwords=pass2(\@oldwords, \@newwords);

  return(@retwords);
}




# @words=splitlatex($string)
# split string according to latex rules
# Each element of words is either
# a word (including trailing spaces and punctuation)
# a latex command
sub splitlatex {
  my ($string) = @_ ;
  my @retval=($string =~ m/$pat/osg);  

  if (length($string) != length(join("",@retval))) {
    print STDERR "\nWARNING: Inconsistency in length of input string and parsed string:\n     This often indicates faulty or non-standard latex code.\n     In many cases you can ignore this and the following warning messages.\n Note that character numbers in the following are counted beginning after \\begin{document} and are only approximate." unless $ignorewarnings;
    print STDERR "DEBUG Original length ",length($string),"  Parsed length ",length(join("",@retval)),"\n" if $debug;
    print STDERR "DEBUG Input string:  |$string|\n" if (length($string)<500) && $debug;
    print STDERR "DEBUG Token parsing: |",join("+",@retval),"|\n" if (length($string)<500) && $debug ;
    @retval=();
    # slow way only do this if other m//sg method fails
    my $last = 0;
    while ( $string =~ m/$pat/osg ) {
      my $match=$&;
      if ($last + length $& != pos $string  ) {
	my $pos=pos($string);
	my $offset=30<$last ? 30 : $last;
	my $dum=substr($string,$last-$offset,$pos-$last+2*$offset);
	my $dum1=$dum;
	my $cnt=$#retval;
	my $i;
	$dum1 =~ s/\n/ /g;
	unless ($ignorewarnings) {
	  print STDERR "\n$dum1\n";
	  print STDERR " " x 30,"^" x ($pos-$last)," " x 30,"\n";
	  print STDERR "Missing characters near word " . (scalar @retval) . " character index: " . $last . "-" .  pos($string) . " Length: " . length($match) . " Match: |$match| (expected match marked above).\n";
	}
	  # put in missing characters `by hand'
	push (@retval, substr($dum,$offset,$pos-$last-length($match)));
#       Note: there seems to be a bug in substr with utf8 that made the following line output substr which were too long,
#             using dum instead appears to work
#	push (@retval, substr($string,$last, pos($string)-$last-length($match)));
      }
      push (@retval, $match);
      $last=pos $string;
    }

  }
  return @retval;
}


# pass1( \@seq1,\@seq2)
# Look for differences between seq1 and seq2.
# Where an common-subsequence block is flanked by deleted or appended blocks, 
# and is shorter than $MINWORDSBLOCK words it is appended
# to the last deleted or appended word.  If the block contains tokens other than words 
# or punctuation it is not merged.
# Deleted or appended block consisting of words and safe commands only are
# also merged, to prevent break-up in pass2 (after previous isolated words have been removed)
# If there are commands with textual arguments (e.g. \caption) both in corresponding 
# appended and deleted blocks split them such that the command and opening bracket 
# are one token, then the rest is split up following standard rules, and the closing 
# bracket is a separate token, ie. turn
# "\caption{This is a textual argument}" into 
# ("\caption{","This ","is ","a ","textual ","argument","}")
# No return value.  Destructively changes sequences
sub pass1 {
  my $seq1 = shift ;
  my $seq2 = shift ;

  my $len1 = scalar @$seq1;
  my $len2 = scalar @$seq2;
  my $wpat=qr/^(?:[a-zA-Z.,'`:;?()!]*)[\s~]*$/;   #'

  my ($last1,$last2)=(-1,-1) ;
  my $cnt=0;
  my $block=[];
  my $addblock=[];
  my $delblock=[];
  my $todo=[];
  my $instruction=[];
  my $i;
  my (@delmid,@addmid,@dummy);

  my ($addcmds,$delcmds,$matchindex);
  my ($addtextblocks,$deltextblocks);
  my ($addtokcnt,$deltokcnt,$mattokcnt)=(0,0,0);
  my ($addblkcnt,$delblkcnt,$matblkcnt)=(0,0,0);

  my $adddiscard = sub {
                      if ($cnt > 0 ) {
			$matblkcnt++;
			# just after an unchanged block 
#			print STDERR "Unchanged block $cnt, $last1,$last2 \n";
                        if ($cnt < $MINWORDSBLOCK 
			    && $cnt==scalar (
				     grep { /^$wpat/ || ( /^\\([\w\d\*]+)((?:\[$brat0\]|\{$pat4\})*)/o 
							   && iscmd($1,\@SAFECMDLIST,\@SAFECMDEXCL) 
							   && scalar(@dummy=split(" ",$2))<3 ) }
					     @$block) )  {
			  # merge identical blocks shorter than $MINWORDSBLOCK 
			  # and only containing ordinary words
			  # with preceding different word
			  # We cannot carry out this merging immediately as this
			  # would change the index numbers of seq1 and seq2 and confuse
			  # the algorithm, instead we store in @$todo where we have to merge
                          push(@$todo, [ $last1,$last2,$cnt,@$block ]);
			}
			$block = []; 
			$cnt=0; $last1=-1; $last2=-1;
		      }
		    };
  my $discard=sub { $deltokcnt++;
                    &$adddiscard; #($_[0],$_[1]);
		    push(@$delblock,[ $seq1->[$_[0]],$_[0] ]);
		    $last1=$_[0] };		      

  my $add =   sub { $addtokcnt++;
                    &$adddiscard; #($_[0],$_[1]);
		    push(@$addblock,[ $seq2->[$_[1]],$_[1] ]);
		    $last2=$_[1] };		      

  my $match = sub { $mattokcnt++;
                    if ($cnt==0) {   # first word of matching sequence after changed sequence or at beginning of word sequence
		      $deltextblocks = extracttextblocks($delblock); 
		      $delblkcnt++ if scalar @$delblock;
		      $addtextblocks = extracttextblocks($addblock);
		      $addblkcnt++ if scalar @$addblock;

		      $delcmds = extractcommands($delblock);
      		      $addcmds = extractcommands($addblock);
		      # keygen(third argument of _longestCommonSubsequence) implies to sort on command (0th elements of $addcmd elements)
		      # the calling format for longestCommonSubsequence has changed between versions of
		      # Algorithm::Diff so we need to check which one we are using
		      if ( $algodiffversion  > 1.15 ) {
			### Algorithm::Diff 1.19
			$matchindex=Algorithm::Diff::_longestCommonSubsequence($delcmds,$addcmds, 0, sub { $_[0]->[0] } );
		      } else {
			### Algorithm::Diff 1.15	
			$matchindex=Algorithm::Diff::_longestCommonSubsequence($delcmds,$addcmds, sub { $_[0]->[0] } );
		      }

		      for ($i=0 ; $i<=$#$matchindex ; $i++) {
			if (defined($matchindex->[$i])){
			  $j=$matchindex->[$i];
			  @delmid=splitlatex($delcmds->[$i][3]);
			  @addmid=splitlatex($addcmds->[$j][3]);
			  while (scalar(@$deltextblocks)  && $deltextblocks->[0][0]<$delcmds->[$i][1]) {
			    my ($index,$block,$cnt)=@{ shift(@$deltextblocks) };
			    push(@$todo, [$index,-1,$cnt,@$block]);
			  }
			  push(@$todo, [ $delcmds->[$i][1],-1,-1,$delcmds->[$i][2],@delmid,$delcmds->[$i][4]]);

			  while (scalar(@$addtextblocks) && $addtextblocks->[0][0]<$addcmds->[$j][1]) {
			    my ($index,$block,$cnt)=@{ shift(@$addtextblocks) };
			    push(@$todo, [-1,$index,$cnt,@$block]);
			  }
			  push(@$todo, [ -1,$addcmds->[$j][1],-1,$addcmds->[$j][2],@addmid,$addcmds->[$j][4]]);
			}
		      }
		      # mop up remaining textblocks
		      while (scalar(@$deltextblocks)) {
			my ($index,$block,$cnt)=@{ shift(@$deltextblocks) } ;
			push(@$todo, [$index,-1,$cnt,@$block]);
		      }
		      while (scalar(@$addtextblocks)) {
			my ($index,$block,$cnt)=@{ shift(@$addtextblocks) };
			push(@$todo, [-1,$index,$cnt,@$block]);
		      }
		      
		      $addblock=[];
		      $delblock=[];
		    }
		    push(@$block,$seq2->[$_[1]]);  
		    $cnt++  };

  my $keyfunc = sub { join("  ",split(" ",shift())) };

  traverse_sequences($seq1,$seq2, { MATCH=>$match, DISCARD_A=>$discard, DISCARD_B=>$add }, $keyfunc );


  # now carry out the merging/splitting.  Refer to elements relative from 
  # the end (with negative indices) as these offsets don't change before the instruction is executed
  # cnt>0: merged small unchanged groups with previous changed blocks
  # cnt==-1: split textual commands into components
  foreach $instruction ( @$todo) {
    ($last1,$last2,$cnt,@$block)=@$instruction ;
    if ($cnt>=0) {
      splice(@$seq1,$last1-$len1,1+$cnt,join("",$seq1->[$last1-$len1],@$block)) if $last1>=0;
      splice(@$seq2,$last2-$len2,1+$cnt,join("",$seq2->[$last2-$len2],@$block)) if $last2>=0;
    } else {
      splice(@$seq1,$last1-$len1,1,@$block) if $last1>=0;
      splice(@$seq2,$last2-$len2,1,@$block) if $last2>=0;
    }
  }

  if ($verbose) { 
    print STDERR "\n";
    print STDERR "  $mattokcnt matching  tokens in $matblkcnt blocks.\n";
    print STDERR "  $deltokcnt discarded tokens in $delblkcnt blocks.\n";
    print STDERR "  $addtokcnt appended  tokens in $addblkcnt blocks.\n";
  }
}


# extracttextblocks(\@blockindex)
# $blockindex has the following format 
# [ [ token1, index1 ], [token2, index2],.. ] 
# where index refers to the index in the original old or new word sequence 
# Returns: reference to an array of the form  
# [[ $index, $textblock, $cnt ], ..
# where $index index of block to be merged
#       $textblock contains all the words to be merged with the word at $index (but does not contain this word)
#       $cnt   is length of block
#
# requires: iscmd
#
sub extracttextblocks { 
  my $block=shift;
  my ($i,$token,$index);
  my $textblock=[];
  my $last=-1;
  my $wpat=qr/^(?:[a-zA-Z.,'`:;?()!]*)[\s~]*$/;  #'
  my $retval=[];

  for ($i=0;$i< scalar @$block;$i++) {
    ($token,$index)=@{ $block->[$i] };
    # store pure text blocks
    if ($token =~ /$wpat/ ||  ( $token =~/^\\([\w\d\*]+)((?:${extraspace}\[$brat0\]${extraspace}|${extraspace}\{$pat4\})*)/o 
				&& iscmd($1,\@SAFECMDLIST,\@SAFECMDEXCL) 
				&& !iscmd($1,\@TEXTCMDLIST,\@TEXTCMDEXCL))) {
      # we have text or a command which can be treated as text
      if ($last<0) {
	# new pure-text block
	$last=$index;
      } else {
	# add to pure-text block
	push(@$textblock, $token); 
      }
    } else {
      # it is not text
      if (scalar(@$textblock)) {
	push(@$retval,[ $last, $textblock, scalar(@$textblock) ]);
      }
      $textblock=[];
      $last=-1;
    }
  }
  # finish processing a possibly unfinished block before returning
  if (scalar(@$textblock)) {
    push(@$retval,[ $last, $textblock, scalar(@$textblock) ]);
  }
  return($retval)
}



# extractcommands( \@blockindex )
# $blockindex has the following format 
# [ [ token1, index1 ], [token2, index2],.. ] 
# where index refers to the index in the original old or new word sequence 
# Returns: reference to an array of the form  
# [ [ "\cmd1", index, "\cmd1[optarg]{arg1}{", "arg2" ,"} " ],.. 
# where index is just taken from input array 
# command must have a textual argument as last argument 
# 
# requires: iscmd 
# 
sub extractcommands { 
  my $block=shift;
  my ($i,$token,$index,$cmd,$open,$mid,$closing);
  my $retval=[];

  for ($i=0;$i< scalar @$block;$i++) {
    ($token,$index)=@{ $block->[$i] };
    # check if token is an alphanumeric command sequence with at least one non-optional argument
    # \cmd[...]{...}{last argument}  
    # Capturing in the following results in these associations
    # $1: \cmd[...]{...}{
    # $2: \cmd
    # $3: last argument
    # $4: }  + trailing spaces
    if ( ( $token =~ m/^(\\([\w\d\*]+)(?:${extraspace}\[$brat0\]|${extraspace}\{$pat4\})*${extraspace}\{)($pat4)(\}\s*)$/so )
	 && iscmd($2,\@TEXTCMDLIST,\@TEXTCMDEXCL) ) {
      #      push(@$retval,[ $2,$index,$1,$3,$4 ]);
      ($cmd,$open,$mid,$closing) = ($2,$1,$3,$4) ;
      $closing =~ s/\}/\\RIGHTBRACE/ ;
      push(@$retval,[ $cmd,$index,$open,$mid,$closing ]);
    }
  }
  return $retval;
}

# iscmd($cmd,\@regexarray,\@regexexcl) checks
# return 1 if $cmd matches any of the patterns in the 
# array $@regexarray, and none of the patterns in \@regexexcl, otherwise return 0
sub iscmd {
  my ($cmd,$regexar,$regexexcl)=@_;
  my ($ret)=0;
  foreach $pat ( @$regexar ) {
    if ( $cmd =~ m/^${pat}$/ ) {
      $ret=1 ; 
      last;
    }
  }
  return 0 unless $ret;
  foreach $pat ( @$regexexcl ) {
    return 0 if ( $cmd =~ m/^${pat}$/ );
  }
  return 1;
}


# pass2( \@seq1,\@seq2)
# Look for differences between seq1 and seq2.  
# Mark begin and end of deleted and appended sequences with tags $DELOPEN and $DELCLOSE
# and $ADDOPEN and $ADDCLOSE, respectively, however exclude { } & and all comands, unless
# they match an element of the whitelist (SAFECMD)
# For words in TEXTCMD but not in SAFECMD, enclose interior with $ADDOPEN and $ADDCLOSE brackets
# Deleted comment lines are marked with %DIF < 
# Added comment lines are marked with %DIF > 
sub pass2 {
  my $seq1 = shift ;
  my $seq2 = shift ;

  my ($addtokcnt,$deltokcnt,$mattokcnt)=(0,0,0);
  my ($addblkcnt,$delblkcnt,$matblkcnt)=(0,0,0);

  my $retval = [];
  my $delhunk   = [];
  my $addhunk   = [];

  my $discard = sub { $deltokcnt++;
                      push ( @$delhunk, $seq1->[$_[0]]) };

  my $add = sub { $addtokcnt++;
                  push ( @$addhunk, $seq2->[$_[1]]) };

  my $match = sub { $mattokcnt++;
		    if ( scalar @$delhunk ) {
                      $delblkcnt++;
		      # mark up changes, but comment out commands
                      push @$retval,marktags($DELMARKOPEN,$DELMARKCLOSE,$DELOPEN,$DELCLOSE,$DELCMDOPEN,$DELCMDCLOSE,$DELCOMMENT,$delhunk);
		      $delhunk = [];
		    }
                    if ( scalar @$addhunk ) {
                      $addblkcnt++;
                      # we mark up changes, but simply quote commands
                      push @$retval,marktags($ADDMARKOPEN,$ADDMARKCLOSE,$ADDOPEN,$ADDCLOSE,"","",$ADDCOMMENT,$addhunk);
		      $addhunk = [];
		    }
		    push(@$retval,$seq2->[$_[1]]) };
 
  my $keyfunc = sub { join("  ",split(" ",shift())) };

  traverse_sequences($seq1,$seq2, { MATCH=>$match, DISCARD_A=>$discard, DISCARD_B=>$add }, $keyfunc );
  # clear up unprocessed hunks
  push @$retval,marktags($DELMARKOPEN,$DELMARKCLOSE,$DELOPEN,$DELCLOSE,$DELCMDOPEN,$DELCMDCLOSE,$DELCOMMENT,$delhunk) if scalar @$delhunk;
  push @$retval,marktags($ADDMARKOPEN,$ADDMARKCLOSE,$ADDOPEN,$ADDCLOSE,"","",$ADDCOMMENT,$addhunk) if scalar @$addhunk;


  if ($verbose) { 
    print STDERR "\n";
    print STDERR "  $mattokcnt matching  tokens. \n";
    print STDERR "  $deltokcnt discarded tokens in $delblkcnt blocks.\n";
    print STDERR "  $addtokcnt appended  tokens in $addblkcnt blocks.\n";
  }

  return(@$retval);
}

# marktags($openmark,$closemark,$open,$close,$opencmd,$closecmd,$comment,\@block)
# returns ($openmark,$open,$block,$close,$closemark) if @block only contains no commands (except white-listed ones),
# braces, ampersands, or comments
# mark comments with $comment
# exclude all other exceptions from scope of open, close like this
# ($openmark, $open,...,$close, $opencomd,command, command,$closecmd, $open, ..., $close, $closemark)
# If $opencmd begins with "%" marktags assumes it is operating on a deleted block, otherwise on an added block
sub marktags {
  my ($openmark,$closemark,$open,$close,$opencmd,$closecmd,$comment,$block)=@_;
  my $word;
  my (@argtext);
  my $retval=[];
  my $noncomment=0;
  my $cmd=-1;    # -1 at beginning 0: last token written is a ordinary word 
                 # 1: last token written is a command
                # for keeping track whether we are just in a command sequence or in a word sequence
  my $cmdcomment= ($opencmd =~ m/^%/);  # Flag to indicate whether opencmd is a comment (i.e. if we intend to simply comment out changed commands)
  my ($command,$commandword,$closingbracket) ; # temporary variables needed below to remember sub-pattern matches

# split this block to flatten out sequences joined in pass1
  @$block=splitlatex(join "",@$block);
  foreach (@$block) {
    $word=$_; 
    if ( $word =~ s/^%/%$comment/ ) {
      # a comment
      if ($cmd==1) {
	push (@$retval,$closecmd) ;
	$cmd=-1;
      }
      push (@$retval,$word); 
      next;
    }
    if (! $noncomment) {
      push (@$retval,$openmark); 
      $noncomment=1;
    }
    # negative lookahead pattern (?!) in second clause is put in to avoid mathcing \( .. \) patterns
    if ( $word =~ /^[&{}\[\]]/ || ( $word =~ /^\\(?!\()([\w*@]*)/ && !iscmd($1,\@SAFECMDLIST,\@SAFECMDEXCL)) ) {
      # word is a command or other significant token (not in SAFECMDLIST)
	## same conditions as in subroutine extractcommand:
	# check if token is an alphanumeric command sequence with at least one non-optional argument
	# \cmd[...]{...}{last argument}  
	# Capturing in the following results in these associations
	# $1: \cmd[...]{...}{
	# $2: \cmd
	# $3: last argument
	# $4: }  + trailing spaces
	### pre-0.3    if ( ( $token =~ m/^(\\([\w\d\*]+)(?:\[$brat0\]|\{$pat4\})*\{)($pat4)(\}\s*)$/so )
      if ( ( $word =~ m/^(\\([\w\d\*]+)(?:${extraspace}\[$brat0\]|${extraspace}\{$pat4\})*${extraspace}\{)($pat4)(\}\s*)$/so )
	   && iscmd($2,\@TEXTCMDLIST,\@TEXTCMDEXCL)  && ( !$cmdcomment || !iscmd($2,\@CONTEXT2CMDLIST, \@CONTEXT2CMDEXCL) )  ) {	 
	# word is a text command - we mark up the interior of the word. But if we are in a deleted block ($cmdcomment=1) and
        # $2 (the command) is in context2, just treat it as an ordinary command (i.e. comment it open with $opencmd)
        # Because we do not want to disable this command
	# here we do not use $opencmd and $closecmd($opencmd is empty) 
	if ($cmd==1) {
	  push (@$retval,$closecmd) ;
	} elsif ($cmd==0) { 
	  push (@$retval,$close) ;
	}
        $command=$1; $commandword=$2; $closingbracket=$4;
	@argtext=splitlatex($3);   # split textual argument into tokens
	# and mark it up (but we do not need openmark and closemark)
        # insert command with initial arguments, marked-up final argument, and closing bracket
	if ( $cmdcomment && iscmd($commandword,\@CONTEXT1CMDLIST, \@CONTEXT1CMDEXCL) ) {
	  # context1cmd in a deleted environment; delete command itself but keep last argument, marked up
	  push (@$retval,$opencmd);
	  $command =~ s/\n/\n${opencmd}/sg ; # repeat opencmd at the beginning of each line
	  # argument, note that the additional comment character is included
          # to suppress linebreak after opening parentheses, which is important
          # for latexrevise
          push (@$retval,$command,"%\n{$AUXCMD\n",marktags("","",$open,$close,$opencmd,$closecmd,$comment,\@argtext),$closingbracket);
	} else {
	  # normal textcmd or context1cmd in an added block
	  push (@$retval,$command,marktags("","",$open,$close,$opencmd,$closecmd,$comment,\@argtext),$closingbracket);  
	}
	push (@$retval,$AUXCMD,"\n") if $cmdcomment ;
	$cmd=-1 ;
      } else {
	# ordinary command
	push (@$retval,$opencmd) if $cmd==-1 ;
	push (@$retval,$close,$opencmd) if $cmd==0 ;
	$word =~ s/\n/\n${opencmd}/sg if $cmdcomment ;   # if opencmd is a comment, repeat this at the beginning of every line
	push (@$retval,$word);
	$cmd=1;
      }
    } else {
      # just an ordinary word or word in SAFECMD
      push (@$retval,$open) if $cmd==-1 ;
      push (@$retval,$closecmd,$open) if $cmd==1 ;
      push (@$retval,$word);
      $cmd=0;
    }
  }
  push (@$retval,$close) if $cmd==0;
  push (@$retval,$closecmd) if $cmd==1;

  push (@$retval,$closemark) if ($noncomment);
  return @$retval;
}

# preprocess($string, ..)
# carry out the following pre-processing steps for all arguments:
# 1. Remove leading white-space
# 2. mark all first empty line (in block of several) with \PAR tokens
# 3. Convert all '\%' into '\PERCENTAGE ' to make parsing regular expressions easier
# 4. Convert all \verb|some verbatim text| commands (where | can be an arbitrary character)
#    into \verb{hash}
# 5. Convert \begin{verbatim} some verbatim text \end{verbatim} into \verbatim{hash}
# 6. Convert _n into \SUBSCRIPTNB{n} and _{nnn} into \SUBSCRIPT{nn}
# 7. Convert ^n into \SUPERSCRIPTNB{n} and ^{nnn} into \SUPERSCRIPT{nn}
# 8. a. Convert $$ $$ into \begin{DOLLARDOLLAR} \end{DOLLARDOLLAR}
#    b. Convert \[ \] into \begin{SQUAREBRACKET} \end{SQUAREBRACKET}

# 9. Add final token STOP to the very end.  This is put in because the algorithm works better if the last token is identical.  This is removed again in postprocessing.
#
# NB: step 6 and 7 is likely to  convert some "_" inappropriately, e.g. in file
#     names or labels but it does not matter because they are converted back in the postprocessing step
# Returns: leading white space removed in step 1
sub preprocess {
  my @leadin=() ;
  for (@_) { 
    s/^(\s*)//s;
    push(@leadin,$1);
    s/\n(\s*?)\n((?:\s*\n)*)/\n$1\\PAR\n$2/g ;
    s/(?<!\\)\\%/\\PERCENTAGE /g ;  # (?<! is negative lookbehind assertion to prevent \\% from being converted
    s/(\\verb\*?)(\S)(.*?)\2/"${1}{". tohash(\%verbhash,"${2}${3}${2}") ."}"/esg;
    s/\\begin\{(verbatim\*?)\}(.*?)\\end\{\1\}/"\\${1}{". tohash(\%verbhash,"${2}") . "}"/esg;
    # Convert _n or _\cmd into \SUBSCRIPTNB{n} or \SUBSCRIPTNB{\cmd} and _{nnn} into \SUBSCRIPT{nn}
    s/_([^{\\]|\\\w+)/\\SUBSCRIPTNB{$1}/g ;
    s/_{($pat4)}/\\SUBSCRIPT{$1}/g ;
    # Convert ^n into \SUPERSCRIPTNB{n} and ^{nnn} into \SUPERSCRIPT{nn}
    s/\^([^{\\]|\\\w+)/\\SUPERSCRIPTNB{$1}/g ;
    s/\^{($pat4)}/\\SUPERSCRIPT{$1}/g ;
    # Convert $$ $$ into \begin{DOLLARDOLLAR} \end{DOLLARDOLLAR}
    s/\$\$(.*?)\$\$/\\begin{DOLLARDOLLAR}$1\\end{DOLLARDOLLAR}/sg;
    # Convert \[ \] into \begin{SQUAREBRACKET} \end{SQUAREBRACKET}
    s/(?<!\\)\\\[/\\begin{SQUAREBRACKET}/sg;
    s/\\\]/\\end{SQUAREBRACKET}/sg;
    # add final token " STOP"
    $_ .= " STOP"
  }
  return(@leadin);
}

#hashstring=tohash(\%hash,$string)
# creates a hash value based on string and stores in %hash
sub tohash {
  my ($hash,$string)=@_;
  my (@arr,$val);
  my ($sum,$i)=(0,1);
  my ($hstr);

  @arr=unpack('c*',$string);

  foreach $val (@arr) {
    $sum += $i*$val;
    $i++;
  }
  $hstr= "$sum";
  if (defined($hash->{$hstr}) && $string ne $hash->{$hstr}) {
    warn "Repeated hash value for verbatim mode in spite of different content.";
    $hstr="-$hstr";
  }
  $hash->{$hstr}=$string;
  return($hstr);
}

#string=fromhash(\%hash,$fromstring)
# restores string value stored in hash
#string=fromhash(\%hash,$fromstring,$prependstring)
# additionally begins each line with prependstring
sub fromhash {
  my ($hash,$hstr)=($_[0],$_[1]);
  my $retstr=$hash->{$hstr};
  if ( $#_ >= 2) {
    $retstr =~ s/^/$_[2]/mg;
  }
  return $retstr;
}


# postprocess($string, ..)
# carry out the following post-processing steps for all arguments:
# * Remove STOP token from the end
# * Replace \RIGHTBRACE by }
# 1. Check all deleted blocks: 
#    a.where a deleted block contains a matching \begin and
#      \end environment (these will be disabled by a %DIFDELCMD statements), for selected environment enable enable
#      these commands again (such that for example displayed math in a deleted equation
#      is properly within math mode.  For math mode environments replace numbered equation
#      environments with their display only variety (so that equation numbers in new file and
#      diff file are identical).  Where the correct type of math environment cannot be determined
#      use a place holder MATHMODE
#    b.where one of the commands matching $COUNTERCMD is used as a DIFAUXCMD, add a statement
#      subtracting one from the respective counter to keep numbering consistent with new file
#    Replace all MATHMODE environment commands by the correct environment to achieve matching
#    pairs
#    c. If in-line math mode contains array environment, enclose the whole environment in \mbox'es
# 2. Remove DIFadd, DIFdel, DIFFaddbegin , ... from picture environments
# 3. Convert DIFadd, DIFdel, DIFFaddbegin , ... into FL varieties
#    within floats (currently recognised float environments: plate,table,figure
#    plus starred varieties).
# 4. Remove empty %DIFDELCMD < lines 
# 4. Convert \begin{SQUAREBRACKET} \end{SQUAREBRACKET} into \[ \]
#    Convert \begin{DOLLARDOLLAR} \end{DOLLARDOLLAR} into $$ $$
# 5. Convert  \SUPERSCRIPTNB{n} into ^n  and  \SUPERSCRIPT{nn} into ^{nnn}
# 6. Convert  \SUBSCRIPTNB{n} into _n  and  \SUBCRIPT{nn} into _{nnn}
# 7. Expand hashes of verb and verbatim environments
# 8. Convert '\PERCENTAGE ' back into '\%'
# 9.. remove all \PAR tokens
# 10.  package specific processing:  endfloat: make sure \begin{figure} and \end{figure} are always
#      on a line by themselves, similarly for table environment
#  4, undo renaming of the \begin and \end in comments

#
# Note have to manually synchronize substitution commands below and 
# DIF.. command names in the header
sub postprocess {
  my ($begin,$len,$cnt,$float,$delblock,$addblock);
  # second level blocks
  my ($begin2,$cnt2,$len2,$eqarrayblock,$mathblock);

  for (@_) { 

    # change $'s in comments to something harmless
    1 while s/(%.*)\$/$1DOLLARDIF/mg ;

    # Remove final STOP token
    s/ STOP$//;
    # Replace \RIGHTBRACE by }    
    s/\\RIGHTBRACE/}/g;
    # Check all deleted blocks: where a deleted block contains a matching \begin and
    #    \end environment (these will be disabled by a %DIFDELCMD statements), enable
    #    these commands again (such that for example displayed math in a deleted equation
    #    is properly within math mode.  For math mode environments replace numbered equation
    #    environments with their display only variety (so that equation numbers in new file and
    #    diff file are identical
    while ( m/\\DIFdelbegin.*?\\DIFdelend/sg ) {
      $cnt=0;
      $len=length($&);
      $begin=pos($_) - $len;
      $delblock=$&;


      ### (.*?[^\n]?)\n? construct is necessary to avoid empty lines in math mode, which result in
      ### an error
      # displayed math environments
      $delblock=~ s/(\%DIFDELCMD < \s*\\begin\{((?:$MATHENV)|SQUAREBRACKET)\}\s*?(?:$DELCMDCLOSE|\n))(.*?[^\n]?)\n?(\%DIFDELCMD < \s*\\end\{\2\})/\\begin{$MATHREPL}$AUXCMD\n$1$3\n\\end{$MATHREPL}$AUXCMD\n$4/sg;
      # also transform the opposite pair \end{displaymath} .. \begin{displaymath} but we have to be careful not to interfere with the results of the transformation in the line directly above
      $delblock=~ s/(?<!${AUXCMD}\n)(\%DIFDELCMD < \s*\\end\{((?:$MATHENV)|SQUAREBRACKET)\}\s*?(?:$DELCMDCLOSE|\n))(.*?[^\n]?)\n?(?<!${AUXCMD}\n)(\%DIFDELCMD < \s*\\begin\{\2\})/\\end{MATHMODE}$AUXCMD\n$1$3\n\\begin{MATHMODE}$AUXCMD\n$4/sg;

      # now look for unpaired %DIFDELCMD < \begin{MATHENV}; if found add \begin{$MATHREPL} and insert \end{$MATHREPL} 
      # just before end of block; again we use look-behind assertion to avoid matching constructions which have already been converted
      if ($delblock=~ s/(?<!${AUXCMD}\n)(\%DIFDELCMD < \s*\\begin\{((?:$MATHENV)|SQUAREBRACKET)\}\s*?(?:$DELCMDCLOSE|\n))/$1\\begin{$MATHREPL}$AUXCMD\n/sg ) {
	$delblock =~ s/(\\DIFdelend$)/\\end{$MATHREPL}$AUXCMD\n$1/s ;
      }
      # now look for unpaired %DIFDELCMD < \end{MATHENV}; if found add \end{MATHMODE} and insert \begin{MATHMODE} 
      # just before end of block; again we use look-behind assertion to avoid matching constructions which have already been converted
      if ($delblock=~ s/(?<!${AUXCMD}\n)(\%DIFDELCMD < \s*\\end\{((?:$MATHENV)|SQUAREBRACKET)\}\s*?(?:$DELCMDCLOSE|\n))/$1\\end{MATHMODE}$AUXCMD\n/sg ) {
	$delblock =~ s/(\\DIFdelend$)/\\begin{MATHMODE}$AUXCMD\n$1/s ;
      }


      # equation array environment
      $delblock=~ s/(\%DIFDELCMD < \s*\\begin\{($MATHARRENV)\}\s*?(?:$DELCMDCLOSE|\n))(.*?[^\n]?)\n?(\%DIFDELCMD < \s*\\end\{\2\})/\\begin{$MATHARRREPL}$AUXCMD\n$1$3\n\\end{$MATHARRREPL}$AUXCMD\n$4/sg;
      $delblock=~ s/(?<!${AUXCMD}\n)(\%DIFDELCMD < \s*\\end\{($MATHARRENV)\}\s*?(?:$DELCMDCLOSE|\n))(.*?[^\n]?)\n?(?<!${AUXCMD}\n)(\%DIFDELCMD < \s*\\begin\{\2\})/\\end{MATHMODE}$AUXCMD\n$1$3\n\\begin{MATHMODE}$AUXCMD\n$4/sg;

      # now look for unpaired %DIFDELCMD < \begin{MATHARRENV}; if found add \begin{$MATHARRREPL} and insert \end{$MATHARRREPL} 
      # just before end of block; again we use look-behind assertion to avoid matching constructions which have already been converted
      if ($delblock=~ s/(?<!${AUXCMD}\n)(\%DIFDELCMD < \s*\\begin\{($MATHARRENV)\}\s*?(?:$DELCMDCLOSE|\n))/$1\\begin{$MATHARRREPL}$AUXCMD\n/sg ) {
	$delblock =~ s/(\\DIFdelend$)/\\end{$MATHARRREPL}$AUXCMD\n$1/s ;
      }
      # now look for unpaired %DIFDELCMD < \end{MATHENV}; if found add \end{MATHMODE} and insert \begin{MATHMODE} 
      # just before end of block; again we use look-behind assertion to avoid matching constructions which have already been converted
      if ($delblock=~ s/(?<!${AUXCMD}\n)(\%DIFDELCMD < \s*\\end\{($MATHARRENV)\}\s*?(?:$DELCMDCLOSE|\n))/$1\\end{MATHMODE}$AUXCMD\n/sg ) {
	$delblock =~ s/(\\DIFdelend$)/\\begin{MATHMODE}$AUXCMD\n$1/s ;
      }

      # parse $delblock for deleted and reinstated eqnarray* environments - within those reinstate \\ and & commands
      while ( $delblock =~ m/\\begin\Q{$MATHARRREPL}$AUXCMD\E\n.*?\n\\end\Q{$MATHARRREPL}$AUXCMD\E\n/sg ) {
	$cnt2=0;
	$len2=length($&);
	$begin2=pos($delblock) - $len2;
	$eqarrayblock=$&;
	# reinstate deleted & and \\ commands
	$eqarrayblock=~ s/(\%DIFDELCMD < \s*(\&|\\\\)\s*?(?:$DELCMDCLOSE|\n))/$1$2$AUXCMD\n/sg ;

	substr($delblock,$begin2,$len2)=$eqarrayblock;
	pos($delblock) = $begin2 + length($eqarrayblock);
      }



#    b.where one of the commands matching $COUNTERCMD is used as a DIFAUXCMD, add a statement
#      subtracting one from the respective counter to keep numbering consistent with new file
      $delblock=~ s/\\($COUNTERCMD)((?:${extraspace}\[$brat0\]${extraspace}|${extraspace}\{$pat4\})*\s*${AUXCMD}\n)/\\$1$2\\addtocounter{$1}{-1}${AUXCMD}\n/sg ;
#     c. If in-line math mode contains array environment, enclose the whole environment in \mbox'es
      while ( $delblock =~ m/($math)(\s*)/sg ) {
	$cnt2=0;
	$len2=length($&);
	$begin2=pos($delblock) - $len2;
	$mathblock="%\n\\mbox{$AUXCMD\n$1\n}$AUXCMD\n";
        next unless $mathblock =~ m/\{$ARRENV\}/ ;
	substr($delblock,$begin2,$len2)=$mathblock;
	pos($delblock) = $begin2 + length($mathblock);
      }

#     splice in modified delblock
      substr($_,$begin,$len)=$delblock;
      pos = $begin + length($delblock);
    }
    # make the array modification in added blocks
    while ( m/\\DIFaddbegin.*?\\DIFaddend/sg ) {
      $cnt=0;
      $len=length($&);
      $begin=pos($_) - $len;
      $addblock=$&;
      while ( $addblock =~ m/($math)(\s*)/sg ) {
	$cnt2=0;
	$len2=length($&);
	$begin2=pos($addblock) - $len2;
	$mathblock="%\n\\mbox{$AUXCMD\n$1\n}$AUXCMD\n";
        next unless $mathblock =~ m/\{$ARRENV\}/ ;
	substr($addblock,$begin2,$len2)=$mathblock;
	pos($addblock) = $begin2 + length($mathblock);
      }

#     splice in modified addblock
      substr($_,$begin,$len)=$addblock;
      pos = $begin + length($addblock);
    }


    ### old place for BEGINDIF, ENDDIF replacement
    # change begin and end commands  within comments such that they
    # don't disturb the pattern matching (if there are several \begin or \end in one line
    # this substitution is insufficient but that appears unlikely)
    s/(%.*)\\begin\{(.*)$/$1\\BEGINDIF\{$2/mg ;
    s/(%.*)\\end\{(.*)$/$1\\ENDDIF\{$2/mg ;

    # Replace MATHMODE environments from step 1a above by the correct Math environment

    # The next line is complicated.  The negative look-ahead insertion makes sure that no \end{$MATHENV} (or other mathematical
    # environments) are between the \begin{$MATHENV} and \end{MATHMODE} commands. This is necessary as the minimal matching 
    # is not globally minimal but only 'locally' (matching is beginning from the left side of the string)
    1 while s/\\begin{((?:$MATHENV)|(?:$MATHARRENV)|SQUAREBRACKET)}((?:.(?!(?:\\end{(?:(?:$MATHENV)|(?:$MATHARRENV)|SQUAREBRACKET)}|\\begin{MATHMODE})))*?)\\end{MATHMODE}/\\begin{$1}$2\\end{$1}/s;
    1 while s/\\begin{MATHMODE}((?:.(?!\\end{MATHMODE}))*?)\\end{((?:$MATHENV)|(?:$MATHARRENV)|SQUAREBRACKET)}/\\begin{$2}$1\\end{$2}/s;
    # convert remaining \begin{MATHMODE} \end{MATHMODE} (and not containing & or \\ )into MATHREPL environments
    s/\\begin{MATHMODE}((?:(.(?!(?<!\\)\&|\\\\))*)?)\\end{MATHMODE}/\\begin{$MATHREPL}$1\\end{$MATHREPL}/sg;
    # others into MATHARRREPL
    s/\\begin{MATHMODE}(.*?)\\end{MATHMODE}/\\begin{$MATHARRREPL}$1\\end{$MATHARRREPL}/sg;

    # now look for AUXCMD math-mode pairs which have only comments (or empty lines between them), and remove the added commands
    s/\\begin{((?:$MATHENV)|(?:$MATHARRENV)|SQUAREBRACKET)}$AUXCMD\n((?:\s*%.[^\n]*\n)*)\\end{\1}$AUXCMD\n/$2/sg; 


    # Remove all mark up within picture environments
    while ( m/\\begin\{($PICTUREENV)\}.*?\\end\{\1\}/sg ) {
      $cnt=0;
      $len=length($&);
      $begin=pos($_) - $len;
      $float=$&;
      $float =~ s/\\DIFaddbegin //g;
      $float =~ s/\\DIFaddend //g;
      $float =~ s/\\DIFadd\{($pat4)\}/$1/g;
      $float =~ s/\\DIFdelbegin //g;
      $float =~ s/\\DIFdelend //g;
      $float =~ s/\\DIFdel\{($pat4)\}//g;
      substr($_,$begin,$len)=$float;
      pos = $begin + length($float);
    }
    # Convert DIFadd, DIFdel, DIFFaddbegin , ... into  varieties
    #    within floats (currently recognised float environments: plate,table,figure
    #    plus starred varieties).
    while ( m/\\begin\{($FLOATENV)\}.*?\\end\{\1\}/sg ) {
      $cnt=0;
      $len=length($&);
      $begin=pos($_) - $len;
      $float=$&;
      $float =~ s/\\DIFaddbegin /\\DIFaddbeginFL /g;
      $float =~ s/\\DIFaddend /\\DIFaddendFL /g;
      $float =~ s/\\DIFadd\{/\\DIFaddFL{/g;
      $float =~ s/\\DIFdelbegin /\\DIFdelbeginFL /g;
      $float =~ s/\\DIFdelend /\\DIFdelendFL /g;
      $float =~ s/\\DIFdel\{/\\DIFdelFL{/g;
      substr($_,$begin,$len)=$float;
      pos = $begin + length($float);
    }
    ### former location of undo renaming of \begin and \end in comments

    # remove empty DIFCMD < lines
    s/^\Q${DELCMDOPEN}\E\n//msg;

    # Expand hashes of verb and verbatim environments (note negative look behind assertion to not leak out of DIFDELCMD comments
    s/(\\verb\*?)\{([-\d]*?)\}/"${1}". fromhash(\%verbhash,$2)/esg;
    s/${DELCMDOPEN}\\(verbatim\*?)\{([-\d]*?)\}/"${DELCMDOPEN}\\begin{${1}}".fromhash(\%verbhash,$2,$DELCMDOPEN)."${DELCMDOPEN}\\end{${1}}"/esg;
    s/\\(verbatim\*?)\{([-\d]*?)\}/"\\begin{${1}}".fromhash(\%verbhash,$2)."\\end{${1}}"/esg;
    # Convert '\PERCENTAGE ' back into '\%'			       
    s/\\PERCENTAGE /\\%/g;
    # remove all \PAR tokens (taking care to properly keep commented out PAR's
    # from introducing uncommented newlines - next line)
    s/(%DIF < )([^\n]*?)\\PAR\n/$1$2\n$1\n/sg;
    # convert PAR commands which are on a line by themselves
    s/\n(\s*?)\\PAR\n/\n\n/sg;
    # convert remaining PAR commands (which are preceded by non-white space characters, usually "}" ($ADDCLOSE)
    s/\\PAR\n/\n\n/sg;

    #  package specific processing: 
    if ( defined($packages{"endfloat"})) {
      #endfloat: make sure \begin{figure} and \end{figure} are always
      #      on a line by themselves, similarly for table environment
      print STDERR "endfloat package detected.\n" if $verbose ;
      # eliminate whitespace before and after
      s/^(\s*)(\\(?:begin|end)\{(?:figure|table)\})(\s*)$/$2/mg;
      # split lines with remaining characters before float enviroment conmmand
      s/^(.+)(\\(?:begin|end)\{(?:figure|table)\})/$1\n$2/mg;
      # split lines with remaining characters after float enviroment conmmand
      s/(\\(?:begin|end)\{(?:figure|table)\})(.+)$/$1\n$2/mg;
    }
    # undo renaming of the \begin and \end  and dollars in comments 
    s/(%.*)\\BEGINDIF\{(.*)$/$1\\begin\{$2/mg ;
    s/(%.*)\\ENDDIF\{(.*)$/$1\\end\{$2/mg ;
    1 while s/(%.*)DOLLARDIF/$1\$/mg ;
#   Convert \begin{SQUAREBRACKET} \end{SQUAREBRACKET} into \[ \]
    s/\\end{SQUAREBRACKET}/\\\]/sg;
    s/\\begin{SQUAREBRACKET}/\\\[/sg;
# 4. Convert \begin{DOLLARDOLLAR} \end{DOLLARDOLLAR} into $$ $$
    s/\\begin\{DOLLARDOLLAR\}(.*?)\\end\{DOLLARDOLLAR\}/\$\$$1\$\$/sg;
# 5. Convert  \SUPERSCRIPTNB{n} into ^n  and  \SUPERSCRIPT{nn} into ^{nnn}
    s/\\SUPERSCRIPTNB{($pat0)}/^$1/g ;
    s/\\SUPERSCRIPT{($pat4)}/^{$1}/g ;
    # Convert  \SUBSCRIPNB{n} into _n  and  \SUBCRIPT{nn} into _{nnn}
    s/\\SUBSCRIPTNB{($pat0)}/_$1/g ;
    s/\\SUBSCRIPT{($pat4)}/_{$1}/g ;

  return;
  }
}


# @diffs=linediff(\@seq1, \@seq2)
# mark up lines like this
#%DIF mm-mmdnn
#%< old deleted line(s)
#%DIF -------
#%DIF mmann-nn
#new appended line %< 
#%DIF -------
# Future extension: mark change explicitly
# Assumes: traverse_sequence traverses deletions before insertions in changed sequences
#          all line numbers relative to line 0 (first line of real file)
sub linediff {
  my $seq1 = shift ;
  my $seq2 = shift ;

  my $block = [];
  my $retseq = [];
  my @begin=('','',''); # dummy initialisation
  my $instring ; 

  my $discard = sub { @begin=('d',$_[0],$_[1]) unless scalar @$block ; 
                      push(@$block, "%DIF < " . $seq1->[$_[0]]) };
  my $add = sub { if (! scalar  @$block) {
		    @begin=('a',$_[0],$_[1]) ;}
		  elsif ( $begin[0] eq 'd' ) {
                    $begin[0]='c'; $begin[2]=$_[1];
		    push(@$block, "%DIF -------") }
                  push(@$block,  $seq2->[$_[1]] . " %DIF > " ) };
  my $match = sub { if ( scalar @$block ) {
                      if ( $begin[0] eq 'd' && $begin[1]!=$_[0]-1) {
			$instring = sprintf "%%DIF %d-%dd%d",$begin[1],$_[0]-1,$begin[2]; }
		      elsif ( $begin[0] eq 'a' && $begin[2]!=$_[1]-1) {
			$instring = sprintf "%%DIF %da%d-%d",$begin[1],$begin[2],$_[1]-1; }
		      elsif ( $begin[0] eq 'c' ) {
			$instring = sprintf "%%DIF %sc%s",
			                     ($begin[1]==$_[0]-1) ? "$begin[1]" : $begin[1]."-".($_[0]-1)  , 
			                     ($begin[2]==$_[1]-1) ? "$begin[2]" : $begin[2]."-".($_[1]-1)  ; }
		      else {
			$instring = sprintf "%%DIF %d%s%d",$begin[1],$begin[0],$begin[2]; }
		      push @$retseq, $instring,@$block, "%DIF -------" ; 
		      $block = []; 
		    }
		    push @$retseq, $seq2->[$_[1]]
		  };
  # key function: remove multiple spaces (such that insertion or deletion of redundant white space is not reported)
  my $keyfunc = sub { join("  ",split(" ",shift())) };

  traverse_sequences($seq1,$seq2, { MATCH=>$match, DISCARD_A=>$discard, DISCARD_B=>$add }, $keyfunc );
  push @$retseq, @$block if scalar @$block; 

  return wantarray ? @$retseq : $retseq ;
}



# init_regex_arr_data(\@array,"TOKEN INIT")
# scans DATA file handel for line "%% TOKEN INIT" line
# then appends each line not beginning with % into array (as a quoted regex)
sub init_regex_arr_data {
  my ($arr,$token)=@_;
  my ($copy);
  while (<DATA>) {
    if ( m/^%%BEGIN $token\s*$/ ) {
      $copy=1; }
    elsif ( m/^%%END $token\s*/ )  {
      last; }
    chomp;
    push (@$arr,qr/^$_$/) if ( $copy && !/^%/ ) ;
  }
  seek DATA,0,0;    # rewind DATA handle to file begin
}


# init_regex_arr_ext(\@array,$arg)
# fills array with regular expressions.
# if arg is a file name, then read in list of regular expressions from that file
# (one expression per line)
# Otherwise treat arg as a comma separated list of regular expressions
sub init_regex_arr_ext {
  my ($arr,$arg)=@_;
  my $regex;
  if ( -f $ arg ) {
    open(FILE,"$arg") or die ("Couldn't open $arg: $!");
    while (<FILE>) {
      chomp;
      next if /^\s*#/ || /^\s*%/ || /^\s*$/ ;
      push (@$arr,qr/^$_$/);
    }
    close(FILE);
  }
  else {
    # assume it is a comma-separated list of reg-ex
    foreach $regex (split(qr/(?<!\\),/,$arg)) {
      $regex =~ s/\\,/,/g;
      push (@$arr,qr/^$regex$/);
    }
  }
}

#exetime() returns time since last execution of this command
#exetime(1) resets this time
my $lasttime=-1;   # global variable for persistence
sub exetime {
  my $reset=0;
  my $retval;
  if ((scalar @_) >=1) {
    $reset=shift;
  }
  if ($reset) {
    $lasttime=times();
  }
  else {
    $retval=times()-$lasttime;
    $lasttime=$lasttime+$retval;
    return($retval);
  }
}


sub usage {
  die <<"EOF"; 
Usage: $0 [options] old.tex new.tex > diff.tex

Compares two latex files and writes tex code to stdout, which has the same
format as new.tex but has all changes relative to old.tex marked up or commented.

--type=markupstyle
-t markupstyle         Add code to preamble for selected markup style
                       Available styles: UNDERLINE CTRADITIONAL TRADITIONAL CFONT FONTSTRIKE INVISIBLE 
                                         CHANGEBAR CCHANGEBAR CULINECHBAR CFONTCBHBAR
                       [ Default: UNDERLINE ]

--subtype=markstyle
-s markstyle           Add code to preamble for selected style for bracketing
                       commands (e.g. to mark changes in  margin)
                       Available styles: SAFE MARGINAL DVIPSCOL
                       [ Default: SAFE ]

--floattype=markstyle
-f markstyle           Add code to preamble for selected style which 
                       replace standard marking and markup commands within floats
                       (e.g., marginal remarks cause an error within floats
                       so marginal marking can be disabled thus)
                       Available styles: FLOATSAFE IDENTICAL
                       [ Default: FLOATSAFE ]

--encoding=enc
-e enc                 Specify encoding of old.tex and new.tex. Typical encodings are
                       ascii, utf8, latin1, latin9.  A list of available encodings can be 
                       obtained by executing 
                       perl -MEncode -e 'print join ("\\n",Encode->encodings( ":all" )) ;'
                       [Default encoding is utf8 unless the first few lines of the preamble contain
                       an invocation "\\usepackage[..]{inputenc} in which case the 
                       encoding chosen by this command is asssumed. Note that ASCII (standard
                       latex) is a subset of utf8]

--preamble=file
-p file                Insert file at end of preamble instead of auto-generating
                       preamble.  The preamble must define the following commands
                       \\DIFaddbegin,\\DIFaddend,\\DIFadd{..},
                       \\DIFdelbegin,\\DIFdelend,\\DIFdel{..},
                       and varieties for use within floats
                       \\DIFaddbeginFL,\\DIFaddendFL,\\DIFaddFL{..},
                       \\DIFdelbeginFL,\\DIFdelendFL,\\DIFdelFL{..}
                       (If this option is set -t, -s, and -f options
                       are ignored.)

--exclude-safecmd=exclude-file
--exclude-safecmd="cmd1,cmd2,..."
-A exclude-file 
--replace-safecmd=replace-file
--append-safecmd=append-file
--append-safecmd="cmd1,cmd2,..."
-a append-file         Exclude from, replace or append to the list of regex
                       matching commands which are safe to use within the 
                       scope of a \\DIFadd or \\DIFdel command.  The file must contain
                       one Perl-RegEx per line (Comment lines beginning with # or % are
                       ignored). A literal comma within the comma-separated list must be
                       escaped thus "\\,",   Note that the RegEx needs to match the whole of 
                       the token, i.e., /^regex\$/ is implied and that the initial
                       "\\" of the command is not included. The --exclude-safecmd
                       and --append-safecmd options can be combined with the --replace-safecmd 
                       option and can be used repeatedly to add cumulatively to the lists.

--exclude-textcmd=exclude-file 
--exclude-textcmd="cmd1,cmd2,..."
-X exclude-file
--replace-textcmd=replace-file
--append-textcmd=append-file
--append-textcmd="cmd1,cmd2,..."
-x append-file         Exclude from, replace or append to the list of regex
                       matching commands whose last argument is text.  See
                       entry for --exclude-safecmd directly above for further details.

--replace-context1cmd=replace-file
--append-context1cmd=append-file
--append-context1cmd="cmd1,cmd2,..."
                       Replace or append to the list of regex matching commands
                       whose last argument is text but which require a particular
                       context to work, e.g. \\caption will only work within a figure
                       or table.  These commands behave like text commands, except when 
                       they occur in a deleted section, when they are disabled, but their
                       argument is shown as deleted text.

--replace-context2cmd=replace-file
--append-context2cmd=append-file
--append-context2cmd="cmd1,cmd2,..."
                       As corresponding commands for context1.  The only difference is that
                       context2 commands are completely disabled in deleted sections, including
                       their arguments.


--config var1=val1,var2=val2,...
-c var1=val1,..        Set configuration variables.
-c configfile           Available variables: 
                          MINWORDSBLOCK (integer)
                          FLOATENV (RegEx)
                          PICTUREENV (RegEx)
                          MATHENV (RegEx)
                          MATHREPL (String)
                          MATHARRENV (RegEx)
                          MATHARRREPL (String)
                          ARRENV (RegEx)
                          COUNTERCMD (RegEx)
                       This option can be repeated.


--packages=pkg1,pkg2,..
                       Tell latexdiff that .tex file is processed with the packages in list 
                       loaded.  This is normally not necessary if the .tex file includes the
                       preamble, as the preamble is automatically scanned for \\usepackage commands.
                       Use of the --packages option disables automatic scanning, so if for any
                       reason package specific parsing needs to be switched off, use --packages=none.
                       The following packages trigger special behaviour:
                       endfloat hyperref amsmath
                       [ Default: scan the preamble for \\usepackage commands to determine
                         loaded packages.]

--show-preamble        Print generated or included preamble commands to stdout.

--show-safecmd         Print list of regex matching and excluding safe commands.

--show-textcmd         Print list of regex matching and excluding commands with text argument.

--show-config          Show values of configuration variables

--show-all             Show all of the above

   NB For all --show commands, no old.tex or new.tex file needs to be given, and no 
      differencing takes place.

--allow-spaces         Allow spaces between bracketed or braced arguments to commands
                       [Default requires arguments to directly follow each other without 
                                intervening spaces]

--flatten              Replace \\input and \\include commands within body by the content
                       of the files in their argument.  If \\includeonly is present in the
                       preamble, only those files are expanded into the document. However, 
                       no recursion is done, i.e. \\input and \\include commands within 
                       included sections are not expanded.  The included files are assumed to 
                       be located in the same directories as the old and new master files,
                       respectively, making it possible to organise files into old and new directories.

--help
-h                     Show this help text.

--ignore-warnings      Suppress warnings about inconsistencies in length between input
                       and parsed strings and missing characters. 

--verbose
-V                     Output various status information to stderr during processing.
                       Default is to work silently.

--version              Show version number.
EOF
}

=head1 NAME

latexdiff - determine and markup differences between two latex files

=head1 SYNOPSIS

B<latexdiff> [ B<OPTIONS> ] F<old.tex> F<new.tex> > F<diff.tex>

=head1 DESCRIPTION

Briefly, I<latexdiff> is a utility program to aid in the management of
revisions of latex documents. It compares two valid latex files, here
called C<old.tex> and C<new.tex>, finds significant differences
between them (i.e., ignoring the number of white spaces and position
of line breaks), and adds special commands to highlight the
differences.  Where visual highlighting is not possible, e.g. for changes
in the formatting, the differences are
nevertheless marked up in the source.

The program treats the preamble differently from the main document.
Differences between the preambles are found using line-based
differencing (similarly to the Unix diff command, but ignoring white
spaces).  A comment, "S<C<%DIF E<gt>>>" is appended to each added line, i.e. a 
line present in C<new.tex> but not in C<old.tex>.  Discarded lines 
 are deactivated by prepending "S<C<%DIF E<lt>>>". Changed blocks are preceded  by
comment lines giving information about line numbers in the original files.  Where there are insignificant
differences, the resulting file C<diff.tex> will be similar to
C<new.tex>.  At the end of the preamble, the definitions for I<latexdiff> markup commands are inserted.
In differencing the main body of the text, I<latexdiff> attempts to
satisfy the following guidelines (in order of priority):

=over 3

=item 1

If both C<old.tex> and C<new.tex> are valid LaTeX, then the resulting
C<diff.tex> should also be valid LateX. (NB If a few plain TeX commands
are used within C<old.tex> or C<new.tex> then C<diff.tex> is not
guaranteed to work but usually will).

=item 2

Significant differences are determined on the level of
individual words. All significant differences, including differences
between comments should be clearly marked in the resulting source code
C<diff.tex>.

=item 3

If a changed passage contains text or text-producing commands, then
running C<diff.tex> through LateX should produce output where added
and discarded passages are highlighted.

=item 4

Where there are insignificant differences, e.g. in the positioning of
line breaks, C<diff.tex> should follow the formatting of C<new.tex>

=back

For differencing the same algorithm as I<diff> is used but words
instead of lines are compared.  An attempt is made to recognize
blocks which are completely changed such that they can be marked up as a unit.
Comments are differenced line by line
but the number of spaces within comments is ignored. Commands including
all their arguments are generally compared as one unit, i.e., no mark-up
is inserted into the arguments of commands.  However, for a selected
number of commands (for example, C<\caption> and all sectioning
commands) the last argument is known to be text. This text is
split into words and differenced just as ordinary text (use options to
show and change the list of text commands, see below). As the
algorithm has no detailed knowledge of LaTeX, it assumes all pairs of
curly braces immediately following a command (i.e. a sequence of
letters beginning with a backslash) are arguments for that command.
As a restriction to condition 1 above it is thus necessary to surround
all arguments with curly braces, and to not insert
extraneous spaces.  For example, write 

  \section{\textem{This is an emphasized section title}}

and not

  \section {\textem{This is an emphasized section title}}

or

  \section\textem{This is an emphasized section title}

even though all varieties are the same to LaTeX (but see
B<--allow-spaces> option which allows the second variety).

For environments whose content does not conform to standard LaTeX or
where graphical markup does not make sense all markup commands can be
removed by setting the PICTUREENV configuration variable, set by
default to C<picture> and C<DIFnomarkup> environments; see B<--config>
option).  The latter environment (C<DIFnomarkup>) can be used to
protect parts of the latex file where the markup results in illegal
markup. You have to surround the offending passage in both the old and
new file by C<\begin{DIFnomarkup}> and C<\end{DIFnomarkup}>. You must
define the environment in the preambles of both old and new
documents. I prefer to define it as a null-environment,

C<\newenvironment{DIFnomarkup}{}{}>

but the choice is yours.  Any markup within the environment will be
removed, and generally everything within the environment will just be
taken from the new file.

It is also possible to difference files which do not have a preamble. 
 In this case, the file is processed in the main document
mode, but the definitions of the markup commands are not inserted.

All markup commands inserted by I<latexdiff> begin with "C<\DIF>".  Added
blocks containing words, commands or comments which are in C<new.tex>
but not in C<old.tex> are marked by C<\DIFaddbegin> and C<\DIFaddend>.
Discarded blocks are marked by C<\DIFdelbegin> and C<\DIFdelend>.
Within added blocks all text is highlighted with C<\DIFadd> like this:
C<\DIFadd{Added text block}>
Selected `safe' commands can be contained in these text blocks as well
(use options to show and change the list of safe commands, see below).
All other commands as well as braces "{" and "}" are never put within
the scope of C<\DIFadd>.  Added comments are marked by prepending
"S<C<%DIF E<gt> >>".

Within deleted blocks text is highlighted with C<\DIFdel>.  Deleted
comments are marked by prepending "S<C<%DIF E<lt> >>".  Non-safe command
and curly braces within deleted blocks are commented out with 
"S<C<%DIFDELCMD E<lt> >>".



=head1 OPTIONS

=head2 Preamble

The following options determine the visual markup style by adding the appropriate
command definitions to the preamble. See the end of this section for a description of 
available styles.

=over 4

=item B<--type=markupstyle> or
B<-t markupstyle>

Add code to preamble for selected markup style. This option defines
C<\DIFadd> and C<\DIFdel> commands.
Available styles: 

C<UNDERLINE CTRADITIONAL TRADITIONAL CFONT FONTSTRIKE INVISIBLE 
CHANGEBAR CCHANGEBAR CULINECHBAR CFONTCBHBAR>

[ Default: C<UNDERLINE> ]

=item B<--subtype=markstyle> or
B<-s markstyle> 

Add code to preamble for selected style for bracketing
commands (e.g. to mark changes in  margin). This option defines
C<\DIFaddbegin>, C<\DIFaddend>, C<\DIFdelbegin> and C<\DIFdelend> commands.
Available styles: C<SAFE MARGINAL DVIPSCOL>

[ Default: C<SAFE> ]

=item B<--floattype=markstyle> or
B<-f markstyle>

Add code to preamble for selected style which 
replace standard marking and markup commands within floats
(e.g., marginal remarks cause an error within floats
so marginal marking can be disabled thus). This option defines all 
C<\DIF...FL> commands.
Available styles: C<FLOATSAFE TRADITIONALSAFE IDENTICAL>

[ Default: C<FLOATSAFE> ]

=item B<--encoding=enc> or 
B<-e enc>

Specify encoding of old.tex and new.tex. Typical encodings are
C<ascii>, C<utf8>, C<latin1>, C<latin9>.  A list of available encodings can be 
obtained by executing 

C<perl -MEncode -e 'print join ("\n",Encode->encodings( ":all" )) ;' >

[Default encoding is utf8 unless the first few lines of the preamble contain
an invocation C<\usepackage[..]{inputenc}> in which case the 
encoding chosen by this command is asssumed. Note that ASCII (standard
latex) is a subset of utf8]

=item B<--preamble=file> or
B<-p file>

Insert file at end of preamble instead of generating
preamble.  The preamble must define the following commands
C<\DIFaddbegin, \DIFaddend, \DIFadd{..},
\DIFdelbegin,\DIFdelend,\DIFdel{..},>
and varieties for use within floats
C<\DIFaddbeginFL, \DIFaddendFL, \DIFaddFL{..},
\DIFdelbeginFL, \DIFdelendFL, \DIFdelFL{..}>
(If this option is set B<-t>, B<-s>, and B<-f> options
are ignored.)

=item B<--packages=pkg1,pkg2,..> 

Tell latexdiff that .tex file is processed with the packages in list
loaded.  This is normally not necessary if the .tex file includes the
preamble, as the preamble is automatically scanned for C<\usepackage> commands.
Use of the B<--packages> option disables automatic scanning, so if for any
reason package specific parsing needs to be switched off, use B<--packages=none>.
The following packages trigger special behaviour:

=over 8

=item C<amsmath> 

Configuration variable amsmath is set to C<align*> (Default: C<eqnarray*>)

=item C<endfloat> 

Ensure that C<\begin{figure}> and C<\end{figure}> always appear by themselves on a line.

=item C<hyperref>

Change name of C<\DIFadd> and C<\DIFdel> commands to C<\DIFaddtex> and C<\DIFdeltex> and 
define new C<\DIFadd> and C<\DIFdel> commands, which provide a wrapper for these commands,
using them for the text but not for the link defining command (where any markup would cause
errors).

=back

[ Default: scan the preamble for C<\\usepackage> commands to determine
  loaded packages.]



=item B<--show-preamble>

Print generated or included preamble commands to stdout.

=back

=head2 Configuration

=over 4

=item B<--exclude-safecmd=exclude-file> or
B<-A exclude-file> or  B<--exclude-safecmd="cmd1,cmd2,...">

=item B<--replace-safecmd=replace-file>

=item B<--append-safecmd=append-file> or 
B<-a append-file> or B<--append-safecmd="cmd1,cmd2,...">

Exclude from, replace or append to the list of regular expressions (RegEx)
matching commands which are safe to use within the 
scope of a C<\DIFadd> or C<\DIFdel> command.  The file must contain
one Perl-RegEx per line (Comment lines beginning with # or % are
ignored).  Note that the RegEx needs to match the whole of 
the token, i.e., /^regex$/ is implied and that the initial
"\" of the command is not included. 
The B<--exclude-safecmd> and B<--append-safecmd> options can be combined with the -B<--replace-safecmd> 
option and can be used repeatedly to add cumulatively to the lists.
 B<--exclude-safecmd>
and B<--append-safecmd> can also take a comma separated list as input. If a
comma for one of the regex is required, escape it thus "\,". In most cases it
will be necessary to protect the comma-separated list from the shell by putting
it in quotation marks.

=item B<--exclude-textcmd=exclude-file> or
B<-X exclude-file> or B<--exclude-textcmd="cmd1,cmd2,...">

=item B<--replace-textcmd=replace-file>

=item B<--append-textcmd=append-file> or 
B<-x append-file> or B<--append-textcmd="cmd1,cmd2,...">

Exclude from, replace or append to the list of regular expressions
matching commands whose last argument is text.  See
entry for B<--exclude-safecmd> directly above for further details.


=item B<--replace-context1cmd=replace-file> 

=item B<--append-context1cmd=append-file> or
=item B<--append-context1cmd="cmd1,cmd2,...">

Replace or append to the list of regex matching commands
whose last argument is text but which require a particular
context to work, e.g. \caption will only work within a figure
or table.  These commands behave like text commands, except when 
they occur in a deleted section, when they are disabled, but their
argument is shown as deleted text.

=item B<--replace-context1cmd=replace-file> 

=item B<--append-context2cmd=append-file> or
=item B<--append-context2cmd="cmd1,cmd2,...">
As corresponding commands for context1.  The only difference is that
context2 commands are completely disabled in deleted sections, including
their arguments.



=item B<--config var1=val1,var2=val2,...> or B<-c var1=val1,..>

=item B<-c configfile>

Set configuration variables.  The option can be repeated to set different
variables (as an alternative to the comma-separated list).
Available variables (see below for further explanations): 

C<MINWORDSBLOCK> (integer)

C<FLOATENV> (RegEx)

C<PICTUREENV> (RegEx)

C<MATHENV> (RegEx)

C<MATHREPL> (String)

C<MATHARRENV> (RegEx)

C<MATHARRREPL> (String)

C<ARRENV> (RegEx)

C<COUNTERCMD> (RegEx)

=item B<--show-safecmd>

Print list of RegEx matching and excluding safe commands.

=item B<--show-textcmd>

Print list of RegEx matching and excluding commands with text argument.

=item B<--show-config>

Show values of configuration variables.

=item B<--show-all>

Combine all --show commands.

NB For all --show commands, no C<old.tex> or C<new.tex> file needs to be specified, and no 
differencing takes place.


=back

=head2 Miscellaneous

=over 4

=item B<--verbose> or B<-V>

Output various status information to stderr during processing.
Default is to work silently.

=item B<--ignore-warnings>

Suppress warnings about inconsistencies in length between input and
parsed strings and missing characters.  These warning messages are
often related to non-standard latex or latex constructions with a
syntax unknown to C<latexdiff> but the resulting difference argument
is often fully functional anyway, particularly if the non-standard
latex only occurs in parts of the text which have not changed.

=item B<--allow-spaces>

Allow spaces between bracketed or braced arguments to commands.  Note
that this option might have undesirable side effects (unrelated scope
might get lumpeded with preceding commands) so should only be used if the
default produces erroneous results.  (Default requires arguments to
directly follow each other without intervening spaces).

=item B<--flatten>

Replace C<\input> and C<\include> commands within body by the content
of the files in their argument.  If C<\includeonly> is present in the
preamble, only those files are expanded into the document. However, 
no recursion is done, i.e. C<\input> and C<\include> commands within 
included sections are not expanded.  The included files are assumed to 
 be located in the same directories as the old and new master files,
respectively, making it possible to organise files into old and new directories. 

Use of this option is not recommended
primarily the processing time for the large documents is prohibitive, and
the resulting difference document no longer reflects the structure of the 
input documents. 

=item B<--help> or
B<-h>

Show help text

=item B<--version>

Show version number

=back

=head2 Predefined styles 

=head2 Major types

The major type determine the markup of plain text and some selected latex commands outside floats by defining the markup commands C<\DIFadd{...}> and C<\DIFdel{...}> .

=over 10

=item C<UNDERLINE>

Added text is wavy-underlined and blue, discarded text is struck out and red
(Requires color and ulem packages).  Overstriking does not work in displayed math equations such that deleted parts of equation are underlined, not struck out (this is a shortcoming inherent to the ulem package).

=item C<CTRADITIONAL>

Added text is blue and set in sans-serif, and a red footnote is created for each discarded 
piece of text. (Requires color package)

=item C<TRADITIONAL>

Like C<CTRADITIONAL> but without the use of color.

=item C<CFONT>

Added text is blue and set in sans-serif, and discarded text is red and very small size.

=item C<FONTSTRIKE>

Added tex is set in sans-serif, discarded text small and struck out

=item C<CCHANGEBAR>

Added text is blue, and discarded text is red.  Additionally, the changed text is marked with a bar in the margin (Requires color and changebar packages).

=item C<CFONTCHBAR>

Like C<CFONT> but with additional changebars (Requires color and changebar packages).

=item C<CULINECHBAR>

Like C<UNDERLINE> but with additional changebars (Requires color, ulem and changebar packages).

=item C<CHANGEBAR>

No mark up of text, but mark margins with changebars (Requires changebar package).

=item C<INVISIBLE>

No visible markup (but generic markup commands will still be inserted.

=back

=head2 Subtypes

The subtype defines the commands that are inserted at the begin and end of added or discarded blocks, irrespectively of whether these blocks contain text or commands (Defined commands: C<\DIFaddbegin, \DIFaddend, \DIFdelbegin, \DIFdelend>) 

=over 10

=item C<SAFE>

No additional markup (Recommended choice)

=item C<MARGIN>

Mark beginning and end of changed blocks with symbols in the margin nearby (using
the standard C<\marginpar> command - note that this sometimes moves somewhat
from the intended position.

=item C<DVIPSCOL>

An alternative way of marking added passages in blue, and deleted ones in red. Note
that C<DVIPSCOL> only works with the dvips converter, e.g. not pdflatex.
(it is recommeneded to use instead the main types to effect colored markup,
although in some cases coloring with dvipscol can be more complete).

=back

=head2 Float Types

Some of the markup used in the main text might cause problems when used within 
floats (e.g. figures or tables).  For this reason alternative versions of all
markup commands are used within floats. The float type defines these alternative commands.

=over 10

=item C<FLOATSAFE>

Use identical markup for text as in the main body, but set all commands marking the begin and end of changed blocks to null-commands.  You have to choose this float type if your subtype is C<MARGIN> as C<\marginpar> does not work properly within floats.

=item C<TRADITIONALSAFE>

Mark additions the same way as in the main text.  Deleted environments are marked by angular brackets \[ and \] and the deleted text is set in scriptscript size. This float type should always be used with the C<TRADITIONAL> and  C<CTRADITIONAL> markup types as the \footnote command does not work properly in floating environments.

=item C<IDENTICAL>

Make no difference between the main text and floats.

=back


=head2 Configuration Variables

=over 10

=item C<MINWORDSBLOCK>

Minimum number of tokens required to form an independent block. This value is
used in the algorithm to detect changes of complete blocks by merging identical text parts of less than C<MINWORDSBLOCK> to the preceding added and discarded parts.

[ Default: 3 ]

=item C<FLOATENV>

Environments whose name matches the regular expression in C<FLOATENV> are 
considered floats.  Within these environments, the I<latexdiff> markup commands
are replaced by their FL variaties.

[ Default: S<C<(?:figure|table|plate)[\w\d*@]*> >]

=item C<PICTUREENV>

Within environments whose name matches the regular expression in C<PICTUREENV>
all latexdiff markup is removed (in pathologic cases this might lead to
 inconsistent markup but this situation should be rare).

[ Default: S<C<(?:picture|DIFnomarkup)[\w\d*@]*> >]

=item C<MATHENV>,C<MATHREPL>

If both \begin and \end for a math environment (environment name matching C<MATHENV>
or \[ and \])
are within the same deleted block, they are replaced by a \begin and \end commands for C<MATHREPL>
rather than being commented out.

[ Default: C<MATHENV>=S<C<(?:displaymath|equation)> >, C<MATHREPL>=S<C<displaymath> >]

=item C<MATHARRENV>,C<MATHARRREPL>

as C<MATHENV>,C<MATHREPL> but for equation arrays

[ Default: C<MATHARRENV>=S<C<eqnarray\*?> >, C<MATHREPL>=S<C<eqnarray> >]

=item C<ARRENV>

If a match to C<ARRENV> is found within an inline math environment within a deleted or added block, then the inlined math 
is surrounded by C<\mbox{>...C<}>.  This is necessary as underlining does not work within inlined array environments.

[ Default: C<ARRENV>=S<C<(?:array|[pbvBV]matrix)> >

=item C<COUNTERCMD>

If a command in a deleted block which is also in the textcmd list matches C<COUNTERCMD> then an
additional command C<\addtocounter{>F<cntcmd>C<}{-1}>, where F<cntcmd> is the matching command, is appended in the diff file such that the numbering in the diff file remains synchronized with the
numbering in the new file.

[ Default: C<COUNTERCMD>=C<(?:footnote|part|section|subsection> ...

C<|subsubsection|paragraph|subparagraph)>  ]

=back

=head1 BUGS

UTF-8 support requires a relatively new version of perl (5.8.0 is sufficient 
but 5.6.2 up would work OK, too).

Option allow-spaces not implemented entirely consistently. It breaks
the rules that number and type of white space does not matter, as
different numbers of inter-argument spaces are treated as significant.

Please send bug reports
to I<tilmann@esc.cam.ac.uk>.  Include the serial number of I<latexdiff>
(from comments at the top of the source or use B<--version>).  If you come across latex
files that are error-free and conform to the specifications set out
above, and whose differencing still does not result in error-free
latex, please send me those files, ideally edited to only contain the
offending passage as long as that still reproduces the problem. 

=head1 SEE ALSO

L<latexrevise>

=head1 PORTABILITY

I<latexdiff> does not make use of external commands and thus should run
on any platform  supporting Perl 5.6 or higher.  If files with encodings 
other than ASCII or UTF-8 are processed, Perl 5.8 or higher is required.

The standard version of I<latexdiff> requires installation of the Perl package
C<Algorithm::Diff> (available from I<www.cpan.org> - 
I<http://search.cpan.org/~nedkonz/Algorithm-Diff-1.15>) but a stand-alone
version, I<latexdiff-so>, which has this package inlined, is available, too.
I<latexdiff-fast> requires the I<diff> command to be present.

=head1 AUTHOR

Copyright (C) 2004-2007 Frederik Tilmann

This program is free software; you can redistribute it and/or modify
it under the terms of the GNU General Public License Version 2

Contributors of fixes and additions: V. Kuhlmann, J. Paisley, N. Becker, T. Doerges, K. Huebner
Thanks to everyone who send in bug reports.

=cut

__END__
%%BEGIN SAFE COMMANDS
% Regex matching commands which can safely be in the
% argument of a \DIFadd or \DIFdel command (leave out the \)
arabic
dashbox
emph
fbox
framebox
hspace
math.*
makebox
mbox
pageref
ref
symbol
raisebox
rule
text.*
shortstack
usebox
dag
ddag
copyright
pounds
S
P
oe
OE
ae
AE
aa
AA
o
O
l
L
frac
ss
sqrt
ldots
cdots
vdots
ddots
alpha
beta
gamma
delta
epsilon
varepsilon
zeta
eta
theta
vartheta
iota
kappa
lambda
mu
nu
xi
pi
varpi
rho
varrho
sigma
varsigma
tau
upsilon
phi
varphi
chi
psi
omega
Gamma
Delta
Theta
Lambda
Xi
Pi
Sigma
Upsilon
Phi
Psi
Omega
ps
mp
times
div
ast
star
circ
bullet
cdot
cap
cup
uplus
sqcap
vee
wedge
setminus
wr
diamond
(?:big)?triangle.*
lhd
rhd
unlhd
unrhd
oplus
ominus
otimes
oslash
odot
bigcirc
d?dagger
amalg
leq
prec
preceq
ll
(?:sq)?su[bp]set(?:eq)?
in
vdash
geq
succ(?:eq)?
gg
ni
dashv
equiv
sim(?:eq)?
asymp
approx
cong
neq
doteq
propto
models
perp
mid
parallel
bowtie
Join
smile
frown
.*arrow
(?:long)?mapsto
.*harpoon.*
leadsto
aleph
hbar
imath
jmath
ell
wp
Re
Im
mho
prime
emptyset
nabla
surd
top
bot
angle
forall
exists
neg
flat
natural
sharp
backslash
partial
infty
Box
Diamond
triangle
clubsuit
diamondsuit
heartsuit
spadesuit
sum
prod
coprod
int
oint
big(?:sq)?c[au]p
bigvee
bigwedge
bigodot
bigotimes
bigoplus
biguplus
(?:arc)?(?:cos|sin|tan|cot)h?
csc
arg
deg
det
dim
exp
gcd
hom
inf
ker
lg
lim
liminf
limsup
ln
log
max
min
Pr
sec
sup
(SUPER|SUB)SCRIPTNB
(SUPER|SUB)SCRIPT
%%END SAFE COMMANDS

%%BEGIN TEXT COMMANDS
% Regex matching commands with a text argument (leave out the \)
addcontents.*
cc
closing
chapter
dashbox
emph
encl
fbox
framebox
footnote
footnotetext
framebox
part
(sub){0,2}section\*?
(sub)?paragraph\*?
makebox
mbox
opening
parbox
raisebox
savebox
sbox
shortstack
signature
text.*
value
underline
sqrt
(SUPER|SUB)SCRIPT
%%END TEXT COMMANDS 

%%BEGIN CONTEXT1 COMMANDS
% Regex matching commands with a text argument (leave out the \), which will fail out of context, but who's arguemtn should be printed as plain text
caption
%%END CONTEXT1 COMMANDS 

%%BEGIN CONTEXT2 COMMANDS
% Regex matching commands with a text argument (leave out the \), which will fail out of context, but who's arguemtn should be printed as plain text
title
author
%%END CONTEXT2 COMMANDS 


%% TYPES (Commands for highlighting changed blocks)

%DIF UNDERLINE PREAMBLE
\RequirePackage[normalem]{ulem}
\RequirePackage{color}\definecolor{RED}{rgb}{1,0,0}\definecolor{BLUE}{rgb}{0,0,1}
\providecommand{\DIFadd}[1]{{\protect\color{blue}\uwave{#1}}}
\providecommand{\DIFdel}[1]{{\protect\color{red}\sout{#1}}}                     
%DIF END UNDERLINE PREAMBLE

%DIF CTRADITIONAL PREAMBLE
\RequirePackage{color}\definecolor{RED}{rgb}{1,0,0}\definecolor{BLUE}{rgb}{0,0,1}
\RequirePackage[stable]{footmisc}
\providecommand{\DIFadd}[1]{{\protect\color{blue} \sf #1}}
\providecommand{\DIFdel}[1]{{\protect\color{red} [..\footnote{removed: #1} ]}}
%DIF END CTRADITIONAL PREAMBLE

%DIF TRADITIONAL PREAMBLE
\RequirePackage[stable]{footmisc}
\providecommand{\DIFadd}[1]{{\sf #1}}
\providecommand{\DIFdel}[1]{{[..\footnote{removed: #1} ]}}
%DIF END TRADITIONAL PREAMBLE

%DIF CFONT PREAMBLE
\RequirePackage{color}\definecolor{RED}{rgb}{1,0,0}\definecolor{BLUE}{rgb}{0,0,1}
\providecommand{\DIFadd}[1]{{\protect\color{blue} \sf #1}}
\providecommand{\DIFdel}[1]{{\protect\color{red} \scriptsize #1}}
%DIF END CFONT PREAMBLE

%DIF FONTSTRIKE PREAMBLE
\RequirePackage[normalem]{ulem}
\providecommand{\DIFadd}[1]{{\sf #1}}
\providecommand{\DIFdel}[1]{{\footnotesize \sout{#1}}}
%DIF END FONTSTRIKE PREAMBLE

%DIF CCHANGEBAR PREAMBLE
\RequirePackage[dvips]{changebar}
\RequirePackage{color}\definecolor{RED}{rgb}{1,0,0}\definecolor{BLUE}{rgb}{0,0,1}
\providecommand{\DIFadd}[1]{\protect\cbstart{\protect\color{blue}#1}\protect\cbend}
\providecommand{\DIFdel}[1]{\protect\cbdelete{\protect\color{red}#1}\protect\cbdelete}
%DIF END CCHANGEBAR PREAMBLE

%DIF CFONTCHBAR PREAMBLE
\RequirePackage[dvips]{changebar}
\RequirePackage{color}\definecolor{RED}{rgb}{1,0,0}\definecolor{BLUE}{rgb}{0,0,1}
\providecommand{\DIFadd}[1]{\protect\cbstart{\protect\color{blue}\sf #1}\protect\cbend}
\providecommand{\DIFdel}[1]{\protect\cbdelete{\protect\color{red}\scriptsize #1}\protect\cbdelete}
%DIF END CFONTCHBAR PREAMBLE

%DIF CULINECHBAR PREAMBLE
\RequirePackage[normalem]{ulem}
\RequirePackage[dvips]{changebar}
\RequirePackage{color}
\providecommand{\DIFadd}[1]{\protect\cbstart{\protect\color{blue}\uwave{#1}}\protect\cbend}
\providecommand{\DIFdel}[1]{\protect\cbdelete{\protect\color{red}\sout{#1}}\protect\cbdelete}
%DIF END CULINECHBAR PREAMBLE

%DIF CHANGEBAR PREAMBLE
\RequirePackage[dvips]{changebar}
\providecommand{\DIFadd}[1]{\protect\cbstart{#1}\protect\cbend}
\providecommand{\DIFdel}[1]{\protect\cbdelete}
%DIF END CHANGEBAR PREAMBLE

%DIF INVISIBLE PREAMBLE
\providecommand{\DIFadd}[1]{#1}
\providecommand{\DIFdel}[1]{}
%DIF END INVISIBLE PREAMBLE


%% SUBTYPES (Markers for beginning and end of changed blocks)

%DIF SAFE PREAMBLE
\providecommand{\DIFaddbegin}{}
\providecommand{\DIFaddend}{}
\providecommand{\DIFdelbegin}{}
\providecommand{\DIFdelend}{}
%DIF END SAFE PREAMBLE

%DIF MARGIN PREAMBLE
\providecommand{\DIFaddbegin}{\protect\marginpar{a[}}
\providecommand{\DIFaddend}{\protect\marginpar{]}}
\providecommand{\DIFdelbegin}{\protect\marginpar{d[}}
\providecommand{\DIFdelend}{\protect\marginpar{]}}
%DIF END BRACKET PREAMBLE

%DIF DVIPSCOL PREAMBLE
%Note: only works with dvips converter
\RequirePackage{color}
\RequirePackage{dvipscol}
\providecommand{\DIFaddbegin}{\protect\nogroupcolor{blue}}
\providecommand{\DIFaddend}{\protect\nogroupcolor{black}}
\providecommand{\DIFdelbegin}{\protect\nogroupcolor{red}}
\providecommand{\DIFdelend}{\protect\nogroupcolor{black}}
%DIF END DVIPSCOL PREAMBLE


%% FLOAT TYPES 

%DIF FLOATSAFE PREAMBLE
\providecommand{\DIFaddFL}[1]{\DIFadd{#1}}
\providecommand{\DIFdelFL}[1]{\DIFdel{#1}}
\providecommand{\DIFaddbeginFL}{}
\providecommand{\DIFaddendFL}{}
\providecommand{\DIFdelbeginFL}{}
\providecommand{\DIFdelendFL}{}
%DIF END FLOATSAFE PREAMBLE

%DIF IDENTICAL PREAMBLE
\providecommand{\DIFaddFL}[1]{\DIFadd{#1}}
\providecommand{\DIFdelFL}[1]{\DIFdel{#1}}
\providecommand{\DIFaddbeginFL}{\DIFaddbegin}
\providecommand{\DIFaddendFL}{\DIFaddend}
\providecommand{\DIFdelbeginFL}{\DIFdelbegin}
\providecommand{\DIFdelendFL}{\DIFdelend}
%DIF END IDENTICAL PREAMBLE

%DIF TRADITIONALSAFE PREAMBLE
% procidecommand color to make this work for TRADITIONAL and CTRADITIONAL
\providecommand{\color}[1]{}
\providecommand{\DIFaddFL}[1]{\DIFadd{#1}}
\providecommand{\DIFdel}[1]{{\protect\color{red}[..{\scriptsize {removed: #1}} ]}}
\providecommand{\DIFaddbeginFL}{}
\providecommand{\DIFaddendFL}{}
\providecommand{\DIFdelbeginFL}{}
\providecommand{\DIFdelendFL}{}
%DIF END FLOATSAFE PREAMBLE

%% SPECIAL PACKAGE PREAMBLE COMMANDS

% Standard \DIFadd and \DIFdel are redefined as \DIFaddtex and \DIFdeltex
% when hyperref package is included.
%DIF HYPERREF PREAMBLE
\providecommand{\DIFadd}[1]{\texorpdfstring{\DIFaddtex{#1}}{#1}}
\providecommand{\DIFdel}[1]{\texorpdfstring{\DIFdeltex{#1}}{}}
%DIF END HYPERREF PACKAGE


==> related.tex <==
% https://docs.google.com/spreadsheets/d/1JODWoEtDBxeOTr-ZqEqm3D-9wfADyNqgMoIOSpukBL0/edit#gid=0

\section{Related Work}
\label{sec:related}


Datacenter network topology.
Disaggregation.
Devices: pswitch, circuit switch, multi-host nic.

Intel IPU










\if 0
In this section, we review emerging network devices
and investigate whether they can be used to implement the
network resource pool, which, in turn provides network-as-a-service
for both disaggregated devices and regular servers.
Our focus is the support for disaggregated devices.
As it requires more functionalities and hence a super set of 
the ones required for regular server case.
Solutions work for the disaggregation setting would naturally
work for the regular-server cluster setting.

To this end, we propose a set of goals that a particular
solution must meet:
\boldpara{1) Port Count}.
The solution must be able to
support the exploded number of endpoints with
a cost-effective network topology.
\boldpara{2) Heterogeneous Endpoints}.
The solution should support various known computation mediums
such as FPGA, ASIC, and CPU, as well as any new ones in the future.
\boldpara{3) Transports and Network Functions}.
As we discussed earlier, the network resource pool is 
consolidating three types of resources: packet processing
in NIC, software network stack and advanced application-specific
network functions. The first type naturally comes with hardware.
The solution must have a mean to support the latter two.
\boldpara{4) Programmability}.
One of the key requirements for any current or future datacenters
is the ability to upgrade or re-program after deployment.
\boldpara{5) Consolidation, Manageability, and Multi-Tenancy}.
The core of pool is resource consolidation,
which relies on good management and multi-tenancy support.

Table~\ref{tabel-related-work} presents all the goals
and whether each reviewed network device or system can meet them.
Next, we will take a deep dive into each one.


\subsection{Programmable Switch}

\subsubsection{Primer}
Unlike traditional switches, the programmable switches
allow users to install specific actions on the switch data path.
thereby enable line-rate packet processing.
The core of programmable switch is Reconfigurable Match Table (RMT),
pioneered by a seminal SIGCOMM'13 paper~\cite{RMT-SIGCOMM13}.
RMT was first proposed to enhance OpenSDN deployment.
Since then, the programmable switches have seen great success in both industry and academic. 
P4~\cite{p4-paper}, a young domain-specific language specifically designed for packet processing, is the de-facto programming language for programmable switches. P4 greatly simplifies
packet manipulation and has helped the wide adoption of programmable switches.

The arise of programmable switch shifted the network computation paradigm:
it breaks the common belief held by distributed system designers
and opens doors to improve, redesign, or create distributed systems in unimaginable ways.
In essence, programmable switch is a centralized computation point
that can mitigate synchronization and consistency issues,
acting as cache front end, or simply be a network function offloading unit. 
Recent systems demonstrate performance improvements in domains like
caching for KV~\cite{netcache-sosp17, incbricks-asplos17},
caching for load-balancing~\cite{distcache-fast19},
in-network coherence directories~\cite{pegasus-osdi20},
congestion control~\cite{hpcc-sigcomm19},
distributed lock management~\cite{netlock-sigcomm20},
databases~\cite{cheetah-sigmod20},
scheduling~\cite{racksched-osdi20},
and network function processing~\cite{tea-sigcomm20}.
%consensus,
%machine learning,

Most recently, researchers started using programmable switches
to consolidate computation resource.
Wang et al.~\cite{wang-hotcloud20} observes programmable switches are
heavily under-utilized, hence use a set of
compile/run-time techniques to deploy multiple p4 programs
onto one programmable switch, thereby enabling multi-tenancy and consolidation.
TEA~\cite{tea-sigcomm20} consolidates NFs at rack-scale,
providing NF-as-a-service to the servers under the ToR switch.
Das et al.~\cite{active-hotnets20} takes a fresh look at
active networking and uses p4 to turn a programmable switch
into a physical computing device akin to a virtual machine.

\subsubsection{Feasibility}

Programmable switch has limited number of ports,
e.g., 64 ports for Intel Tofino2, hence not able to
accommodate the exploded number of disaggregated devices.
Further, with the diminishing of Dennard Scaling and Moore's Law,
the merchant chip is not likely to see dramatic computation power increase,
which in turn limits the number of ports a certain chip can support.

Most of commodity programmable switches are Ethernet-based.
To communicate with such switches,
an endpoint requires an Ethernet gear
(could be any physical form: a chip, a device, or integrated IPs)
with at least L1 and L2 functionalities (i.e., a PHY and a MAC). 
Since all disaggregated devices are directly attached to the network,
it is reasonable to assume they have such Ethernet gear equipped.
As for regular servers, they already have NIC installed.
In all, programmable switches are able to support heterogeneous devices.
Note that both the switch and the endpoints are free to
use other physical and link layer protocols (e.g., Infiniband),
there is nothing fundamental about using Ethernet except it is
already widely used so its beneficial continue using it.

As we mentioned earlier, several work~\cite{tea-sigcomm20,active-hotnets20,wang-hotcloud20}
have tried to consolidate NFs and applications onto programmable switches.
No work has tried to build transport on it, though we believe it is doable.
However, the multi-tenancy support is still at its infancy.
Most of the existing work leverage compile-time tricks to
overcome hardware limitations, which result in some inevitable cost.
With enough momentum, the vendors might wight in and develop certain
virtualization features on programmable switches.
It would be interesting to explore what those features might be.

\subsubsection{Summary}

For both regular server's network disaggregation and consolidation,
programmable switches can partially meet their goals.
Servers can offload their transport processing,
network functions, and advanced application-specific functions to
the programmable switches -  this is already possible now.
However, current commodity programmable switches
are not able to meet the goals for disaggregated datacenter.
Specifically, it is not able to solve the exploded port counts
without a significant increase in cost.

%What about line cards.

\subsection{Circuit Switch}

\subsubsection{Primer}

Circuit switch establishes a dedicated channel between
endpoints connected to it. It guarantees the full bandwidth
of the channel and remains connected for the duration of a
certain session. It creates an illusion as if endpoints are
directly and physically connected.

Circuit switch operates at the physical layer with no buffers,
no arbitration, and no packet inspection mechanisms.
Thus, they are cheaper and more power-efficient than
traditional electrical packet switch. As a result,
circuit switches could support hundreds or even thousands of
ports with lower CAPEX and OPEX than equivalent packet switches,
making it a good candidate to interconnect disaggregated devices in a rack.

Circuit switch has seen great improvement over the previous decade.
Around 2010, Helios~\cite{helios-sigcomm10} first proposes to integrate circuit switches into
the datacenter network and uses a hybrid packet and circuit switching mode.
Mordia~\cite{mordia-sigcomm13} improves the switching time from
tens of milliseconds to microsecond level. In response, Mordia proposes
a proactive scheduling mechanism instead of a reactive one.
REACToR~\cite{reactor-nsdi14} leverages Mordia's fast switching and builds a hybrid
ToR using both packet and circuit switches, enjoy the benefits of both.
But REACToR is sensitive to the traffic pattern.
Until then, circuit switch solutions were tightly coupling
their data plane with the control plane. The control plane
reconfigures the switches in response to traffic demands.
Such solutions cannot scale well.
Hence, RotorNet~\cite{rotornet-sigcomm17} proposes a fully decentralized
control plane solution using specialized hardware and a round-robin policy.
In addition, RotorNet can scale to 1000s of ports with 10 us switching delay.
The latest work, Sirius~\cite{sirius-sigcomm20} achieves nanosecond-level
switching time (3.84 ns for end-to-end reconfiguration).
Overall, the state-of-the-art circuit switch is able to
achieve fast nanosecond-level switching, works with decentralized control plane,
while still able to provide high port counts and consumes very little energy.
Given the foreseeable limitations of electrical packet switch,
circuit switch is gradually making its way into datacenters (e.g., Shoal~\cite{shoal-nsdi19} and dRedBox~\cite{dRedBox-DATE}).

\subsubsection{Feasibility}

Clearly, circuit switch is a good candidate to deploy networks in disaggregated datacenters.
As it supports high port counts hence able to accommodate the exploded number of devices.
Further, circuit switch is able to overcome the over-subscription problem while operating
with very low energy consumption compared to traditional packet switch.

To use circuit switch,
endpoints need to use specialized physical and link layer protocols,
with companion upper layer software~\cite{alex-thesis2020}.
This is relatively easier to achieve in servers with regular NICs
than the heterogeneous devices.
Past work has built an FPGA-based NIC~\cite{alex-thesis2020} for this purpose.
Similar to the programmable switch case,
we anticipate devices using circuit switch would incorporate customized network gear (e.g., a device, a chip, or IPs).

However, circuit switch is not able to
run any computation other than the scheduling algorithm (if any).
Unlike electrical packet switch which encapsulates the control complexity
within the switch, circuit switch \textit{exposes} the control complexity
to the rest of the network~\cite{rotornet-sigcomm17}.
Hence, circuit switch is not able to meet any other goals requiring computation.

\subsubsection{Summary}

Circuit switch has several appealing traits
such as high port counts, power efficient, and excellent scalability.
These make it a good candidate to \textit{build} disaggregated datacenters,
but not necessary for network consolidation.
Its lack of computation power is the key limitation.
If future circuit switch technologies are able to incorporate
any form of computation, then it would become one of the best choices
to build network resource pool.

\subsection{Coherent Fabrics}
\subsubsection{Primer}

In recent years, there are several industry proposals to build new interconnect
fabrics across endpoints in a server or in a rack.
They include Gen-Z~\cite{GenZ}, CXL~\cite{CXL}, OpenCAPI~\cite{OpenCAPI}, and CCIX~\cite{CCIX}.
These fabrics usually provide a universal memory interface and hardware-level memory/cache coherence across different endpoints.

Gen-Z~\cite{GenZ} is a new datacenter-scale fabric providing low latency
and high bandwidth accesses to remote resources.
It supports byte-addressable memory access, block memory access, and
accelerator-specific messaging interface.
Gen-Z is a full-stack solution, it specifies the physical layer,
link layer, network layer, transport layer, and above virtual memory interfaces.
It also defines its own routers and switches.
Each Gen-Z compliant device has a Gen-Z controller attached.
This controller translates user requests into Gen-Z requests
and sends to remote.

OpenCAPI~\cite{OpenCAPI}, CCIX~\cite{CCIX}, and CXL~\cite{CXL}
are all intra-server memory coherent interconnects.
OpenCAPI attaches CPUs to accelerators and I/O devices with minimal overhead.
It provides coherent memory interface across CPU and various devices.
CCIX provides a similar set of features.
On top of those capabilities, CXL further exposes a window directly
into the processor caching hierarchy.
All of them use the widely available PCIe physical and link layer to transmit data within the chassis.

Recently, CXL and Gen-Z consortium announced that
they will bridge their protocols and improve compatibility.
It is likely that in the near future,
CXL could be extended out beyond server boundary
and have coherent access to remote memory (or accelerators) via Gen-Z.
%Likewise, IBM has OpenCAPI has been extended to access disaggregated memory.
Those emerging coherent fabric protocols are gradually
making their ways into datacenters and being used for disaggregation purpose.

\subsubsection{Feasibility}

We will focus on Gen-Z as it is the only datacenter-scale fabric for now.
Unfortunately, there are no commercial Gen-Z products available, so we will
draw our discussion purely based on its latest specification~\cite{GenZ}.

In theory, Gen-Z's topology is able to support high port count.
It uses a combination of routers and switches, and they can be
customized for high port count.
However, they run at link layer or network layer,
thereby lacking any other computation power.
Hence, they are not able to support packet processing offload, nor resource consolidation.

As Gen-Z attaches its own controller to each device,
it is able to support any types of heterogeneous devices.
Also, it supports per-device customization.

\subsubsection{Summary}

Most of the emerging coherent fabrics are still under heavy development
(except OpenCAPI, which is already used in IBM Power series), no commercial
products are available. All of them have great potentials but with high uncertainties.

The main obstacle in adopting these fabrics is the requirement to
replace existing network infrastructure with new switches and new hardware network controllers (one at each endpoint).
These controllers cannot be easily managed or reconfigured, and they are not programmable.

Although these emerging coherent fabrics
are beneficial for traditional disaggregation on compute or memory,
they cannot satisfy the requirements for network disaggregation.

\subsection{Middleboxes and NFV}
\subsubsection{Primer}

Middleboxes, also known as hardware-based network appliances, originally
resided in specialized hardware boxes from various vendors.
They provide network functionalities such as firewall, packet filtering,
NAT, load balancing, and so on.
They are mostly black boxes for network operators.

In the early 2000s, people were still championing middleboxes~\cite{walfish-osdi04}.
But starting form early 2010s, as the workloads were rapidly changing,
people started questioning middleboxes' black box nature
and proposed software-centric middlebox deployment,
which resulted in consolidated middlebox architecture~\cite{comb-nsdi12}.
Around the same time, APLOMB~\cite{aplomb-sigcomm20} took a step further
by outsouring enterprise middleboxes processing all together to the cloud.
Despite middleboxes' usefulness and ubiquitousness, they come with
a set of problems, many of which arise from the fact that they are
hardware-based: they are costly, difficult to manage, and their
functionality is hard or impossible to change.

In response, also in the early 2010s,
the Network Function Virtualization (NFV) concept was proposed.
NFV advocates moving traditional network functions out of
proprietary middleboxes into virtualized software applications
that can be run on commodity, general purpose processors.

The past decade was a golden age for NFV.
Along the timeline, it is very clear what researchers were
focusing on at their time.
In the beginning, single-machine solutions such as ClickOS~\cite{clickos-nsdi14} arise just to enable virtualized
NF development. Not soon after, E2~\cite{e2} was proposed
to help distributed NF deployment. E2 deals with a set of typical
distributed system issues such as failure handling and scaling.
However, during 2016, despite all the promised benefits of NFV,
there has been little progress towards large-scale deployment.
One of the reasons is performance degradation due to virtualization.
Hence, NetBricks~\cite{netbricks} uses safe language Rust to avoid that.
In the same vein, Metron~\cite{metron-nsdi18} and ResQ~\cite{resq-nsdi18}
also propose low-level processor hacks to improve single machine efficiency.

It was clear that CPU will not be able to keep up with the
fast growing network speed.
As a result, there was a renewed interest in moving NFV
back to specialized hardware.
Notably, early work ClickNP~\cite{clickos-nsdi14} deploys NF to
FPGA-based programmable NICs.
FPGA provides massive cheap parallelism and is an ideal medium to run NFs.
Many work followed~\cite{flowblaze-nsdi19,panic-osdi20} and Microsoft
has deployed FPGA-based NF platform in their Azure cloud~\cite{azure-nsdi18}.

Over the years, the whole space moved from specialized middleboxes
to consolidated software-based NFs, and finally find their
way back to using specialized hardware.
But unlike original closed middleboxes, these new hardware (e.g., programmable switch or programmable NIC) are open, programmable,
and supported by the community at large.

\subsubsection{Feasibility}

Both middleboxes and NFV are not able to provide
high number of ports. As the former being a specialized box
and the latter mostly runs on commodity hardware.
Likewise, both of them cannot support heterogeneous endpoints
, nor can they support offloaded transports.
By design, both of them are able to run offloaded NFs. 

Similarly, both of them could support resource consolidation.
Prior work has tried to consolidate middleboxes~\cite{comb-nsdi12}.
As for NFV consolidation, TEA~\cite{tea-sigcomm20} accomplish that using programmable switches,
PANIC~\cite{panic-osdi20} uses programmable NIC,
and SNF~\cite{snf-socc20} uses a serverless framework.
For manageability, middleboxes' closed system nature makes it hard to manage and scale.
On the contrary, NFV is relatively easier to manage and has much more mature systems.

\subsubsection{Summary}

Overall, middlebox is no longer considered a good
solution for future datacenter development,
as its black box nature cannot fit in.
NFV systems are more diverse and open,
in which both hardware and software have open standard and
backed by the community.
For regular server datacenters,
NFV has already been consolidated and provided as a service~\cite{tea-sigcomm20,snf-socc20,panic-osdi20}.
However, none of these systems is able
to do so for disaggregated datacenters.


\subsection{Multi-host NIC}
\subsubsection{Primer}
Multi-host NIC~\cite{Intel-RedRockCanyon,Mellanox-Multihost}, as its name suggests, is a physical NIC shared by multiple hosts.
It connects to hosts via extended PCIe cables.
It appears as independent NIC to each host.
Internally, it can partition its uplink bandwidth among connected hosts,
follow a certain policy (e.g., fair partition).
To host, it is no different than using a normal exclusive NIC,
hence each host runs its own network stack.
Multi-host NIC is proposed to consolidate network resources
in virtualized environment, but it has never been widely deployed.

\subsubsection{Feasibility}

Multi-host NICs reduces the number of ports ToR switch needs,
and it consolidates traditional NIC functionalities.
However, it still requires each end host to run its transport and network
functions in software.
Also, multi-host NICs do not support programmability or rapid on-field upgradability.

\subsubsection{Summary}

Multi-host NIC can meet the port count goal.
Since it is using a more general PCIe interface, it could
potentially support heterogeneous devices.
Although it is designed to consolidate resources,
it only does so for physical and link layer resources.
Higher level protocols such as transports and network functions
cannot be offloaded to the multi-host NIC.

\subsection{Summary of Network Device Review}

We have now reviewed programmable switch,
circuit switch, coherent fabrics, middleboxes, NFV, and multi-host NIC.
Table~\ref{tabel-related-work} summarizes whether each system can meet
the goals for network disaggregation and consolidation.
Unfortunately, none of them can make the cut.
Programmable switch and NFV are the closest solution for regular-server
datacenter, but they are not able to solve exploded port count and
to accommodate heterogeneous devices. Coherent fabrics and multi-host NIC
are able to meet specific goals for disaggregated datacenter, but
lack the support for computation offload and consolidation.

We find that programmable switch, circuit switch, and NFV
all made their first appearance in the early 2010s.
The past decade has witnessed their rapid growth:
programmable switch and NFV are widely deployed in
datacenters~\cite{hpcc-sigcomm19,azure-nsdi18};
though circuit switch has received less adoption,
it is gaining its momentum~\cite{dRedBox-DATE,sirius-sigcomm20}.

\textit{But are they the right devices to build next decade's datacenter network?}
Our answer is no.
We think the next-generation datacenter,
including regular-server and disaggregated,
should use a disaggregated and consolidated network,
for the reasons in Section~\ref{sec:motivation}.
But none of the above device is able to meet our goals.
As a result, we propose a new device called \sysname,
which meets all the goals in Table~\ref{tabel-related-work}
\fi

==> system.tex <==
\section{System}
\label{sec:system}


==> tbl-related-work.tex <==
{
\begin{table*}[th]\smallsize
\begin{center}
\begin{tabular}{ p{1.7in} | p{0.5in} | p{0.85in} | p{0.6in} | p{0.55in} | p{0.8in}  | p{0.7in} }

\textbf{Solution} & \textbf{Port Count \textasteriskcentered} & \textbf{Heterogeneous End-Points \textasteriskcentered} & \textbf{Offloaded Transport} & \textbf{Network Function} & \textbf{Manageability} & \textbf{Consolidated Resources} \\
\hline
\hline
Programmable Switch~\cite{RMT-SIGCOMM13,netcache-sosp17} & \xmark & \cmark & \cmark & \cmark  & $\bigcirc$  & $\bigcirc$ \\
\hline
Circuit Switch~\cite{sirius-sigcomm20,shoal-nsdi19,dRedBox-DATE} & \cmark & \cmark & \xmark & \xmark  & \xmark  &\xmark \\
\hline
Coherent Fabrics~\cite{GenZ,CXL,CCIX} & $\bigcirc$ & \cmark & \xmark & \xmark & \xmark & \xmark\\
\hline
Middleboxes~\cite{walfish-osdi04,comb-nsdi12,aplomb-sigcomm20} & \xmark  & \xmark  & \xmark & \cmark & \xmark  & \cmark  \\
\hline
NFV~\cite{clickos-nsdi14,e2,netbricks} & \xmark  & \xmark  & \xmark & \cmark & \cmark & \cmark \\
\hline
Multi-Host NIC~\cite{Intel-RedRockCanyon,Mellanox-Multihost} & \cmark &  $\bigcirc$ & \xmark & \xmark & \xmark  & $\bigcirc$ \\
\hline
\hline
\textbf{\sysname}     & \cmark & \cmark &  \cmark & \cmark & \cmark & \cmark \\
\hline
\end{tabular}
\end{center}
\mycaption{tabel-related-work}{Comparison of Network Solutions.}
{
\textasteriskcentered\ features only applicable to disaggregated datacenters.
$\bigcirc$ partially support.
}
\end{table*}
}


==> tbl-techniques.tex <==
% https://homes.cs.washington.edu/~arvind/papers/pcp.pdf

{
\begin{table*}[th]\footnotesize
\begin{center}
\begin{tabular}{ p{1in} | p{1.5in} |p{3.3in} | p{0.5in}}

\textbf{Goal} &
\textbf{Mechanism} &
\textbf{Description} &
\textbf{Section} \\
\hline
\hline

Connectivity            & Reliable link layer & enable connection between supernic and endpoints & XX \\
\hline
Endpoint Integration    & Endpoint shim layer & APIs and lighteweight states & XX \\
\hline
\hline

Perf & Partial NF Chaining & XXXX  & XXX \\
\hline

Perf & Service-level Parallelism & XXXX  & XXX \\
\hline

Perf & Instance-level Parallelism & XXXX  & XXX \\
\hline

Correctness & Reorder Buffer & parallel services and instances & XXX \\
\hline

Perf \& Security & Resource Partition & Partition resource to improve aggregated on-board throughput & XXX \\
\hline
\hline

Management & Softcore & Runs management plane (all policies) & XX \\
\hline

Consolidation & Packet Store & Shared central packet buffer & XX \\
\hline

Fairness & Credit Allocation & Eager and \& on-demand policies & XXX \\
\hline

Fairness & Header/PIFO Queues & XX & XXX \\
\hline

XX & NF Wrapper & XXXX & XXX \\
\hline

Security & Segmented VM & XXXX & XXX \\
\hline


PR Facility & PR Region Decoupler & Logically isolates static and dynamic PR regions, with quiescence API & XXX \\
\hline

Computation Scaling & PR-based Auto Scaling & PR can replace, add, and remove NFs during runtime & XXX \\
\hline

Computation Scaling & Bitstream Store & A table of bitstreams saved in on-board DRAM & XXX \\
\hline

Better Deployment & Bitstream AutoGen & A framework to generate wrapped bitstreams using user netlists & XXX \\
\hline


\end{tabular}
\end{center}
\mycaption{table-techniques}{Technique Summary.}
{
PR: Partial Reconfiguration.
NF: Network Function.
}
\end{table*}
}


==> tbl-two-tbl-example.tex <==
{
\begin{table*}[th]\footnotesize
\begin{minipage}{\figWidth}
\begin{center}
\begin{center}
\begin{tabular}{ c | c | c | c  }
\small  & \small  & \small  & \small  \\
\hline
 &  &  &  \\
 &  &  &  \\
 &  &  &  \\
 &  &  &  \\
\end{tabular}
\end{center}
\mycaption{tbl-tbl1}{Empty Table.}
{
blablabl
}
\end{center}
\end{minipage}
\begin{minipage}{\figSep}
\hspace{\figSep}
\end{minipage}
\begin{minipage}{\figWidth}
\begin{center}
\begin{center}
\begin{tabular}{ c | c | c | c | c | c }
\small Workload & \small Read & \small Update & \small Scan & \small Insert & \small R/U \\
\hline
A & 50\% & 50\% & - & - & - \\
B & 95\% & 5\% & - & - & - \\
C & 100\% & - & - & - & - \\
D & 95\% & - & - & 5\% & - \\
E & - & - & 95\% & 5\% & - \\
F & 50\% & - & - & - & 50\% \\
\end{tabular}
\end{center}
\mycaption{tbl-tbl2}{YCSB Workload Properties.}
{
blablabla
}
\end{center}
\end{minipage}
%\vspace{-0.1in}
\end{table*}
}

